Why did developers migrate Android applications from Java to Kotlin?

Currently, the majority of apps running on mobile devices are Android apps developed in Java. However, developers can now write Android applications using a new programming language: Kotlin, which Google adopted in 2017 as an official programming language for developing Android apps. Since then, Android developers have been able to: a) start writing Android applications from scratch using Kotlin, b) evolve their existing Android applications written in Java by adding Kotlin code (possible thanks to the interoperability between the two languages), or c) migrate their Android apps from Java to Kotlin. This paper aims to study this last case. We conducted a qualitative study to find out why Android developers have migrated Java code to Kotlin and to bring together their experiences about the process, in order to identify the main difficulties they have faced. To execute the study, we first identified commits from open-source Android projects that have migrated Java code to Kotlin. Then, we emailed the developers that wrote those migrations. We thus obtained information from 98 developers who had migrated code from Java to Kotlin. This paper presents the main reasons identified by the study for performing the migration. We found that developers migrated Java code to Kotlin in order to access programming language features (e.g., extension functions, lambdas, smart casts) that are not available with Java for Android development, and to obtain safer code (i.e., avoid null-pointer exceptions). We also identified research directions that the research community could focus on in order to help developers to improve the experience of migrating their Java applications to Kotlin.

==> Migration Kotlin-Java_4rev/future_research_challenges.tex/future_challenges_original.tex <==


\subsection{Main challenges that could be targeted by the research community}
\label{sec:directions}

In this paper we conducted an \emph{exploratory} survey, which are used as pre-study to a more thorough investigation, and may provide new possibilities that could be analyzed and should therefore be followed up in the more focused or thorough survey \cite{experimentationSE2012}. 
In this section, we present those new possibilities that may be exploited by the research community.


\point{Auto-converter tools:}
The survey we conducted show that developers have used the auto-converter code and have modified the output code to have a more idiomatic code.
The automated-generated code is like \quotes{code written with Kotlin syntax but still keeping Java style}.
The potential research directions are twofold. 
First, to detect the cases where Java code that is not correctly converted by state-of-the-art tools.
Second, to define new automated code conversion approaches and tools which generate idiomatic code, and consequently, attempt to reduce the modifications that developers have to do. 
For example, an initial work by Courtney and Neilsen \cite{CATA2019:Vetting} presents an alternative conversion tool.


\point{Detection of technical debt:} 
\emph{Technical-debt} issues can appear on application after it was (partially or fully) migrated.
According to Avgeriou et al.~\cite{avgeriou_et_al:DR:2016:6693} the term \emph{technical debt} refers to delayed tasks and immature artifacts (code, architecture, design) that incur extra costs in the future in the form of increased cost of change during evolution and maintenance. 

A research challenge is to identify, define,  model, and catalogue,   technical-debt~\cite{Izurieta2016WorkingTD} associated to the migration from Java and Kotlin.
Other works has focused, for instance, on defining and analyzing the architecture of Android applications (e.g.~\cite{Verdecchia2019Guidelines,Bagheri2016ArchitetureAndroid}) and on the detection of \emph{architectural} technical debt issues (e.g. \cite{Verdecchia2018ATD}).
However, to our knowledge, no work has done studied the impact of the migration on the architecture of the application nor the technical debt that the migration could introduce.


\point{Refactoring  Kotlin code after migration:}
A challenge for researchers is to define approaches and tools that propose \emph{refactorings} on Kotlin applications after the migration is (partially or fully) done.
We envision two directions.
First, to identify (and potentially automatically remove) \emph{code} technical-debt items (such as code smells and code patterns~\cite{avgeriou_et_al:DR:2016:6693}), previously identified and catalogued. 
According to Snipes and Jedlitschka~\cite{avgeriou_et_al:DR:2016:6693} common tools that support automated refactoring do not address more elaborate technical debt items such as code smells and code patterns. 
Moreover, tools that identify and remove code smells (such as JDeodorant~\cite{Tsantalis2008JDeodorant}) target to Java code. To our knowledge, no refactoring tool targets Kotlin code.
Secondly, we envision refactorings that make Kotlin code (human written or generated by a tool) more idiomatic. 
For example, one could propose the use of new Kotlin features not previously used by the developer, such as \emph{smart casts} or \emph{named parameters}.

\point{Supporting migration activity:}
A potential research direction is to define guidelines, approaches and tools which help developers to migrate their apps.
\emph{Gradual} migrations are convenient for migrating large applications (e.g. Duolingo~\cite{duolingo_migration2020}), because it allows developers and companies to migrate some parts of their apps at the same time they evolve other parts, add new features and release new versions.
 

Gradual (or iterative) migration has been already studied on legacy applications~(e.g., \cite{DeLucia2008DevelopingLegacy}) and consists on first decomposing the legacy apps~\cite{Brodie1995Legacy} and then integrating the decomposed parts using \emph{wrappers} (e.g.,~\cite{CANFORA200099}). 
On the contrary, migration from Java and Kotlin does not need such wrappers, as both languages are interoperable. 
There, a developer needs to define a \emph{migration strategy} which defines consecutive migration steps, and for each of them, a subset of components or code files to be migrated.
This could be a challenging task, specially on large applications: the wrong selection of files to be migrated could increase the migration effort due to emerging errors~\cite{AbdelAziz2020MigEnterprise}. 
We envision the definition of guidelines, approaches and tools which help developers to define a migration strategy and to select the files, packages, or components to be migrated in one particular step in order to minimize the migration effort.


\point{Estimating cost of migration:}
One of the main problems about migrations reported by our survey and by literature on migration (e.g., \cite{Khadka2014LegacyModernization}) is about unfinished migrations due to lack of time or resources.
Models for estimating cost and effort of migration could help developers and companies to  forecast those issues.
Cost and effort estimation of development and maintenance activities has been widely studied during last 30 years (see survey from~\cite{Jorgensen2007SurveyCost}).
A challenge for researchers on migration is to define models that estimate the cost of \emph{migrating} Android apps to Kotlin. 
For that, we envision the estimation of three costs:
\begin{inparaenum}[\it 1.]
\item  cost of migrating the code from Java to Kotlin (C1),
\item cost of  maintaining the migrated Kotlin code (C2), and
\item cost of  maintaining the existing code without migrating it to Kotlin (C3) (which could computed based on existing costs models e.g., \cite{Jorgensen1995,KITCHENHAM200257}).
\end{inparaenum}
Then, by comparing those costs (i.e. C1 + C2 vs C3), developers could better support their decisions about to migrate or not, and consequently, to eventually save time, effort and money.

\point{Kotlin code comprehensibility:} Some participants from our survey mentioned us that the compact syntax of Kotlin affected the readability of code.
A research direction could focus on empirically studying the comprehensibility of Kotlin code.
For doing that, it would be necessary to implement static code analysis tools and to, potentially, define new comprehensibility measures that target Kotlin code.
As pointed by Wyrich et al. ~\cite{Wyrich2020Comprehensibility} those tools would attempt to automatically measure code comprehensibility, to point out sections of the code that are difficult to comprehend and should therefore be refactored.
To our knowledge, there is  no previous work on comprehensibility of Kotlin code.


\point{Testing of migrated apps}:
A research challenge is to generate test cases which 
\begin{inparaenum}[\it a)]
\item  do \emph{regression testing} after the migration (i.e., to verify the behaviour of the app has not change after the Java to Kotlin conversion)
\item verify the migrated code does not introduce new bugs.
\end{inparaenum}
One of the challenges we envision is to test the interaction between the migrated Kotlin code with the no migrated Java code.
Even both languages are interoperable, Kotlin is a null safe language, it tries to avoid nullable variables.
Consequently, the behaviour of the application can change (i.e., an exception is thrown) when the Java code passes \emph{null} values to the migrated Kotlin code, which could be written without contemplating the nullability of parameters and variables.



==> Migration Kotlin-Java_4rev/links_gray_biblio.tex <==
Section 3.1.1 
"One of them one told us:
In short I was sick of using java. As a professional android developer there is no reason to use java, especially the incredibly limited version of java you get on Android.}
The majority of the interviewed developers stated that migrating to Kotlin was a way to ``hack'' this problematic: Kotlin provides  moderns features (e.g., lambdas, data class, smart cast, null safe)"
https://dzone.com/articles/java-vs-kotlin-which-programming-language-is-bette -> See the section Kotlin Is the "Modern" Language 
https://blog.udemy.com/kotlin-vs-java-9-benefits-of-kotlin-for-your-business/ -> Third benefit

Section 3.1.2
"Kotlin eliminates the possibility of empty pointers froma compilation perspective: potential NPEs are detected at compile time instead of crashing apps at runtime" 
https://blog.udemy.com/kotlin-vs-java-9-benefits-of-kotlin-for-your-business/ -> second benefit
https://dzone.com/articles/java-vs-kotlin-which-programming-language-is-bette ->Section Issue With NullPointerExceptions
https://www.rishabhsoft.com/blog/kotlin-for-android-development
https://www.androidauthority.com/kotlin-vs-java-783187/
https://docs.google.com/document/d/1ReS3ep-hjxWA8kZi0YqDbEhCqTt29hG8P44aA9W0DM8/edit#heading=h.v6i4iyf7kkxh -> The author of this document is a very well-know Android developer, he was the creator of famous Android Library
https://engineering.talkdesk.com/migrating-from-java-to-kotlin-the-easy-way-37b25a379d72
http://petersommerhoff.com/dev/kotlin/kotlin-for-java-devs/#what-now
https://engineering.autotrader.co.uk/2020/02/21/migrating-to-kotlin-what-to-look-out-for.html
Section 3.1.3
https://dzone.com/articles/java-vs-kotlin-which-programming-language-is-bette -> Community support
https://dzone.com/articles/java-vs-kotlin-which-language-android-developer-sh -> "Even though currently, almost all Android code, examples, and apps are in Java, it will change in the future because Google has declared Kotlin as the official language for Android app development. Many companies have already started using Kotlin for their Android app development, and that's the main reason I think Java developers should learn Kotlin in 2018."
https://www.techrepublic.com/article/should-android-devs-switch-from-java-to-kotlin-heres-googles-advice-on-swapping-programming/
Other links:
https://www.toptal.com/android/kotlin-boost-android-development

==> Migration Kotlin-Java_4rev/logs.tex <==

Red-moon
commit ed27961ca829124dcf81ff40945394dc6d268b4d
Author: Stephen Michel <stephen.michel@tufts.edu> 2016-11-11 01:19:09
Committer: Stephen Michel <stephen.michel@tufts.edu> 2016-11-11 01:19:09
Parent: 52a4c3933bfeca188dc8fa398ac0098c59891882 (fix errors in automatic kotlin conversion)
Child: de6b6843cad3e56d3271db4f81ebe1d686e6d306 (fix build errors and some warnings)
Branches: master, origin/HEAD, origin/feature_android-tv, origin/master, origin/onboarding, origin/root-mode, origin/tileLogging, origin/v1-rootmode

Mostly functional location switch. convert to kotlin because studio is stupid.

Automatic conversion also automatically stages the file, making it impossible
to for me to separate changes I made before converting (which were going to
be in a separate commit) and the conversion itself. Thanks, Obama.


==> Migration Kotlin-Java_4rev/migratedExamples.tex <==
Case one commit migrated (in branch Develop) but not merged into the master:

``This branch is 4 commits ahead, 1 commit behind master.''

https://github.com/fennifith/Status/compare/develop

https://github.com/fennifith/Status/commit/5790480a4176f1dc089d42169955cafd5b5e73c9


## https://github.com/k9mail/k-9/compare/manage-folders-item


## lot of commits in develop branch
https://github.com/TwidereProject/Twidere-Android





==> Migration Kotlin-Java_4rev/old-content/notes-ideas.tex <==



%%% An idea of story:

Does Kotlin help developers to write Android apps with better quality?

If yes: 

How can be help Java developers to 
migrate Java apps to Kotlin?
encourage and help to start developing on Kotlin?

If no:

Which features of Kotlin must evolve for a massive adoption? (Note: maybe out of scope for us, but, we can collaborate with JetBrains -I have a contact there-)
%%



\mcomment{Remark the option to upload patterns -preload patterns already discovered-}
\mcomment{To preload is the key for the gerenal experiment: compute patterns from all projects, then load, then compute frequency (intra-extra-projects)}

\mcomment{Recall two step pattern recognition: patterns coming from individual mappings}

\mcomment{Diffs of patterns}


\mcomment{The algorithm also shows if we consider the parents of the affected node: we can scale up in the affected AST.}

\mcomment{Role matching}

\mcomment{two additional matching features: considering context (Parent) + Roles in labels}


\mcomment{Users using rename command}




What happen in the migration.
e.g. in the Java code when a file is migrated.
1 file is migrated, the other is 

Migration
a1dcbf9f97202bb85d2cb5fc4873dc16854f1a86

Test
eed2f2ec3dabb28199450c54aae6745125adead0

%Patterns from mappings:
%The algorithm  has the ability to add to the pool patterns  

==> Migration Kotlin-Java_4rev/old-content/old_miga.tex <==
\section{\miga{}: a framework for analyzing the migration of an application along its software history}
\label{sec:migaframework}

\subsection{Goals of \miga{}}
\label{sec:miga_goal}

\miga{} is a framework for studying the evolution of software applications i.e., the changes done over an application along its history.
In particular, \miga{} focuses on studying applications that, during its evolution, have been migrated to one programming language to another (or others).
Thus, \miga{} aims at extracting knowledge about that languages migration activity.
This extracted knowledge would allow a researcher to understand how developers use new technologies (e.g., emerging programming languages used -specially- in mobile such as Kotlin), and to characterize the migration activity from one technology (e.g., Java) to another (e.g, Kotlin).

%the history of applications of that have been migrated from one or more program language to another (or others)  with the goal of extract knowledge about the language(s) migration.

\subsection{\miga{} in a Nutshell}
\label{sec:miga_nutshell}

%Figure \ref{} shows the steps done by \miga.
 \miga{} receives as input a list of versions of one applications (chronologically ordered) and produces as output the summary of its evolution including all the information about the migration from one language to another.
That output contains for each version $v_i$ different information such the program languages affected in that version, the changes done by $v_i$ at different levels (e.g., line and AST level), and the different change patterns found.



\subsection{Architecture and Implementation of \miga{}}
\label{sec:architecture}

The \miga{} framework is built on top of Coming \cite{coming2019}, a framework built on Java for studying the evolution of applications.
\miga{} frameworks takes as input the location of a GIT repository on disk.
It navigates each commit in chronological order, starting from the oldest one.
Each \emph{commit} adds, removes or introduces changes into \emph{files}, producing a new version of the application.

Beyond Git repositories, Coming (and consequently \miga{}) is capable of analyzing other types of inputs such as pairs of files located in the file system.\footnote{\url{https://github.com/SpoonLabs/coming/blob/master/docs/extension_points.md#input-reader}}


\miga{} applies over each commit a series of \emph{Analyzers}.
Analyzers are organized as a pipeline: each one does a specific task, takes as input all the files affected by the commit (including added, removed, modified files), processes the input, and finally passes the result of its analysis (in addition to the input received) to the next analyzers.

%The analyzers that \miga{} currently provides are:
The current implementation of \miga{} provides analyzers to: 
\begin{enumerate}
\item {Analyze added, removed and modified files from a commit},
\item {Analyze commit messages}
\item {Compute lines of code of a version associated to a commit}
\item {Create  Java ASTs for the Java files affected by a commit},
\item {Create  Kotlin ASTs for the Kotlin files affected by a commit},
\item {Compute the differences introduced by a commit at the AST level},
\item {Detect and analyze commits that migrate code}.
%\item {Kotlin AST diff} (as explained in Section \ref{}),
%\item {Features extractor from Diff\inred{mention?}}
%\item {\inred{Pattern matching from Kotlin changes}},%AST diff
%\item {Pattern matching from Java changes (as explained in Section \ref{})}
\end{enumerate}

%\inred{in the algorithm to put the diff algo as input}
Finally, once \miga{} processes all the commits from the input, it processes the results produced by each analyzer from each commit, with the goal of creating the summary of the results. 
The Output Processor are the components that takes the output produced by one or more analyzers and produces a new output. 
For example, an output processor  counts the number of commits that have both modifications in both Java and Kotlin files. Another output processor exports all the results to JSON format.

All the analyzers previously presented have been used in this paper to study the applications that are migrated to one language to another.

%In particular, \miga{} 
%it computes the intra-language change patterns (i.e., the patterns that express changes from one language) and the inter-languages change patterns (i.e., the patterns that express changes happening in two or more program languages).

\miga{} can be easily extended using the extension mechanism provided by the underlying platform (Coming \cite{coming2019}):
new analyzers and output processors can be easily added.\footnote{Extension points of Coming: \url{https://github.com/SpoonLabs/coming/blob/master/docs/extension_points.md}}


\subsection{Analyzers from \miga{} for studying code migration}
\label{sec:miga:migrationanalyzers}

In this section we detail the functionality provided by \miga{} for studying the migration of applications.
Note that this functionality is not fully provided by the core of Coming.



\subsubsection{Analyzing Files from Commit}
\label{sec:files_commit}

\newcommand{\langsrc}{\new{$Lang\_Src$}}
\newcommand{\langdst}{\new{$Lang\_Dst$}}

\miga{} extends Coming by adding the functionality for analyzing commits written in more than one language. (Note that Coming only focuses on Java code).
This functionality is required for studying the migration of applications.

A commit can modify a version of an application in different ways.
For instance, if we consider one applications having two programming languages, one called \langsrc{} (Source) and another \langdst{} (Destination), there are 6 different \emph{actions}  done by a commit:

\newcommand{\Caddsrc}{\new{$Commit\_add\_src$}}
\newcommand{\Cadddst}{\new{$Commit\_add\_dst$}}
\newcommand{\Cremsrc}{\new{$Commit\_rem\_src$}}
\newcommand{\Cremdst}{\new{$Commit\_rem\_dst$}}
\newcommand{\Cupsrc}{\new{$Commit\_up\_src$}}
\newcommand{\Cupdst}{\new{$Commit\_up\_dst$}}


\begin{enumerate}
    \item \Caddsrc: Add new \langsrc{} file,
    \item \Cadddst{}: Add new \langdst{} file,
     \item \Cremsrc{}: Remove \langsrc{} file, 
    \item \Cremdst{}: Remove \langdst{} file, 
    \item \Cupsrc{}: Updates Files in language \langsrc,
    \item \Cupdst{}: Updates Files in language \langdst.
\end{enumerate}

In particular, the current implementation of \miga{} is able to work with two program languages: Java and Kotlin. In case of analyzing the migration of Java app to Kotlin, the \langsrc{}  language is Java, and the \langdst{} is Kotlin.

\subsubsection{File-level Migration}
\label{sec:file_migration}

The first analyzer provided by \miga{} is able to detect commits that carry out \emph{File-level Migrations}.
This case represents the migration of code from one file written in one language to another file written in a different language.
According to the actions presented in Section \ref{sec:files_commit}, this migration case happens when a commit Adds and Removes files from different languages: a commit containing action  \Caddsrc{} and \Cremdst{},  or \Cadddst{} and \Cremsrc{}), and the names of the files are the same (excluding the file extension).

\subsubsection{Analyzing Finer-grained Migration (code level)}
\label{sec:fine_grained_migration}

In addition to the file-level migration explained in Section \ref{sec:file_migration}, \miga{} is able to analyze the migration at a fine-grained level, which we named \emph{code-level migration}.
This migration happens when a developers migrates code by, for instance, updating two (or more) existing files written in two different languages. 
This situation corresponds to the cases \Cupsrc{} and \Cupdst{} from Section \ref{sec:files_commit}.
From one of those files, code is removed (e.g., Java code) and in the other, code is added (e.g., Kotlin code).

The current implementation of  \miga{} provides an analyzer that focuses on detecting one particular \emph{code-level} migrations: \emph{methods}.
The goal is to detect migration cases that migrate a particular method written in Java to a new method written in Kotlin. Note that \miga{} is also capable to detect migrations from Kotlin to Java, however, in this paper we focus on the migration Java to Kotlin.

In this paper we focus on method-level migration, even \miga{} also provides the possibility to detect other code-level migrations, such as properties or blocks. 


\paragraph{From file to AST}
\label{sec:ast_parser}

The  Finer-grained Migration analyzer works at the AST level. 
Thus, \miga{} converts every code file affected by a commit to an AST (Abstract Syntax Tree) and stores them for further analysis such as fine-grained differencing.

If a commit modifies a file $f$, \miga{} creates the AST for the version of the file \emph{before}  the modification (i.e., the previous version of the file), and another AST for the file with the changes introduced by the commit.
Then, \miga{} stores that pairs of ASTs.

\miga{} provides code source parser for different program languages. In this work, we focus on two: one for parsing Java code, another for parsing Kotlin code.


\paragraph{Computing AST diff}
\label{sec:ast_diff}


%\miga{} 
MigA focuses on studying the changes that happen in files that are modified  by a commit (cases from  \Cupsrc{} and \Cupdst{}).
Thus, for each  commit $c$ that updates a file $f$, \miga{} computes the differences between the AST of the previous version of the file $f$ (i.e., the version without having the change introduced by $c$) and the current version of  $f$ (i.e., the version with the changes introduced by $c$).
For computing the AST diff, \miga{} uses GumTree algorithm \cite{Falleri:2014:FAS}.
The output of that comparison is a list of AST changes, where each change is an operation (GumTree has four: Insert, Remove, Update and Move) over an AST node.
%%%



\paragraph{Detection of code-level migration}
\label{sec:method_migration}

As difference from the migration case mentioned in Section \ref{sec:file_migration}, the code-level migration is at a fine-grained level: a portion of a file (e.g., a method) is migrated rather than the complete file.

For detecting code-level migration in one commit $c$, \miga{} takes as input the output of the AST diff algorithm explained in Section \ref{sec:ast_diff}.
There, \miga{} computes the AST diff for each updated file $c$.
Then, \miga{} checks the extension of the updated files to verify that the commits affects code written in more than one language. 
If the commit only affects code written in one language, the code-level migration does not take place.
If the commit affects two or more files, i.e., updates files from different languages, 
then \miga{} computes the $diff$ for each file and its precedent version. 
Thus,  each $diff$ is related to a particular language.
 
Finally, 
\miga{} finds for INSERT operations that affect \emph{methods} in one diff (e.g., a diff from Kotlin files), *and* DELETE operations that also affect methods in the other diff (e.g., a diff from Java files).
If \miga{} found those pairs of operations, it stores them for a subsequent analysis.
Note that, by default, \miga{} does not match  the method names, even it is possible to do it.

%After that, \miga{} checks the method names of each pair of INSERT - DELETE operation.
%if the names matches, it is a \emph{perfect} migration.

%%name analysis.

\subsection{Detection of other types of migrations}

\miga{} is able to detect other types of migrations.
One that combines the two previous strategies consist on finding commits that do both:
\begin{inparaenum}[\it a) ]
\item adds a \langdst{} file, and
\item updates a \langsrc{} file by removing a method.
\end{inparaenum}
This case contemplates that a developer removes a method from a file written in one language \langsrc{} (e.g., Java) and adds, at the same time, a new file written in \langdst{} language (e.g., Kotlin) containing the new implementation of the removed method.

Our goal is that other researcher uses the analyzers provided by \miga{} for creating new strategies for detecting migrations of code.


%%%%%%%%%



\begin{comment}


\subsection{Discovering Code Change Patterns}
\label{sec:change_patterns}


\subsubsection{Pattern detection algorithm}
The goal of \miga{} is to detect the most frequent code changes that happen on this scenario (i.e., when files are updated).\inred{UPDATE}
For that, in this paper we propose a new algorithm, called \algoname{}, for  change pattern detection which we introduce below in the next Section \ref{sec:pattern_detection}.
%Using this algorithm, called \algoname{}, we are able to capture, the patterns 
%We use this algorithm for detecting two kind of patterns:
%1) frequent changes that happens in one language (be Src or Dest),
%2) patterns of changes between two or more languages.


%The goal of \migga{} is to extract knowledge about the migration.
%In particular, 
\miga{} focuses on extracting two types of code change patterns:
\begin{inparaenum}
\item intra-languages change patterns which capture frequent changes produced in one particular language.
\item inter-languages change pattern (\emph{migration patterns}) which capture frequent changes involving two or more languages.
\end{inparaenum}
Moreover, \miga{} classifies commits according to a migration taxonomy.
%


\subsubsection{Intra-language change pattern}

\miga{} reads those inputs for each project analyzed and, to compute the most frequent patterns, applies a procedure similar to that one explained in Section \ref{}.
It first creates an empty Pattern pool.
Then, it gradually reads each pattern and compare it with those already in the pool using the algorithm presented in \ref{}.
if the pattern already exists ($pt$), it associates all instances from project into ($pt$). Otherwise it add it to the pool.

\subsubsection{Inter-language change pattern}

Similar to \ref{}. the difference is that a pattern has two components: one represents the Java pattern, the other one the Kotlin pattern.
When \miga{} matches two patterns, it applies two times the algorithms \ref{}: one for the Java part, the other for the Kotlin.
\miga will consider a pattern matching if the similarity of \emph{both} parts are larger than a threshold $txxxx$.


\subsection{Analyzing commit message}
\label{sec:commit message}

Previously in this section, we have focused on studying the files affected by the commit for detecting migration cases.
The  \emph{commit message} is written by the developers with the propose of explaining what the commit has, the main changes introduced by it, etc.
\miga{} also is able to study the \emph{commit message} for detecting commits that migrate code.
For that, \miga{} filters commits which message includes keywords such as `migration', `converted', etc.

\end{comment}

%%commit message keywords: converted, automated


%%%%%%%%%%%%%%%%%%%%%
%%%
%%%%%%%

\section{Methodology}
\label{sec:methodology}


%\newcommand{\rqevolution}{{RQ 1: How do mobile apps having Kotlin code evolve during their history?
%}}

\newcommand{\rqappsmigrated}{{RQ 1: How many Android applications have been fully migrated to Kotlin?
}}


\newcommand{\rqwhymig}{{RQ 2: 
%Why did developers migrate?
For which reasons have developers migrated their Android applications from Java to Kotlin?
}} %%


\newcommand{\rqmigrationdone}{{
%Previous
%RQ2: How the migration from Java to Kotlin is done?
%\new{What are the strategies of migration code?}
\new{RQ 3: How did developers migrate from Java to Kotlin?}
}}


\newcommand{\rqproportion}{{RQ 3: Are the mobile apps which latest versions have both Java and Kotlin in  process of being migrated?}}
%%How does not migrated 



==> Migration Kotlin-Java_4rev/old-content/others-old.tex <==
%files after the introduction of Dst
\begin{comment}
\begin{enumerate}
    \item Add Kotlin file Remove Java file
    \item Add Java file Remove Remove file

Add Java File

    \item Updates Changes in Java (language Src)
    \item Updates Changes in Kotlin (language Dest)
    
    
\end{enumerate}
\end{comment}

==> Migration Kotlin-Java_4rev/old-content/removed_Methodology_TSE.tex <==

\section{Methodology}
\label{sec:methodology}

To respond the research questions, in this section we first present a tool, named \miga{}, that analyzes repositories of applications.
Then, we explain how we used it to respond the research questions.
Finally, we present the methodology we applied to carry out a survey which consisted on interviews with developers that migrated code to Kotlin.


\subsection{Methodology applied for analyzing commits}

To detect commits that migrate code, we build a tool called \miga{}.
%
It allows researchers to study the evolution of software applications i.e., the changes done over an application along its history.
In particular, \miga{} focuses on analyzing applications that, during their evolution, have been migrated to one programming language to another (or others).
%
In this section we present \miga{} and we describe how we process its output for responding the research questions.
%
\label{sec:migaframework}

\subsubsection
{Architecture and Implementation of \miga{}}
\label{sec:architecture}


\miga{} is built on top of Coming \cite{coming2019}, a framework for studying the evolution of applications.
\miga{} frameworks takes as input the location of a GIT repository on disk. 
It navigates each commit in chronological order, starting from the oldest one.
\miga{} extends Coming with new analyzers for studying the migration of applications. 
In particular, \miga{}: 
\begin{inparaenum}[\it a)]
\item {Analyzes added, removed and modified files from a commit},
\item {Analyzes commit messages},
\item {Compute lines of code of a version associated to a commit},
\item {Creates  Java ASTs for the Java files affected by a commit},
\item {Creates  Kotlin ASTs for the Kotlin files affected by a commit},
\item {Computes the differences introduced by a commit at the AST level},
\item {Detects commits that migrate code}.
As output, \miga{} generates a JSON file containing, for each commit, the information produced by each aforementioned analyzers.
%\item {Features extractor from Diff\inred{mention?}}
%\item {\inred{Pattern matching from Kotlin changes}},%AST diff
%\item {Pattern matching from Java changes (as explained in Section \ref{})}
\end{inparaenum}


\subsubsection{Lines of code per language}
For responding the first research question (RQ1), we analyze the output of \miga{} containing  per each commits $C$:
\begin{inparaenum}[\it a)]
\item the lines of source code (sLOC), and 
\item number of files 
\end{inparaenum} for each program language used on the version associated to $C$.


\subsubsection{Migration interval}
\label{sec:method:migrationinterval}

For responding the second research question (RQ2), 
we detect from the \miga's output, for each application:
\begin{inparaenum}[\it a)]
\item the first commit that uses Kotlin code, and
\item the last that  uses Java code.
\end{inparaenum} 
We call \emph{migration interval} to the portion of the application's history between those two commits.
%
The \emph{migration interval length} of a migrated application is the number of commits that happen between the two previously retrieved commits.
%
%$Migration\; Interval \; Length \;(MIL)  = Index_{last\_Java\_commit} - Index_{first\_Kotlin\_commit}$, 
%where $Index_{c}$ is the  $index$  of  commit $c$ from a list of commits chronologically sorted.

We further compute the \emph{proportion} of the migration interval w.r.t all the commits from the history of one application by dividing the length of the interval by the total number of commits.


\subsubsection{Detecting commits that migrate code}
\label{sec:commit_migration}

Moreover, also for responding research question 2, we implemented on \miga{} the detection of three types of commits that migrate code.
Those are:

\paragraph{File-level Migration}
\label{sec:file_migration}
\miga{} is able to detect \emph{File-level Migrations} commits.
They are commits that migrate code
by removing one Java file and adding a new Kotlin file.
\miga{} checks that  the names of those files are the same (excluding the file extension).

\paragraph{Finer-grained code level migration}
\label{sec:fine_grained_migration}
\label{sec:method_migration}

\miga{} is able to detect  commits that migrate code at a fine-grained level, which we named \emph{code-level migration}.
This type of migration happens when a developer migrates code by updating two (or more) existing files written in two different languages: 
Java code is removed and Kotlin code is added.
%
The current implementation of  \miga{}  is able of detecting on \emph{methods} level migrations.\footnote{
Even it is not covered in this paper, \miga{} can detect other code-level migrations, such as properties or blocks.}

For detecting method-level migration commits, \miga{} applies the following steps on each commit:
\begin{inparaenum}[\it a)]
\item verifies that 1 or more Java files \emph{and} 1 or more Kotlin files are updated by a commit $c$;
\item for each updated Java or Kotlin file $f$, \miga{} creates an AST (Abstract Syntax Tree) from $f$ and another from the previous version of $f$, i.e. $f_p$;
\item \miga{} computes the differences between the ASTs obtained from $f$ and  $f_p$, using GumTree algorithm \cite{Falleri:2014:FAS}. The output is a list of AST changes, where each change is an operation (Insert, Remove, Update and Move) done over an AST node;
\item \miga{} finds for INSERT operations that affect \emph{methods} in the $diff$ obtained from comparing Kotlin files, and DELETE operations that also affect methods in the other $diff$ obtained from comparing Java files.\footnote{By default, \miga{} does not match the method names, even it is possible to apply string matching heuristics.}
\end{inparaenum}

\paragraph{Update-Insert Migration}
\label{sec:update_insert_migration}
%
%
\miga{} can detect commits that removes a piece of code (e.g., method) from a file written in Java and, at the same time, adds a new file written written in Kotlin.
The implementation of this detector is based on the two previously described cases.

\paragraph{Other types of migrations}
Beyond those three types of commits that migrate code, there could be other that also migrate code.
%
We leave the discover and characterization of such types, and the detection of commit corresponding to the emerging types for future work. In Section \ref{sec:discussion} we discuss some future directions for discovering them.


\begin{comment}
\subsubsection{Commit composition}
\label{sec:method:proportion}
\todo{re-do?}
Moreover, in RQ 1, we study the composition of commits according to the program languages they affect.
The classify commits in 4 types \todo{weird sentence}: 
\begin{inparaenum}[\it 1)]
\item Pure-Java (commits that affect Java code but not Kotlin),
\item Pure-Kotlin (commits that affect Kotlin code but not Java),
\item Mix (commits that affects both Java and Kotlin code),
\item Other (commits that do not affect nether Java nor Kotlin code, e.g., XML files).
\end{inparaenum}
%By affected we mean that a commit adds, modifies or removes one or more files.
\todo{To me moved to Migration study and to compute it after Kotlin is introduced}
\end{comment}



\subsubsection{Amount and proportion of Kotlin code}
\label{sec:method:amountkotlin}

For responding the first  and fourth research questions, 
\miga{} computes, for each application $a$ and for each commit $c$, the number of Java and Kotlin lines of codes (sLOC) of the version of $a$ given by $c$.
It also computes the proportion of Kotlin code by dividing the sLOC of Kotlin per the total sLOC (i.e., Java sLOC + Kotlin sLOC).
Then, for each application, 
we compute the variation of both amount of sLOC and proportion between the latest commit done and an older commit.
In particular, we consider two older commits:
\begin{inparaenum}[\it 1)]
\item the \emph{first commit} that introduces Kotlin,  and
\item a ``\emph{recent commit}'', which corresponds to the commit done just before the latest 10\% of all commits.
\end{inparaenum}
For example, if one application has 110 commits and Kotlin was introduced in the commit \#10, we compare the amount/proportion of Kotlin code between the commit \#110 (latest) and: 
\begin{inparaenum}[\it a)]
\item the \emph{first commit}: \#10 (first Kotlin commit),
\item  the \emph{recent commit}: \#100 (beginning of the last 10\%  from all the Kotlin commits).
\end{inparaenum}


\subsection{Methodology applied for executing the survey}
\label{sec:methodology:survey}

For responding research questions 3, 4 and 5, we conducted a survey with developers.
In this section, we detail the characteristics and initial results of this survey.

\subsubsection{Survey purpose}

We carry out a survey with the main goal of collecting information about the migration of Java code to Kotlin in the context of Android development.
Our survey is explanatory~\cite{experimentationSE2012}: we try to explain why developers migrated their applications. 
The survey follows the format of interviews via email and aims at gathering both qualitative and quantitative data.

We initially asked developers a single question via email:
\quotes{Why did you migrate code from Java to Kotlin?}.
Then, once we received an answer from them, we further asked new questions according to their replies.
For example: 
\begin{inparaenum}[\it a)]
\item \quotes{Did you use the auto-converter code tool provided by the IDE?},
\item \quotes{Which was the criterion (if any) to choose those classes to migrate?},
\item \quotes{Your project still has Java code, Why has it not been completely migrated yet?}.
\end{inparaenum}

We choose this format of exploratory survey, composed of an initial question and followed by a loosely structured questionnaire, to follow the recommendations given by~\cite{experimentationSE2012}, which indicates that letting interviewers handle the questionnaire instead of the respondents themselves offers a number of advantage, such as observing the answers and ask questions according to the observation. 

\subsubsection{Survey setup}

\miga{} framework is able to return \emph{all} commits that migrate Java code to Kotlin from our dataset of Android applications (Section \ref{sec:dataset}).
From each commit, we retrieved the name 
and the email address of the developer that made the commit.
That information is the repository history (GIT).
Then, we sent to each developer that made a migration a personalised email that mentioned that we have analyzed the code of her/his application (mentioning the app name) and we have detected that she/he has write a commit (or several) that migrated code from Java to Kotlin. 

\subsection{Survey results}

We could successfully send, in total, 249 emails.\footnote{Some emails could not be successfully delivered (e.g., those from development companies which employers do not work there any more).}
We got the response from \nremailreplies{} developers, all them from different projects.
This means that $\sim$30\% of developers that migrated Java code to Kotlin in applications from the dataset we study (Section \ref{sec:dataset}) have participated in our survey.
Those interviewed developers are from, at least, 17 countries.
%Even the goal of this paper is not to present a demography study of developers (we did not ask about their country, experience, current status, etc), 
%by analyzing their profiles and email addresses we obtained that those developers are from, at least, 17 different countries. 
%Germany, United States, Korea, Japan, China, India, Brazil, Portugal, Czech Republic,  Spain, France, Canada, Portugal, Italy, Switzerland, Netherlands, among others.
Note that not all participants replied \emph{all} the questions we asked them.
Along this paper we \emph{literally} present answers from developers, without doing any kind of modification (e.g., typos or grammar issues).

Once we collected all answers, 
we detailed analyzed each interview (i.e., a thread of emails with answers and responses) to collect all valuable information for responding research questions 3 (why they migrated), 4 (why not fully migrated) and 5 (advises).


\subsection{Dataset of Android Applications studied}
\label{sec:dataset}
Given Google has officially adopted Kotlin as programming language for Android, 
our goal is to study the migration from Java to Kotlin of Android applications.
For this reason, we analyze Android applications from the FAMAZOA dataset \cite{GoisMateus2019}, which contains 374 Android  with at least one commit done in Kotlin.
FAMAZOA dataset was built by combining open-source applications mined from different sources such as F-Droid\footnote{F-Droid: dataset of open-source Android applications \url{https://f-droid.org}} repository and Android Time Machine \cite{Geiger2018:data}.


%%%%%%%

==> Migration Kotlin-Java_4rev/old-content/removed_TSER1.tex <==
%%%% From discussion part

\subsection{Future Uses of \miga{}}

\miga{} can be used by other researchers to study the evolution of the migration activity of applications written in other program languages.
\miga{} can be extended using the extension mechanism provided by the underlying platform (Coming \cite{coming2019}).
%\footnote{Extension points: \url{https://github.com/SpoonLabs/coming/blob/master/docs/extension_points.md}}
A researcher can add: 
\begin{inparaenum}[\it a)]
\item new programming language parsers (currently \miga{} provides parsers for Java and Kotlin, and
\item new analyzers (in addition to those presented in Section \ref{sec:architecture}).
%\item and output processors.
\end{inparaenum}

One of the future direction we plan to study is the detection of migration change patterns.
This will allow us to detect commits that migrates code which do not fall into the three types of migration commits we defined in Section \ref{sec:commit_migration}.
For that, we define \emph{inter-languages change pattern} as a pattern which captures frequent changes involving two or more languages.
We aim at detecting
\emph{Inter-language change patterns} that occur on commits that affect both Kotlin and Java files.
We now present an initial experiment in that direction.

\subsubsection{Discovering Inter-language change patterns}
\label{sec:inter-patterns}
We carried out a first experiment for discovering Inter-language change patterns.
We applied frequent itemset (FIS) algorithm \cite{Agrawal:1993:MAR}, in particular Apriori algorithm \cite{Agrawal:1996:FDA},
on commits that update one or more Kotlin files \emph{and} one or mode Java files.
A \emph{frequent itemset} is, given examples that are sets of items and a minimum frequency,  any set of items that occur at least in the minimum number of examples \cite{Toivonen2010}. 
We created an itemset per each commit, where each item is a single AST change.
Each itemset has 1 or more changes on the Java AST \emph{and} 1 or more changes on the Kotlin AST.
As mentioned in Section \ref{sec:architecture} \miga{} outputs this information per each commit.
%
We applied FIS over the changes extracted from 422 commits that update both Java and Kotlin, those commits come from 33 migrated apps (note that the remaining 53 out of 86 apps from set \emph{\migrapps{}} do not have any commits that updates both Java and Kotlin).

Table \ref{tab:apriori} shows a sample of the most frequent \emph{inter-language change patterns} we found using FIS. 
The first row shows that the 1.6\% of the commits analyzed update a Method Invocation located inside a Java method  \emph{and also} it updates method Invocation located inside in a Kotlin Function.
One frequent item (row 7) corresponds to the method-level migration discussed in Section \ref{sec:res:methodlevelmigration}.
However, beyond that pattern,  most of frequent itemsets do not  remove code.
This can be explained by the fact that, when migrating, developers also need to update the remaining Java code (e.g., to update the references to the migrated code).
%
We leave for future work the research on other pattern detection algorithms.


\subsection{Further characterization of migrations}

One of our goals was to understand which functionality was migrated to Kotlin.
We aimed to respond the question: \quotes{Which functionality was migrated to Kotlin?}.
Most of developers confirmed us that they have started the migration by migrating POJO (Plain Old Java Object) to Kotlin's \emph{Data Classes}.
They all agreed that is a straightforward and simple migration.
However, beyond that finding, due to the diversity and complexity of the answers, we could not develop generalized conclusions about which functionalities.
%
We let this question open for future work.

%%%%%%%%%%%%%%
%% OLD RQ 4
%%****

\subsection{\rqproportion}
\label{sec:rq:proportion}

\begin{figure}
\captionsetup{justification=centering}
    \centering
 \begin{subfigure}[b]{0.15\textwidth}%%0.32
        \includegraphics[width=\textwidth]{lines_Passandroid.pdf}
        \caption{{\scriptsize PassAndroid}: Amount and proportion of Kotlin code increase.}
        \label{fig:linesPassandroid}
    \end{subfigure}
    \begin{subfigure}[b]{0.15\textwidth}
         \includegraphics[width=\textwidth]{lines_Photolinkviewer.pdf}
           \caption{
           %Photolinkviewer App:  Amount of Kotlin and Java code decrease, proportion of Kotlin code also decreases.
           {\scriptsize PhotoLinkViewer}:  Amount and proportion  of Kotlin code decrease.
           }
      \label{fig:linesPhotolinkviewer}
    \end{subfigure}
     \begin{subfigure}[b]{0.15\textwidth}
    \includegraphics[width=\textwidth]{lines_Daycounter.pdf}
        \caption{{\scriptsize DayCounter}: Amount of Kotlin code increase, but the proportion decreased. % due to the reintroduction of Java code.
        }
    \label{fig:linesDaycounter}
    \end{subfigure}

    \caption{Evolution of 3 apps not yet fully migrated. Axis X corresponds to commits, axis Y to sLOC.}
 
    \label{fig:evolutions_trends}
\end{figure}



\begin{table}[t]
\centering
\label{tab:summarybothlang}
 \begin{tabular}{|c |  r r r |r|  } \hline
Latest $c$ & Prop $\uparrow$ & Prop $\downarrow$&  Prop = & Total\\
 \cline{2-5}
 
versus& \multicolumn{4}{c|}{Amount Kotlin  $\uparrow$} \\
\cline{2-5}

\hline
 First  $c$  & 163 (76.17\%) & 35 (16.36\%) & 0 (0.00\%) & 198 (92.52\%)  \\
%Last  50\% & 148 (69.16\%) & 32 (14.95\%) & 0 (0.00\%) & 180 (84.12\%)  \\
%Last 30\%& 149 (69.63\%) & 22 (10.28\%) & 0 (0.00\%) & 171 (79.91\%)  \\
%Last  20\% & 148 (69.16\%) & 15 (7.01\%) & 0 (0.00\%) & 163 (76.17\%)  \\
Recent $c$& 139 (64.95\%) & 13 (6.07\%) & 0 (0.00\%) & 152 (71.03\%)  \\
\hline
\hline
&  \multicolumn{4}{c|}{Amount Kotlin  $\downarrow$}\\
\cline{2-5}
%& Prop $\uparrow$ & Prop $\downarrow$&  Prop = & Total\\
\hline
 First $c$ & 1 (0.47\%) & 4 (1.87\%) & 0 (0.00\%) & 5 (2.34\%)  \\
%Last  50\% & 5 (2.34\%) & 5 (2.34\%) & 0 (0.00\%) & 10 (4.67\%)  \\
%Last  30\% & 5 (2.34\%) & 12 (5.61\%) & 0 (0.00\%) & 17 (7.94\%)  \\
%Last   20\% & 3 (1.40\%) & 17 (7.94\%) & 0 (0.00\%) & 20 (9.35\%)  \\
Recent $c$& 4 (1.87\%) & 22 (10.28\%) & 0 (0.00\%) & 26 (12.15\%)  \\
\hline
\hline
 &  \multicolumn{4}{c|}{Amount Kotlin =}  \\
\cline{2-5}
%& Prop $\uparrow$ & Prop $\downarrow$&  Prop = & Total\\
\hline
 First $c$ & 0 (0.00\%) & 6 (2.80\%) & 5 (2.34\%) & 11 (5.14\%)  \\
%Last    50\% & 4 (1.87\%) & 12 (5.61\%) & 8 (3.74\%) & 24 (11.21\%)  \\
%Last    30\% & 4 (1.87\%) & 13 (6.07\%) & 9 (4.21\%) & 26 (12.15\%)  \\
%Last    20\% & 4 (1.87\%) & 15 (7.01\%) & 12 (5.61\%) & 31 (14.49\%)  \\
Recent $c$& 5 (2.34\%) & 16 (7.48\%) & 15 (7.01\%) & 36 (16.82\%)  \\
 \hline
 \end{tabular}
\caption{The table groups the apps that increase ($\uparrow$), decrease ($\downarrow$) or equality ($=$):
{\it a)} the amount of Kotlin code, 
{\it b)} the proportion of Kotlin code.
For each application, we made two comparisons:
{\it 1)} the latest commit and the first commit that  introduces Kotlin, 
{\it 2)} the latest commit and a \emph{recent} commit with Kotlin. (The letter $c$ means `commit').
}

\label{tab:result}
\end{table}

We now study the evolution of the applications that have not been completely migrated to Kotlin yet (i.e., set  \emph{\colanguage}).
As reported in Section \ref{sec:res:langusedhistory}, the number of such applications is 214 (out of 374). 

We response this research question via two studies.
First, we present a quantitative study based on the evolution of the amount of code computed using \miga.
Then, we present a qualitative study based on the interviews we made to developers.


\subsubsection{Evolution of Amount of Java and Kotlin Code}
Table \ref{tab:result}  shows the results: each cell corresponds to the number of applications having the amount and proportion of Kotlin code increased~($\uparrow$), decreased~($\downarrow$) and equals~($=$) w.r.t. a previous commit done in the past.
We now discuss three cases of code evolution.

\todo{move to partially}

\paragraph{Case 1: Amount of Kotlin Code Increase}
\label{sec:amountincrease}

Let's focus on the first section of the Table \ref{tab:result} (Amount  Kotlin~$\uparrow$).
For the 92.52\% of the applications, the latest commits has more Kotlin code that the first commit that introduced code.
Figure \ref{fig:linesPassandroid}  shows the evolution of the amount of Java and Koltin code from one of those apps.
However, the number of apps that have more Kotlin code in the latest w.r.t a \emph{recent commit} (see definition in \ref{sec:method:amountkotlin}) is lower:  71\%.
Figure \ref{fig:linesPhotolinkviewer} shows the evolution of code from one apps.

Moreover, the 76.17\% of the apps (163 apps) have a larger proportion of code w.r.t the first version.
The percentage is lower when we compare the proportion of the last commit and the \emph{recent} commit: 64.95\% (139 apps).
We believe that those applications are potentially in process of being migrated. 
That situation  could eventually lead into the total migration of the Java code to Kotlin.
On the contrary, for 16.36\% of the apps (35 apps) proportion of Kotlin code has decreased (column Prop $\downarrow$).
This means that those apps have received more Java code than Kotlin.
Figure \ref{fig:linesDaycounter} shows one of those apps: after a total migration to Kotlin, Java code was reintroduced.


\paragraph{Case 2: Amount of Kotlin code decreases}
\label{sec:amountdecreate}
The second section from Table \ref{tab:result} (Amount Kotlin $\downarrow$) shows that few apps (5, i.e. 2.34\%) have less Kotlin code than the initial commit with Kotlin.
However, the 12\% of the apps (26) have less code than their \emph{recent commit}.
We suspect that this reduction is consequence of code refactoring.


\paragraph{Case 3: Amount of Kotlin code remains constant}
\label{sec:amountequals}
Last section from Table \ref{tab:result} (Amount Kotlin~$=$) shows that the 16.82\% of the applications (36) have the same amount of Kotlin code w.r.t the \emph{recent commit} (last row). 
For the 7.48\% (column 3, Prop~$\downarrow$) of them, new Java code is introduced in the latest commits, guiding the evolution of such apps. 


\begin{tcolorbox}
%The 76.17\% 
The 64.95\% of the applications having both Kotlin and Java in their latest version evolves increasing both the amount and the proportion of Kotlin code. 
We conjecture that, if those applications continue evolving following that evolution trend, in the near future they could be completely migrated to Kotlin.
\end{tcolorbox}

%%%%%%%%%%% END OLD RQ 4 Mining analysis


%%% OLD RQ 1 and 2********


\subsection{\rqappsmigrated{}}
\todo{fully or partially}


\todo{Two subsection: Fully migrated and partially migrated, with the content of RQ4}
To respond this research question, we first analyze the languages used:
\begin{inparaenum}[\it a)]
\item at the beginning of the development, 
\item during the development of an application, and finally
\item  in the last commit.
\end{inparaenum}
%
The fully migrated applications detected in this research question, as well those not fully migrated, will be studied in the next research questions.

\subsubsection{Initial Programming Language}
\label{sec:res:initiallang}


We analyze 374 Android applications from \dataset{} dataset.
By construction, all applications from there have, at least, one file with Kotlin code and, eventually, one file with Java code.

Table \ref{tab:lang} presents the results. 
In total, 65  apps were initially written only using Kotlin code.\footnote{\label{lab:javatest}
From the 65 apps, 21 have Java code corresponding to test cases  named `ExampleUnitTest.java' and `ApplicationTest.java' automatically generated by IDEs such as Android Studio when a project is created. Those tests have not been modified after the creation. For this reason, we ignore them.}
%One example of such applications is Kingfish, which initial commit\footnote{Initial commit of app Kingfish: 5c448ed6a2805a23b002c8e5e156fb43ca1d3cf7.} has a Kotlin file and two automatically generated Java test files named `ExampleUnitTest.java' and  `ApplicationTest.java'.  Note that developers from those projects did not modify those tests during the evolution of the apps. 
%
From the remaining 309 apps, 269 started being developed just using Java code (i.e., Java code was used before  Kotlin code),
and 40 apps have been developed using both Kotlin and Java since the first version pushed to their respective version control systems.


\begin{table}[t]
\centering
 \begin{tabular}{|l||  r | r |   } 
 \hline
Language& \multicolumn{2}{c|}{Number  Applications having:} \\
\cline{2-3}
& Initial  version  & Latest version  \\
\hline
Java &269&4\\
\hline
Kotlin &65&156\\%%60+96
\hline
Both &40&214\\
\hline
\hline
Total& \multicolumn{2}{c|}{374}\\
 \hline
 \end{tabular}
\caption{Number of apps having Java and Kotlin version in their first and last versions.\todo{remove}}
\label{tab:lang}
\end{table}

\subsubsection{Languages used along the history}
\label{sec:res:langusedhistory}

Our dataset has in total 60 apps (16\%) completely written in Kotlin along their history.\footnote{
Between the 60 apps, there are 16 that introduce (but not evolve) the automatically generated tests mentioned in footnote \ref{lab:javatest}.}
%
The rest, 314 apps  (84\%), evolves by adding and modifying Kotlin and Java code (at the same or different time).
%%%Long version commented
\begin{comment}

In total, 44 apps have been developed using just Kotlin code along their complete history, without having a single line of Java code. 
Moreover, we found that 16 additional apps that were written in Kotlin and have one or more commits including the mentioned  test files automatically written in Java (Section \ref{sec:res:initiallang}) and no more Java code in any commit from their history.\footnote{In Section \ref{sec:res:initiallang} we report 21 apps that introduce automated generated tests in their first commits, and in Section \ref{sec:res:langusedhistory}  we report 16 apps that  introduce those tests in any part of their history, not only at the beginning. This means that 5 apps (21 - 16) add one or more Java files (different from those testing files) during their evolution.} 
Consequently, by ignoring such files and considering those apps as Pure Kotlin, our dataset has in total 60 (16\%) apps completely written in Kotlin.
%
The rest, 314 apps  (84\%) evolve by adding and modifying Kotlin and Java code (at the same or different time).
\end{comment}

\newcommand{\migrapps}{{Migrated-Apps-j2k}}
\newcommand{\colanguage}{{Mix-Java-Kotlin Apps}}

\subsubsection{Languages used in the last version}
\label{sec:res:langusedlastversion}

We now focus on the remaining 314 apps (i.e., 374 - 60) which have Java and, eventually, Kotlin.
%
214 apps have both Kotlin and Java in the latest commit. 
Those apps form the set named \emph{\colanguage{}}.
%
%
Now, let's inspect the remaining 100 apps (314 - 214).
In this paper we are particularly interested in 86 of them, which have been initially written exclusively on Java and \emph{fully} migrated to Kotlin. Those apps from the set named \emph{\migrapps}.

We now describe the other 14 apps (100 - 86), which we do not study in this paper.
First, there are 10 apps that have  initial commits written in Koltin,  and Java code was introduced and subsequently removed.
\begin{comment}
\begin{inparaenum}[\it a)]
\item  5 apps have been initially written using both Kotlin and Java.
\item 5 apps have only Kotlin code in their initial version, and Java code was introduced and subsequently removed.
\end{inparaenum}
\end{comment}
Then, the remaining 4 applications had Kotlin code but it was removed, remaining only Java code in their latest versions.
\begin{comment}
%({Material-flashlight})
For one of them, their developers have started written it in Kotlin and, at the middle of its history, the developers completely migrated to Java.
The others 3 app have been initially developed in Java, then the developers added some functionalities on Kotlin, which were finally removed, remaining, again, only Java code.
\end{comment}
We interviewed one developer that introduced Kotlin on one of those apps.
He told us: 
\quotes{I tried to migrate [...] but other contributors just find it complicated to incorporate two languages style in a single project and, eventually reverted the project to some time before}.


\begin{tcolorbox}
86 Android applications (out of 314) were completely migrated from Java to Kotlin.
Then, 
214 apps were initially written in Java and they have been partially migrated.
\end{tcolorbox}

%%%Removed, not interesting here%%
\begin{comment}
\subsubsection{Moment of First use of Kotlin}
\label{sec:res:kotlinfirstintroduction}


\begin{figure}[t]
\centering
%\begin{subfigure}
 \includegraphics[scale=0.5]{histogram_introduction_kotlin_percentage_374.pdf}
  \caption{Distribution of Introduction moments of  Kotlin code for all applications (374). Zero value means the beginning of the history, 1 means the end. Consequently, the histogram shows that  more than 110 apps have an introduction moment near to zero, which means that Kotlin is used for a first time at the beginning of the project history.}
 \label{fig:hist_kotlin_intro_all}
%\end{subfigure}
\end{figure}

Histogram \ref{fig:hist_kotlin_intro_all} shows the distribution of the \emph{Introduction moment}  of Kotlin code (as explained in Section \ref{sec:method:intromoment}).
%The \emph{introduction moment} is  measure that divides the commit number (following a chronologically order) that introduces Kotlin for the first time into an app $A$   by the total number of commits from $A$.
%
The mean and the median are both ~0.40, which means that Kotlin is introduced, on average, after the first 40 \% of the commits of the application.
%For X applications the introduction  moment  is 0, which means that Kotlin is used from scratch.
We found that 62  apps have a later introduction greater than 0.8, which mean that Kotlin was introduced at the end of the application history. 

%%%Removed, not interesting here%%
\end{comment}


%'project': 'Voice', 'range': 2017,


%allInitsKotlin: len: 374 min: 0.0 max: 0.9837745516652434 mean: 0.40154541258002113  median: 0.4047670695908008 standdesv: 0.3387344410657114 
%late introduction  62: ['zandy', 'k-9', 'DnestrCinema', 'DocScan', 'SimpleHTMLTesterAndroid', 'StreetComplete', 'SystemUITuner2', 'insapp-android', 'madrid-pollution-android-app', 'GeoQuake', 'dlt', 'YoNoDesperdicio', 'trolley-tracker-android-client', 'Botanist', 'spaRSS-DecSync', 'Alarmio', 'Screenshot-Sharer', 'MensaUPB', 'GrowTracker-Android', 'uhabits', 'kiwix-android', 'MGit', 'youreawinner', 'FRCAndroidWidget', 'ComputingTutorAndroidApp', 'SimpleBitcoinWidget', 'easysshfs', 'FAST', 'penn-mobile-android', 'Geocaching4Locus', 'SimpleMarkdown', 'Retribution', 'PosTrainer', 'Status', 'CCIP-Android', 'UnitConverterUltimate', 'rectball', 'materialistic', 'PushNotificationTester_App', 'SoundWaves', 'Lawnchair', 'Sofia-Traffic', 'EH17Fahrplan', 'cpustats', 'rxbsuir', 'ShutUp', 'ContractionTimer', 'LocalStorage', 'buntata-app', 'unitconverter-android', 'BibleQuote-for-Android', 'Umweltzone', 'android-app', 'commcare-android', 'NHentai-android', 'KonashiInspectorForAndroid', 'opacclient', 'speedofsound', 'mtmods4android', 'AutoStopRace', 'NCBSinfo', 'Checklist']



%OpenLaunc migrates one component and the rolback.
%sexytopo introduces one file written in Kotlin and then it is removed.


\subsection{\rqmigrationdone}
\label{sec:res:migration}

We now focus on the 86 apps from set  \emph{\migrapps} that started being developed using Java and were subsequently completely migrated to Kotlin.

To respond this research question, 
we do two experiments.
First, we study the \emph{migration intervals} to characterize the duration of the migrations in terms of commits.
%
Then, we analyze commits inside the migration interval to detect those that could have migrated code. 

\subsubsection{Migration Intervals}

\todo{Summarize and move to RQ 1}

Histogram \ref{fig:kotlin_migration_duration} shows the distribution of the length the \emph{migration intervals}\footnote{For ease of reading, we removed from the Histogram \ref{fig:kotlin_migration_duration} two \emph{outliers}: Rocket.Chat.Android which  interval has 1988 commits  and Voice with 2018.}
and Histogram \ref{fig:kotlin_migration_duration_normalized} shows the distribution of  their lengths normalized by the total number of commits from the application.
This normalization has as goal to observe the duration of the migration w.r.t the complete history of one application.
%For example, the interval of the previously mentioned Red app covers the 37\% of its history (i.e., the proportion is 0.37 =  187 / 502, where 502 is the total number of  commits).
%
From them, we identified two main migration strategies. Those are:

\begin{figure}[t]
\captionsetup{justification=centering}
    \centering
 \begin{subfigure}[b]{0.15\textwidth}%0.42
        \includegraphics[width=\textwidth]{lines_Simplebitcoinwidget.pdf}
        %%simple
        \caption{SBitcoinWidget: $mi$ = 1 commit}
        \label{fig:linesSimplebitcoinwidget}
    \end{subfigure}
    \begin{subfigure}[b]{0.15\textwidth}
         \includegraphics[width=\textwidth]{lines_Localstorage.pdf}
           \caption{Localstorage: $mi$ = 4 commits}
      \label{fig:linesLocalstorage}
    \end{subfigure}
    \begin{comment}
     \begin{subfigure}[b]{0.15\textwidth}
 \includegraphics[width=\textwidth]{lines_Uncmorfi.pdf}
  \caption{UNCmorfi: $mi$ =  28   commits \todo{to remove it}}
 \label{fig:lines-UNCmorfi}
    \end{subfigure} 
      \end{comment}
     \begin{subfigure}[b]{0.15\textwidth}
    \includegraphics[width=\textwidth]{lines_Red.pdf}
        \caption{Red: $mi$ = 188   commits}
    \label{fig:linesRed}
    \end{subfigure}
    \caption{Evolution of Kotlin and Java code for 3 applications having  migration intervals  ($mi$) with different lengths. Axis X corresponds to commits, axis Y to sLOC.}
    \label{fig:examples_mig_interval}
\end{figure}

\begin{figure}[t]

\begin{subfigure}{0.48\linewidth}
 \includegraphics[scale=0.3]{histogram_range_84.pdf}
  \caption{Lengths of Migration Intervals (in number of commits)}
 \label{fig:kotlin_migration_duration}
\end{subfigure}
\hfil
%\begin{figure}[t!]
\begin{subfigure}{0.48\linewidth}
 \includegraphics[scale=0.3]{histogram_range_Percentage_84.pdf}
  \caption{Lengths of Migration Intervals divided by number of commits.\todo{remove/appendix}}
 \label{fig:kotlin_migration_duration_normalized}
\end{subfigure}
\caption{Distribution of the migration interval  lengths corresponding to the 86 apps from set  \emph{\migrapps}.}
\label{fig:kotlin_migration_duration_main}
\end{figure}


%rangeZero 29: ['SimpleBitcoinWidget', '2chmatome', 'PosTrainer', 'JanYoShare', 'FRCAndroidWidget', 'KonashiInspectorForAndroid', 'NCBSinfo', 'kmn_bot-tool', 'SimpleHTMLTesterAndroid', 'easysshfs', 'VoiceMessageBoard', 'Android-SearchView-Demo', 'home-button', 'stew', 'Status-Bar-Tachometer', 'vanilla-music-metadata-fetch', 'AnkiEditor', 'Stratum0Widget', 'MockAppDemo', 'Screenshot-Sharer', 'SunWidget', 'SystemUITunerRedesign', 'speedofsound', 'Simple-Thank-You', 'baresip-studio', 'Simple-Flashlight', 'SELinuxModeChanger', 'tincapp', 'youreawinner']

\paragraph{One-Step migration}
%%33.7\%

%% Clarification: 31 are the 29 with 1 + 2 apps with negative 33.7\%
In total, 31  projects (out of 86 apps from \emph{\migrapps}, that is, the 36\%)  have migration interval lengths equals to 1, which means that they were migrated in \emph{exactly} one commit.
Those commits remove all Java files and introduce the Kotlin code. 
One of those applications is `SimpleBitcoinWidget', which code  evolution is presented in Figure \ref{fig:linesSimplebitcoinwidget}. 
%: in one commit the complete Java code is replaced by Kotlin code.
%\footnote{Commit id: 417e2e86c8d7c72b77443b273b36b885276d285f from app SimpleBitcoinWidget.} 

Eight developers that replied to our interview request had migrated their apps in one single commits. 
Half of them confirmed us that they migrated the code using the converter tool provided by the IDE Android Studio.
%
%The other ones migrated \emph{by hand}.
%One developer told us about that: \quotes{The app is not a large project so migrating from Java was not a big deal}.

%Another one told us that, beyond migrating its app in One-step: \quotes{I converted the entire project class by class, over the course of weeks}.


%project': 'red', 'range': 187, 'rangepercentage': 0.37250996015936255}

%%Not necessary to mention
\begin{comment}
Additionally, we found  two applications which migration intervals are \emph{negative}.
However, the migration were done quite similarly to the previous 29 apps: 
one commit first removes all Java code, and then, in the next commit, the Kotlin code is introduced.
%rangeNegative 2: ['remindermail', 'DeuFeiTage']
\end{comment}

\begin{tcolorbox}
%The 33.7\%
The 36\% of the migrated applications were completely migrated  in one step (i.e one single commit).
\end{tcolorbox}

%%% Escalonadas

\paragraph{Staggered migration}

For the rest of the 55 applications (out of 86,  i.e., that is the 64\%), their \emph{migration interval lengths} are greater than one commit.
There, the migrations were gradually done: some version have both Java and Kotlin code.
For example, LocalStorage and Red apps, which code evolution trends are presented in Figures \ref{fig:linesLocalstorage}  and \ref{fig:linesRed}, present intervals with length 4 and 188 commits, respectively.
%
Histogram \ref{fig:kotlin_migration_duration} shows the distribution of the migration intervals for all migrated applications.
Even discarding those 31 migrated in one-step, we observe that most apps were fully migrated in intervals smaller than 50 commits.
However, there are apps with larger intervals. 
For example, that one from SimpleGalery has 266 commits.

We then normalized the intervals. 
As shown by the Histogram \ref{fig:kotlin_migration_duration_normalized}, for most of the apps, the normalized interval's lengths are near to zero, which means that their migrations happened during a short period during their history. 
Coming back to SimpleGalery app, even its interval is one of the largest we found, it's relative small compared to its large complete history: the proportion is 0.093.
%There are some applications with short migration intervals, but they cover a larger portion of history.
%For example, the migration interval of Unstoppable app has 6 commits, and the total number of commits from its history is 23, thus the proportion is 0.26.
%On the contrary, other apps have larger intervals but smaller proportions. For example, SimpleGalery has an interval of 266 and the proportion is 0.093. 


%rangePositive 55: ['red-moon', 'LocalStorage', 'slounik', 'red', 'Simple-Calendar', 'coins-android', 'DmsExplorer', 'davdroid', 'Wiktor-Navigator', 'SheepsGoHome', 'whitakers-words-android', 'Cineaste', 'Voice', 'Podcasts-RAC1-Android', 'ShowsRage', 'toto-anticipation', 'icsdroid', 'Geocaching4Locus', 'AndroidCupsPrint', 'Fractals', 'bo-android', 'PlanningPoker', 'Simple-Notes', 'ScreenStream', 'Msync', 'cryptogram', 'android-torchlight', 'android-app', 'Rocket.Chat.Android', '2050', 'Electric-Fields', 'wulkanowy', 'StockTicker', 'Simple-Draw', 'PackageTracker', 'progressbars', 'hand-and-foot-scores', 'Simple-App-Launcher', 'UNCmorfi', 'Monger-Android', 'Simple-File-Manager', 'show-java', 'Simple-Music-Player', 'unstoppable', 'Simple-Gallery', 'ValenBisi', 'aaf-easydiary', 'Simple-Camera', 'si_counter', 'GPS-Texter', 'VNDB-Android', 'BatteryChargeLimit', 'NightLight', 'apolline-android', 'LanbahnPanel']

\begin{comment}
Figure \ref{fig:scatter_range} shows the relation between the \emph{migration interval}  and that normalized value.
At the left-bottom of the plot  where both proportion of migration and length trend to zero,  are located most of the applications, including the 29 mentioned applications with interval equals to zero. 
This means that migrations happens in few commits consecutive commits inside a large history in terms of number of commits. 
There are some application with short migration intervals, but they covers a larger portion of history, e.g., `Unstoppable' app has 6 commits in its migration interval but the total number of commit is 23, thus the proportion is 0.26.
On the contrary, other projects, such as  SimpleGalery, have larger intervals but the its proportion is lower (for SimpleGalery those values are  266 and 0.093, resp.).


 \begin{figure}[t]
\centering
    \includegraphics[width=0.75\textwidth]{scatter_range_84.pdf}
       \caption{Length (axis X) and proportion (axis Y) of the Migration interval of each migrated application.}
    \label{fig:scatter_range}
 \end{figure}

\end{comment}

%%%%%

\begin{tcolorbox}
Most of the  apps were completely migrated from Java to Kotlin in few commits and the migration interval represents less than the 10\% of the complete history of those applications.
\end{tcolorbox}


%Small: (32) ['SimpleBitcoinWidget', 'remindermail', '2chmatome', 'PosTrainer', 'JanYoShare', 'FRCAndroidWidget', 'KonashiInspectorForAndroid', 'NCBSinfo', 'kmn_bot-tool', 'SimpleHTMLTesterAndroid', 'AndroidCupsPrint', 'easysshfs', 'VoiceMessageBoard', 'DeuFeiTage', 'Android-SearchView-Demo', 'home-button', 'stew', 'Status-Bar-Tachometer', 'vanilla-music-metadata-fetch', 'AnkiEditor', 'Stratum0Widget', 'MockAppDemo', 'Screenshot-Sharer', 'SunWidget', 'SystemUITunerRedesign', 'speedofsound', 'Simple-Thank-You', 'baresip-studio', 'Simple-Flashlight', 'SELinuxModeChanger', 'tincapp', 'youreawinner'] 

%Si_counter special case few Java code

%Davdroid most migration in few

%Rocket.Chat.Android remains two dummies test until 9f39b8645fb50124f6656fe3f334ad4e80aa5b45.
%%last with Java 3ee6de980dd77680c896fe6954c5f817540ec340
%%5509fb5b16fea584f9dbdd985834b9ec9efcf922 remove all Java

\begin{comment}
A particular case is Rocket.Chat.Android, which interval is an \emph{outlier}. 
Their developers stared developing that application in Java, arriving to version  with 20K lines of Java code. 
Later, In the commit, they introduced Kotlin language and during X commits the amount of Kotlin commit moderaly increases, remaining the amount of Java code almost constant. However, in one particular commit\footnote{5509fb5b16fea584f9dbdd985834b9ec9efcf922 } both Java and Kotlin are removed, and the next step the app is rewritten from scracht using mainly Kotlin. 
Few Java code is introduced in this new version, which is gradually removed until the app only contain Kotlin code.
\end{comment}

%%%%%%%%%%%%%%%%
%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsubsection{Detection of commits that Migrate Java to Kotlin}
\label{sec:res:migtypes}

\todo{Remove?}
We now focus on the detection of commits that migrates code from the 86 completely migrated apps. %from Java to Kotlin.
%
We aim to detect the three types of migration commits presented in  Section \ref{sec:commit_migration}. 

\paragraph{Migrations of Files}
\label{sec:res:migrationfiles}

\begin{figure}[t]
%\centering
\begin{subfigure}{0.45\linewidth}% 0.45
 \includegraphics[scale=0.30]{histogram_migrationCommits_84.pdf} % 0.40
  \caption{Distribution of  the number of File-migration commits.}
 \label{fig:kotlin_migration_commits}
\end{subfigure}
\hfil
%\begin{figure}[t!]
\begin{subfigure}{0.45\linewidth}
 \includegraphics[scale=0.30]{histogram_migrationCommits_proportion_84.pdf}
  \caption{Distribution of Proportion of File-migration commits. 
  }
 \label{fig:kotlin_migration_commits_proportion}
\end{subfigure}
\caption{Distribution of the number and proportion of  commits that migrate Files from Java to Kotlin per application.
}
 \label{fig:kotlin_migration_commits_all}
\end{figure}
%computeMigrationFilesAndMigInterval.py


The histogram \ref{fig:kotlin_migration_commits}  shows the distribution of the number of commits that migrate Files (Section \ref{sec:file_migration}) from the set  \emph{\migrapps} (in total 86 apps).
It shows that the majority of the applications (i.e.~$>$50) have few commits that migrate files: from 1 to 5. 
%For example, on of those apps is FRCAndroidWidget, which has one commit\footnote{Commit id: 5d3a0d5a3158b9b463a00ff347f1d5d0398cfa67 from app FRCAndroidWidget} that migrates all the 43 files written in Java to Kotlin. 
%There, its migration interval is 1.
%
On average the number of migration commits is  8.25  and the median is  2.
%The project with greatest number of migration commits is  DmsExplore. %, with 71 of such commits done in a migration interval of 274 (proportion of 25.8\%).

The histogram  \ref{fig:kotlin_migration_commits_proportion} shows the proportion of File migration commits divided by the lengths of the migration intervals.
In total, for 35 apps the proportion is 1 (the bar at the rightmost), meaning that \emph{every} commit in the migration interval migrates, at least, one file from Java to Kotlin.
%commits that migrate files cover the whole migration interval. 
%One of those apps is the previously mentioned FRCAndroidWidget.
%%Commented to reduce the length
\begin{comment}
%Another one, named Cineaste, has a migration interval of 11: on each commit done on that interval, at least one file is migrated to Kotlin, having some commits that migrates up to 12 files.
\end{comment}
\begin{comment}
%%Reduced  
Another app, named UNCmorfi which code evolution is presented in Figure \ref{fig:lines-UNCmorfi}, has an interval with 28 commits,  27  of them commits migrate a single file. 
The proportion of migration commits is  0.96 (96\%,  27/28). 
Note that those commits eventually also modify already written code. 
For instance, commit e446dd\footnote{Commit id: e446dd6e7f4311f9d85e8e6c4c16b58c193b4edd from app UNCmorfi.} modifies Kotlin code from a file (MenuFragment.kt) that was migrated from Java to Kotlin ten commits before.\footnote{Commit id: 5a2111e9b45552f3aaa7850518734a623eebe6ac from app UNCmorfi.}
\end{comment}
On the contrary, the proportion of commits that migrate files inside the migration interval is lower for other apps.
For instance, the application GPS-Texter has a migration interval of 93 commits and only 15 of them (16\%)  migrate code. 
Those commits are alternated with others that are not related to such type of migration.
%, e.g. there are commits such as c82a1d\footnote{commit id: c82a1d5221f27977a322da47dfebda81a03a49d8. Commit message: ``Refactoring: Changed layout names.''} that exclusively updates 7 existing Java files.
%\new{The evolution of those applications mixes both 
%\begin{inparaenum}[\it a)]
%\item maintenance of Java code,
%\item migration of Java code to Kotlin.
%\end{inparaenum}
% }

\begin{tcolorbox}
We identified two groups of apps, based on their  migration interval lengths:
\begin{inparaenum}[\it 1)]
\item apps which most of the commits from their intervals migrate Files, 
%(e.g., FRCAndroidWidget, UNCmorfi);
\item apps which migrations of files are \emph{mixed} with  maintenance activities such as refactoring of Java code. %(e.g., GPS-Texter).
\end{inparaenum}
\end{tcolorbox}

We suspect that file-level migration is done using the auto-converter tool provided by IDEs, which allows developer to migrate a single Java file to Kotlin.

 
%Project DmsExplorer: 71 275 0.258182

%%MigJvToKt: len: 84 min: 1 max: 71 mean: 8.25  median: 2.0 
%MigJv2Kt (proportion): len: 84 min: 0.0029498525073746312 max: 1.0 mean: 0.5681630774635431  median: 0.6666666666666666 

%MigJvToKt AR: len: 84 min: 0 max: 9 mean: 0.8214285714285714  median: 0.0 
%MigJv2Kt AR (proportion): len: 84 min: 0.0 max: 1.0 mean: 0.13478755306942516  median: 0.0 

%MigJvToKt MIG: len: 84 min: 0 max: 71 mean: 7.988095238095238  median: 2.0 
%MigJv2Kt MIG (proportion): len: 84 min: 0.0 max: 1.0 mean: 0.5593078803114628  median: 0.6333333333333333 

\begin{comment}
\begin{figure}[t]
\centering
 \includegraphics[scale=0.45]{scatter_migcommit_vs_miginterval_84.pdf}
  \caption{}
 \label{fig:scatter_migcomit_interval}
\end{figure}
\end{comment}


%\inred{IntersectionL plot distribution of size according to the proportion.}
%Figure \ref{fig:scatter_migcomit_interval}

%%%%%%%%%%%

\paragraph{Fine-grained code migrations}
\label{sec:res:methodlevelmigration}

\todo{Remove?}
We found 11 projects (out of 86 fully migrated projects) that contain, at least, one commit that removes one method from a Java file and adds a method in a Kotlin file (Section \ref{sec:method_migration}).
The average and median number of Method-level migration commits on those 11 projects are 2.36 and 2 respectively.
%Stats project Mig2Mig : len: 11 min: 1 max: 6 mean: 2.3636363636363638  median: 2 standdesv: 1.3666633071248098 
Moreover, we found 13 projects having, at least one commit that removes methods from Java files and, at the same time, adds a new Kotlin file (Section \ref{sec:update_insert_migration}). 
The average and median number of such commits on the 13 projects are 2.3  and  2,  respectively.
%len: 13 min: 1 max: 5 mean: 2.3076923076923075  median: 2 standdesv: 1.3234346564680963

%The commits that present this type of migration shows that there are developers do migration \emph{by hand} because the IDE does only provide (up to now) a tool that converts Java file to  Kotlin file.

We suspect that commits of this type of migration correspond to  migrations written \emph{by hand} because the IDE does only provide (up to now) a tool that converts Java file to Kotlin file.

\begin{tcolorbox}
The migration of Java to Kotlin is mainly done through File-level migrations.
Those convert one Java file to Kotlin and preserve the file names (excepting the file extension).
\end{tcolorbox}

%%%%%% Commented 
\begin{comment}

\newcommand{\lstbg}[3][0pt]{{\fboxsep#1\colorbox{#2}{\strut #3}}}
\lstdefinelanguage{diff}{
 % basicstyle=\ttfamily\small,
   basicstyle=\ttfamily\tiny,
  morecomment=[f][\lstbg{red!20}]-,
  morecomment=[f][\lstbg{green!20}]+,
  morecomment=[f][\textit]{@@},
}

\begin{figure}[t]
\caption{Commit that migrates one method from Java (left) to Kotlin (right)}
\begin{subfigure}{.20\textwidth}
\begin{lstlisting}[language=diff]
diff --git a/app/.../Preview.java 
b/app/.../Preview.java
index df8bfee..a563fb9 100644
@@ -305,20 +305,6 @@
 .....
-  private int getMaxVideoResolution() {
-      final int maxRes = 
-     mConfig.getMaxVideoResolution();
-      switch (maxRes) {
-          case 0:
-              return 400000;
-          case 1:
-              return 1000000;
-          case 2:
-              return 2100000;
-          default:
-              return 0;
-      }
-  }
...
}
\end{lstlisting}
%\caption{Java version}
\end{subfigure}
\begin{subfigure}{.20\textwidth}
\begin{lstlisting}[ language=diff]
diff --git a/app/.../Utils.kt 
b/app/.../Utils.kt
index 436d973..24797c4 100644
@@ -150,5 +150,21 @@
 ...... 
+
+     fun getMaxVideoResolution(config: Config): Int {
+         return 
+  when (config.maxVideoResolution) {
+             0 -> 400000
+             1 -> 1000000
+             2 -> 2100000
+             else -> 0
+         }
+     }
  }
 }
\end{lstlisting}
%\caption{Kotlin version}
\end{subfigure}
\label{fig:method_migration}
\end{figure}


Figure \ref{fig:method_migration}  shows as example one of such commits, found in app Simple-Camera.\footnote{Commit: e8cb8d14648a1f8472c266001db0233d69258eeb from app Simple-Camera.}
The commit removes the method named `getMaxVideoResolution'  which contains a Switch-Case statement in its body.
At the same time, the commit adds into an existing Kotlin file (`Utils.kt') a new method also called `getMaxVideoResolution' containing in its body a `When' statement, which is the Kotlin version of the Java Switch-Case instruction.

\end{comment}

\begin{comment}
\begin{tcolorbox}
The file-level  commit migration is much frequent than the method-level commit migration.
However, it still contributes to the migration  from Java to Kotlin of 13 apps.
\end{tcolorbox}
\end{comment}

%Project with method mig Java to Kotlin File Insert 13: dict_keys(['red', 'Simple-Calendar', 'coins-android', 'Voice', 'Podcasts-RAC1-Android', 'Simple-Notes', 'Rocket.Chat.Android', 'wulkanowy', 'Simple-File-Manager', 'Simple-Music-Player', 'Simple-Gallery', 'aaf-easydiary', 'apolline-android']) 
%All with method migration 16: {'Simple-Gallery', 'aaf-easydiary', 'wulkanowy', 'Simple-Camera', 'PackageTracker', 'Simple-Calendar', 'red', 'Simple-Notes', 'Podcasts-RAC1-Android', 'Simple-Music-Player', 'ShowsRage', 'apolline-android', 'coins-android', 'Simple-File-Manager', 'Rocket.Chat.Android', 'Voice'}


%%%%%%%%%%
%%%%%% RQ 
%%%%%%%%%%%



\section{Methodology}
\label{sec:methodology}

To respond the research questions, in this section we first present a tool, named \miga{}, that analyzes repositories of applications.
Then, we explain how we used it to respond the research questions.
Finally, we present the methodology we applied to carry out a survey which consisted on interviews with developers that migrated code to Kotlin.


\subsection{Methodology applied for analyzing commits}

To detect commits that migrate code, we build a tool called \miga{}.
%
It allows researchers to study the evolution of software applications i.e., the changes done over an application along its history.
In particular, \miga{} focuses on analyzing applications that, during their evolution, have been migrated to one programming language to another (or others).
%
In this section we present \miga{} and we describe how we process its output for responding the research questions.
%
\label{sec:migaframework}

\subsubsection
{Architecture and Implementation of \miga{}}
\label{sec:architecture}


\miga{} is built on top of Coming \cite{coming2019}, a framework for studying the evolution of applications.
\miga{} frameworks takes as input the location of a GIT repository on disk. 
It navigates each commit in chronological order, starting from the oldest one.
\miga{} extends Coming with new analyzers for studying the migration of applications. 
In particular, \miga{}: 
\begin{inparaenum}[\it a)]
\item {Analyzes added, removed and modified files from a commit},
\item {Analyzes commit messages},
\item {Compute lines of code of a version associated to a commit},
\item {Creates  Java ASTs for the Java files affected by a commit},
\item {Creates  Kotlin ASTs for the Kotlin files affected by a commit},
\item {Computes the differences introduced by a commit at the AST level},
\item {Detects commits that migrate code}.
As output, \miga{} generates a JSON file containing, for each commit, the information produced by each aforementioned analyzers.
%\item {Features extractor from Diff\inred{mention?}}
%\item {\inred{Pattern matching from Kotlin changes}},%AST diff
%\item {Pattern matching from Java changes (as explained in Section \ref{})}
\end{inparaenum}


\subsubsection{Lines of code per language}
For responding the first research question (RQ1), we analyze the output of \miga{} containing  per each commits $C$:
\begin{inparaenum}[\it a)]
\item the lines of source code (sLOC), and 
\item number of files 
\end{inparaenum} for each program language used on the version associated to $C$.


\subsubsection{Migration interval}
\label{sec:method:migrationinterval}

For responding the second research question (RQ2), 
we detect from the \miga's output, for each application:
\begin{inparaenum}[\it a)]
\item the first commit that uses Kotlin code, and
\item the last that  uses Java code.
\end{inparaenum} 
We call \emph{migration interval} to the portion of the application's history between those two commits.
%
The \emph{migration interval length} of a migrated application is the number of commits that happen between the two previously retrieved commits.
%
%$Migration\; Interval \; Length \;(MIL)  = Index_{last\_Java\_commit} - Index_{first\_Kotlin\_commit}$, 
%where $Index_{c}$ is the  $index$  of  commit $c$ from a list of commits chronologically sorted.

We further compute the \emph{proportion} of the migration interval w.r.t all the commits from the history of one application by dividing the length of the interval by the total number of commits.


\subsubsection{Detecting commits that migrate code}
\label{sec:commit_migration}

Moreover, also for responding research question 2, we implemented on \miga{} the detection of three types of commits that migrate code.
Those are:

\paragraph{File-level Migration}
\label{sec:file_migration}
\miga{} is able to detect \emph{File-level Migrations} commits.
They are commits that migrate code
by removing one Java file and adding a new Kotlin file.
\miga{} checks that  the names of those files are the same (excluding the file extension).

\paragraph{Finer-grained code level migration}
\label{sec:fine_grained_migration}
\label{sec:method_migration}

\miga{} is able to detect  commits that migrate code at a fine-grained level, which we named \emph{code-level migration}.
This type of migration happens when a developer migrates code by updating two (or more) existing files written in two different languages: 
Java code is removed and Kotlin code is added.
%
The current implementation of  \miga{}  is able of detecting on \emph{methods} level migrations.\footnote{
Even it is not covered in this paper, \miga{} can detect other code-level migrations, such as properties or blocks.}

For detecting method-level migration commits, \miga{} applies the following steps on each commit:
\begin{inparaenum}[\it a)]
\item verifies that 1 or more Java files \emph{and} 1 or more Kotlin files are updated by a commit $c$;
\item for each updated Java or Kotlin file $f$, \miga{} creates an AST (Abstract Syntax Tree) from $f$ and another from the previous version of $f$, i.e. $f_p$;
\item \miga{} computes the differences between the ASTs obtained from $f$ and  $f_p$, using GumTree algorithm \cite{Falleri:2014:FAS}. The output is a list of AST changes, where each change is an operation (Insert, Remove, Update and Move) done over an AST node;
\item \miga{} finds for INSERT operations that affect \emph{methods} in the $diff$ obtained from comparing Kotlin files, and DELETE operations that also affect methods in the other $diff$ obtained from comparing Java files.\footnote{By default, \miga{} does not match the method names, even it is possible to apply string matching heuristics.}
\end{inparaenum}

\paragraph{Update-Insert Migration}
\label{sec:update_insert_migration}
%
%
\miga{} can detect commits that removes a piece of code (e.g., method) from a file written in Java and, at the same time, adds a new file written written in Kotlin.
The implementation of this detector is based on the two previously described cases.

\paragraph{Other types of migrations}
Beyond those three types of commits that migrate code, there could be other that also migrate code.
%
We leave the discover and characterization of such types, and the detection of commit corresponding to the emerging types for future work. In Section \ref{sec:discussion} we discuss some future directions for discovering them.


\begin{comment}
\subsubsection{Commit composition}
\label{sec:method:proportion}
\todo{re-do?}
Moreover, in RQ 1, we study the composition of commits according to the program languages they affect.
The classify commits in 4 types \todo{weird sentence}: 
\begin{inparaenum}[\it 1)]
\item Pure-Java (commits that affect Java code but not Kotlin),
\item Pure-Kotlin (commits that affect Kotlin code but not Java),
\item Mix (commits that affects both Java and Kotlin code),
\item Other (commits that do not affect nether Java nor Kotlin code, e.g., XML files).
\end{inparaenum}
%By affected we mean that a commit adds, modifies or removes one or more files.
\todo{To me moved to Migration study and to compute it after Kotlin is introduced}
\end{comment}



\subsubsection{Amount and proportion of Kotlin code}
\label{sec:method:amountkotlin}

For responding the first  and fourth research questions, 
\miga{} computes, for each application $a$ and for each commit $c$, the number of Java and Kotlin lines of codes (sLOC) of the version of $a$ given by $c$.
It also computes the proportion of Kotlin code by dividing the sLOC of Kotlin per the total sLOC (i.e., Java sLOC + Kotlin sLOC).
Then, for each application, 
we compute the variation of both amount of sLOC and proportion between the latest commit done and an older commit.
In particular, we consider two older commits:
\begin{inparaenum}[\it 1)]
\item the \emph{first commit} that introduces Kotlin,  and
\item a ``\emph{recent commit}'', which corresponds to the commit done just before the latest 10\% of all commits.
\end{inparaenum}
For example, if one application has 110 commits and Kotlin was introduced in the commit \#10, we compare the amount/proportion of Kotlin code between the commit \#110 (latest) and: 
\begin{inparaenum}[\it a)]
\item the \emph{first commit}: \#10 (first Kotlin commit),
\item  the \emph{recent commit}: \#100 (beginning of the last 10\%  from all the Kotlin commits).
\end{inparaenum}


\subsection{Methodology applied for executing the survey}
\label{sec:methodology:survey}

For responding research questions 3, 4 and 5, we conducted a survey with developers.
In this section, we detail the characteristics and initial results of this survey.

\subsubsection{Survey purpose}

We carry out a survey with the main goal of collecting information about the migration of Java code to Kotlin in the context of Android development.
Our survey is explanatory~\cite{experimentationSE2012}: we try to explain why developers migrated their applications. 
The survey follows the format of interviews via email and aims at gathering both qualitative and quantitative data.

We initially asked developers a single question via email:
\quotes{Why did you migrate code from Java to Kotlin?}.
Then, once we received an answer from them, we further asked new questions according to their replies.
For example: 
\begin{inparaenum}[\it a)]
\item \quotes{Did you use the auto-converter code tool provided by the IDE?},
\item \quotes{Which was the criterion (if any) to choose those classes to migrate?},
\item \quotes{Your project still has Java code, Why has it not been completely migrated yet?}.
\end{inparaenum}

We choose this format of exploratory survey, composed of an initial question and followed by a loosely structured questionnaire, to follow the recommendations given by~\cite{experimentationSE2012}, which indicates that letting interviewers handle the questionnaire instead of the respondents themselves offers a number of advantage, such as observing the answers and ask questions according to the observation. 

\subsubsection{Survey setup}

\miga{} framework is able to return \emph{all} commits that migrate Java code to Kotlin from our dataset of Android applications (Section \ref{sec:dataset}).
From each commit, we retrieved the name 
and the email address of the developer that made the commit.
That information is the repository history (GIT).
Then, we sent to each developer that made a migration a personalised email that mentioned that we have analyzed the code of her/his application (mentioning the app name) and we have detected that she/he has write a commit (or several) that migrated code from Java to Kotlin. 

\subsection{Survey results}

We could successfully send, in total, 249 emails.\footnote{Some emails could not be successfully delivered (e.g., those from development companies which employers do not work there any more).}
We got the response from \nremailreplies{} developers, all them from different projects.
This means that $\sim$30\% of developers that migrated Java code to Kotlin in applications from the dataset we study (Section \ref{sec:dataset}) have participated in our survey.
Those interviewed developers are from, at least, 17 countries.
%Even the goal of this paper is not to present a demography study of developers (we did not ask about their country, experience, current status, etc), 
%by analyzing their profiles and email addresses we obtained that those developers are from, at least, 17 different countries. 
%Germany, United States, Korea, Japan, China, India, Brazil, Portugal, Czech Republic,  Spain, France, Canada, Portugal, Italy, Switzerland, Netherlands, among others.
Note that not all participants replied \emph{all} the questions we asked them.
Along this paper we \emph{literally} present answers from developers, without doing any kind of modification (e.g., typos or grammar issues).

Once we collected all answers, 
we detailed analyzed each interview (i.e., a thread of emails with answers and responses) to collect all valuable information for responding research questions 3 (why they migrated), 4 (why not fully migrated) and 5 (advises).


\subsection{Dataset of Android Applications studied}
\label{sec:dataset}
Given Google has officially adopted Kotlin as programming language for Android, 
our goal is to study the migration from Java to Kotlin of Android applications.
For this reason, we analyze Android applications from the FAMAZOA dataset \cite{GoisMateus2019}, which contains 374 Android  with at least one commit done in Kotlin.
FAMAZOA dataset was built by combining open-source applications mined from different sources such as F-Droid\footnote{F-Droid: dataset of open-source Android applications \url{https://f-droid.org}} repository and Android Time Machine \cite{Geiger2018:data}.


%%%%%%%%%% RQs from TSE


%\newcommand{\rqevolution}{{RQ 1: How do mobile apps having Kotlin code evolve during their history?
%}}


\newcommand{\rqappsmigrated}{{RQ 1: How many Android applications have been fully migrated to Kotlin?
}}


\newcommand{\rqmigrationdone}{{
RQ 2: How did developers migrate from Java to Kotlin?
}}

\newcommand{\rqwhymig}{{RQ 3: 
%Why did developers migrate?
Why (for which reasons) have developers migrated their Android applications from Java to Kotlin?
}}


\newcommand{\rqwhynotmig}{{RQ 3: 
Why do developers not \emph{fully} migrate their Android applications from Java to Kotlin?
}}


\newcommand{\rqproportion}{{RQ 4: Are the mobile apps which latest versions have both Java and Kotlin in  process of being migrated?}}




\newcommand{\rqadvise}{{RQ 5: What are the main advises to Android developers based on the interviews?}} 


The research questions that guide our research are:
\begin{enumerate}

\item{\it{ \rqappsmigrated{} }}

We automatically analyze a dataset of Android apps having Kotlin code to filter those that have been fully migrated from Java to Kotlin.

%{\bf \underline{Finding}:} 
\finding{From 374 Android apps analyzed, 86 apps have been completely migrated from Java to Kotlin.}

%\new{To know how many applications were migrated from Java to Kotlin, we analyze the programming language used at the beginning of the development (i.e., firsts commits) and at the most recent commits.
%This analysis would allow to classify apps in 3 classes:
%\begin{inparaenum}[\it a)]
%\item apps only written in Kotlin
%\item Apps fully migrated from Java to %Kotlin
%\item Apps partially migrated from Java to Kotlin.
%\end{inparaenum}
%}


\item  {\it{\rqmigrationdone}}

We analyze the history (code repository) of Android applications that have been fully migrated.
We compute for each app the portion of the history corresponding to the migration.
Then, we  retrieve the commits that carry out the code migration.
From them, we are able to identify the developers that have written the migrations.

\finding{
%The majority of those apps (53) have been migrated in less than 10 consecutive commits \todo{continue}
The  36\%  of  the  migrated  applications  were  completely migrated in one single commit.
%
Those apps do not have any version that contains both Java and Kotlin.
%Moreover, 
}

%
%This allow us 

%In this section we analyze the apps that were initially  written in Java and then, along their history,  were completely migrated to Kotlin with the goal of characterizing the migration activity.

%We analyze the following dimensions:
%\begin{enumerate}
%\item Duration of the migration from  Java to Kotlin (in terms of \#commits),
%\item Detection of commits that migrate code,
%In particular, we focus on two types of migrations defined in Section \ref{sec:miga:migrationanalyzers}:
%\begin{inparaenum}[\it 1)]
%\item File-level migration, and 
%\item Method-level migration. 
%\end{inparaenum}
%\item Inter-language change patterns  that occur on commits that affect both Kotlin and Java files, 
%\item Commit messages of migration commits.
%\item \new{use of Tool?}.
%\end{enumerate}


\item{\it{\rqwhymig}}

We ask developers that have migrated code the main reasons of migrating their Android applications.
%of adopting Kotlin code.
%


\finding{We present the ten main reasons we extracted from the interviews, those include: 
\begin{inparaenum}[\it a)]
\item to avoid limitations of Java versions, 
\item to produce safer code, 
\item to use a modern program language with new features, and 
\item to follow Google's direction.
\end{inparaenum}
}

\item {\it{ \rqproportion}}

We study the apps apps having both languages, but not completely migrated, to determine whether they are in the process of being  migrated from Java to Kotlin.
%\todo{Say something about the trend}
We also contact those developers to know the reasons about those application have not been fully migrated yet.

\finding{For, at least, the 63\% of the  214 apps not completely migrated, the amount and proportion of Kotlin code increase along the time.
The interviews with developers show that they did not finish the migration because of:
\begin{inparaenum}[\it a)]
\item only Java code that needs to be modified is migrated, 
\item only new code is written in Kotlin,
\item lack of time to complete the migration.
\end{inparaenum}
}

\item{\it{\rqadvise}}

We present recurrent episodes and advises that developers mentioned us during the interviews.
%We summarize the main advises developers mentioned us during development 
%based on the interviews which can be used as advises by
%Android developers that plan to migrate from Java to Kotlin.

\finding{We found that:
\begin{inparaenum}[\it a)]
\item Developers used the auto-converter tool for migrating code, however, the converted code often needs to be manually modified;
\item Coroutines simplify the implementation of concurrency in Android;
\item Kotlin code is easier to read and maintain according to the majority of the interviewed developers.
\end{inparaenum}
}

%\new{The interviews with Android developers give us the opportunity to capture the events that could we used by Android developers that have not programmed their Android apps using Kotlin yet.
%\todo{refine}}


\end{enumerate}


%%%%%%%%%end RQs from TSE


%%%% Table Future work
\begin{table}[t]
%\scriptsize
\tiny
\centering
 \begin{tabular}{|l |l|l|} 
\hline
{\tiny Size}&{\tiny Support}&Frequent Item sets\\
\hline
\hline
2 &1.60 \%&  UPD-Invocation in Method (J), UPD-Method Invocation in Method (K)\\
\hline
2 &0.94 \%&  UPD-Local Variable in If (J),UPD-Method Invocation in Method (K)\\
\hline
2 &0.94 \%&  UPD-Invocation in Method  (J), UPD-Property Declaration (K)\\
\hline
2 &0.75 \%& UPD-Local Variable  in Method (J),  UPD-Method Invocation inside If (K)\\
\hline
2 &0.72 \%&  UPD-Invocation in Method (J), INS-Method in Class (K)\\
\hline
\multicolumn{3}{|c|}{...}\\
\hline
2 &0.42 \%&  DEL-Method in Class (J), INS-Method in Class (K)\\
\hline
\multicolumn{3}{|c|}{...}\\
\hline
%2 &0.70 \%&  UPD-Invocation Method (J), INS-Property Declaration inside Method (K)\\
%\hline
%\multicolumn{3}{|c|}{...}\\
%\hline
4 &0.40 \%& DEL-If in Method (J), DEL-Assignment in If (J),\\
 &&  UPD-Local Variable Method (K), UPD-Method Invocation in If (K)\\
\hline

\multicolumn{3}{|c|}{...}\\

\hline

 \end{tabular}
\caption{Sample of most frequent item sets. Each item is composed by
a) action (Insert, Delete, Update),
b) entity type (e.g., Invocation),
c) language (`J' for Java, `K' for Kotlin).
}
\label{tab:apriori}
\end{table}

%%%%%%%%%%%%


%%% Miga steps:
\subsubsection
{Architecture and Implementation of \miga{}}
\label{sec:architecture}


\miga{} is built on top of Coming \cite{coming2019}, a framework for studying the evolution of applications.
\miga{} frameworks takes as input the location of a GIT repository on disk. 
It navigates each commit in chronological order, starting from the oldest one.
\miga{} extends Coming with new analyzers for studying the migration of applications. 
In particular, \miga{}: 
\begin{inparaenum}[\it a)]
\item {Analyzes added, removed and modified files from a commit},
\item {Analyzes commit messages},
\item {Creates  Java ASTs for the Java files affected by a commit},
\item {Creates  Kotlin ASTs for the Kotlin files affected by a commit},
\item {Computes the differences introduced by a commit at the AST level},
\item {Based on the output previous steps, it detects commits that migrate code using heuristics}.
As output, \miga{} generates a JSON file containing, for each commit, the information produced by each aforementioned analyzers.
\end{inparaenum}


\subsubsection{Heuristics for Detecting commits that migrate code}
\label{sec:commit_migration}

We now focus on the three heuristics we implement on  \miga{} to detect three types of commits that migrate code.

\paragraph{File-level Migration}
\label{sec:file_migration}
\miga{} is able to detect \emph{File-level Migrations} commits.
They are commits that migrate code
by removing one Java file and adding a new Kotlin file.
\miga{} checks that  the names of those files are the same (excluding the file extension).

\paragraph{Finer-grained code level migration}
\label{sec:fine_grained_migration}
\label{sec:method_migration}

\miga{} is able to detect  commits that migrate code at a fine-grained level, which we named \emph{code-level migration}.
This type of migration happens when a developer migrates code by updating two (or more) existing files written in two different languages: 
Java code is removed and Kotlin code is added.
%
The current implementation of  \miga{}  is able of detecting on \emph{methods} level migrations.\footnote{
Even it is not covered in this paper, \miga{} can detect other code-level migrations, such as properties or blocks.}

For detecting method-level migration commits, \miga{} applies the following steps on each commit:
\begin{inparaenum}[\it a)]
\item verifies that 1 or more Java files \emph{and} 1 or more Kotlin files are updated by a commit $c$;
\item for each updated Java or Kotlin file $f$, \miga{} creates an AST (Abstract Syntax Tree) from $f$ and another from the previous version of $f$, i.e. $f_p$;
\item \miga{} computes the differences between the ASTs obtained from $f$ and  $f_p$, using GumTree algorithm \cite{Falleri:2014:FAS}. The output is a list of AST changes, where each change is an operation (Insert, Remove, Update and Move) done over an AST node;
\item \miga{} finds for INSERT operations that affect \emph{methods} in the $diff$ obtained from comparing Kotlin files, and DELETE operations that also affect methods in the other $diff$ obtained from comparing Java files.\footnote{By default, \miga{} does not match the method names, even it is possible to apply string matching heuristics.}
\end{inparaenum}

\paragraph{Update-Insert Migration}
\label{sec:update_insert_migration}
%
%
\miga{} can detect commits that removes a piece of code (e.g., method) from a file written in Java and, at the same time, adds a new file written written in Kotlin.
The implementation of this detector is based on the two previously described cases.

\paragraph{Other types of migrations}
Beyond those three types of commits that migrate code, there could be other that also migrate code.
%
We leave the discover and characterization of such types, and the detection of commit corresponding to the emerging types for future work. In Section \ref{sec:discussion} we discuss some future directions for discovering them.


% end miga steps

==> Migration Kotlin-Java_4rev/old-content/removed_initial_version.tex <==
%%%%Old metodology 3.3.3

\subsubsection{Introduction moment}
\label{sec:method:intromoment}

For responding the two first research questions (RQ1 and RQ2), we find, for each application $A$, the commit that first introduces Kotlin code. Then we compute the number of that commit  i.e., the index of them in a list of commits from $A$, chronologically sorted.
Finally, the \emph{introduction moment} is this commit number divided by the total number of commits from $A$. For example, if an application has 60 commits and Kotlin is introduced in the commit number 25, the \emph{introduction moment}  is 15 / 60 = 0.25.


%%%%Old 4.2.1
\subsubsection{Introduction of Kotlin}
\label{sec:res:introkotlinmig}

\begin{figure}[!t]
\centering
%\begin{subfigure}
 \includegraphics[scale=0.5]{histogram_introduction_kotlin_percentage_86.pdf}
  \caption{Introduction of Kotlin on the 86 applications from set \emph{\migrapps}  initially written  in Java and then completely migrated to Kotlin.}
 \label{fig:kotlin_intro_totally_migrated}
%\end{subfigure}
\end{figure}

Histogram from Figure \ref{fig:kotlin_intro_totally_migrated} shows the \emph{introduction} moment of those applications completely migrated from Java to Kotlin. 
We highlight from the figure three \emph{clusters} of applications. 
\begin{inparaenum}[\it a)]
\item A first group of apps written in with Kotlin since the beginning (but not necessary since the first version). 
App `{SheepsGoHome}' is one of those apps. 
\item A second group were Kotlin was introduced at the middle of the application's history, for example, app `Coins-android' has 702 commits and Kotlin was introduced in the commit number 379.
\item A last group (smaller than the previous two) with a \emph{late} introduction of Kotlin. 
Apps `SimpleBitcoinWidget', `LocalStorage', which code evolutions are presented in Figures \ref{fig:linesSimplebitcoinwidget} and \ref{fig:linesLocalstorage} respectively, are two apps with late introduction of Kotlin.
\end{inparaenum}


%%%OLD 4.1.4

\subsubsection{Types of files affected by commits}
\label{sec:commitscomposition}


\begin{figure}[t!]
\begin{subfigure}{0.48\linewidth}
 \includegraphics[scale=0.4]{compositionMigratedFromJava.pdf}
  \caption{Distribution of the percentage of commits according to the type  considering Apps completely migrated from Java to Kotlin. (86 apps in total)}
 \label{fig:composition_commits_migrated}
\end{subfigure}
\hfil
\begin{subfigure}{0.48\linewidth}
 \includegraphics[scale=0.4]{compositionBoth.pdf}
\caption{Distribution of the percentage of commits according to the type  considering  Apps with Java and Kotlin at the latest version (214 apps in total).}
 \label{fig:composition_commits_both_final}
 \end{subfigure}
\caption{Distribution of Types of Commits: Pure-Java, Pure-Kotlin, Mix-Java-Kotlin, Other (e.g., configuration files). \todo{It should be nice pre-and post introduction}}
\label{fig:dist_commits}
\end{figure}




Figure \ref{fig:dist_commits} presents the distribution of the percentage of commits  of apps previously mentioned according to the commit classification presented in Section \ref{sec:method:proportion}. 

Sub-figures \ref{fig:composition_commits_migrated}  considers only commits from the set \emph{\migrapps} and shows that most of the commits affect files that  include neither Java nor Kotlin (bar `Other`), for example, those are XML and pom (Maven configuration) files. 
Then, the rest of the commits affects one program language (either Java or Kotlin). 
The distribution of Pure-Java and Pure-Kotlin commits are similar, but with a slightly larger percentage of Pure-Kotlin  commits than Pure-Java.
Finally, few commits affect both languages at the same time (Mix-Java-Kotlin). 

Sub-figure \ref{fig:composition_commits_both_final} considers apps from \emph{\colanguage{}}.
The distribution is different from that one observed from completely migrated apps (set \emph{\migrapps}): they have more Pure-Java commits than Pure-Kotlin.
Moreover, the distribution of Other files seems similar.
Finally, the percentage of commits affecting both Kotlin and Java (`Mix') is lower than those `Pure', but larger than the distribution of the same type of commits on set \emph{\migrapps}.
Indeed, Mix commits presents some outliers showing that those can represent more than the 20\% of the commits. %\footnote{BikeSharing is one for such apps: :  BikeSharing: 52.38 9.52 28.57 9.52 100.00 } 


\begin{tcolorbox}
%Finding: 
Most of the commits from apps having both languages only affect one single programming language. Few commits affect, at the same time, Kotlin and Java code.
\end{tcolorbox}

%%%%%

%%From  methodology
\subsubsection{Inter-language change pattern}
\label{sec:method:changepatterns}

%\subsubsection{Detecting change patters using frequent itemsets}
%\label{sec:method:fis}

In this work, we focus on finding change patterns (we call them `Inter-language change pattern')  that represent  frequent changes  done by commits that affect both Kotlin and Java code
%Those changes are present in commits that updates one or more Kotlin files and one or mode Java Files.
For that, we apply frequent itemset  algorithm \cite{Agrawal:1993:MAR} over the code changes taken from such commits.
A \emph{frequent itemset} is, given examples that are sets of items and a minimum frequency,  any set of items that occurs at least in the minimum number of examples \cite{Toivonen2010}.  
In our case, an \emph{item} is a single AST change  (see Section \ref{sec:ast_diff}) and an \emph{example} is a set of all AST changes  associated to a code element (e.g., a Commit, Method, File, etc.) affected by a commit.
%We represent a item as follow
An item is represented as a String, thus we transform an AST change  by joining:
\begin{inparaenum}[\it a)]
\item AST action (e.g., Insert),
\item type of the affected AST node,
\item the types of the parent's node,
\item the language (Koltin or Java)
\end{inparaenum}
In this experiment we use the code granularity defined by ChangeDistiller \cite{Fluri2007CDT} (e.g., invocations, assignments, control flow instructions).

Then, we create examples from all commits  affecting both Java and Kotlin files by combining each example taken from an updated Java file  with each one taken from an updated Kotlin file.
Consequently, each example has: 
\begin{inparaenum}[\it a)]
\item one or more items corresponding to changes in Kotlin code, and 
\item one or mores item corresponding to changes in Java code.
\end{inparaenum}


\begin{comment}

In this paper, we focus on finding change patterns at the \emph{method}-level, as done by different previous work \cite{}.
Consequently, an \emph{example} has all the changes from a commit associated to a particular method.
This means that, for example, we create 2 examples from a commit that changes two methods. 
We use Apriori  algorithm \cite{Agrawal:1996:FDA} for finding frequent itemsets.


\end{comment}

\subsubsection{Analysis of Commit Messages from Migration commit}
\label{sec:method:commitmessages}
\todo{remove?}
We find for keywords  that may sugest  migrations inside the  messages  asociated to migration commits (Section \ref{sec:file_migration}) from applications that have been completely migrated from Java to Kotlin.
The list of keywords we used is: 
`convert*',  `migrat*', `rewrit*', `updat*', `port*', `switch*', `transf*', `mov*', and `shift*'.

\new{
We found that the official Kotlin documentation highlights the ability of doing the staggered migration:
\quotes{Kotlin's philosophy is that you don't have to migrate the entire application. Start with a single module or feature, see how it goes, and then gradually move other parts as you see fit}.\footnote{Kotlin documentation: last visit 20-03-2020. \url{https://www.jetbrains.com/lp/mobilecrossplatform/}}
This is possible because Java and Kotlin are 100\% interoperable.
}


%%%%%% OLDS methodology - heuristic

%
\paragraph{Method-level migration}
\label{sec:method_migration}
It corresponds to commits that  remove a method from a Java file and add a method in a Kotlin file.
The heuristic for detecting such migration first verifies, for each commit $C$, that 1 or more Java files \emph{and} 1 or more Kotlin files are updated by $C$.
If that happens, the heuristic computes the two edit-scripts using the AST (Abstract Syntax Tree) differencing algorithm GumTree \cite{Falleri:2014:FAS}.
An AST level edit-script is a set of operations (Insert, remove, update and move) that transform one AST from a file into another AST.
The first one, $edit\_script_{Java}$,  contains the changes between the Java file updated by $C$ and its previous version.
The second one, $edit\_script_{Kotlin}$, contains the changes between the Kotlin file updated by $C$ and its previous version.
Finally, the heuristic searches for Delete operations that affect methods from $edit\_script_{Java}$ and for Insert operations that affect methods from $edit\_script_{Kotlin}$.
If it finds those methods, it marks commit $C$ as \emph{method}-level migration.

\paragraph{Update-Insert Migration}
\label{sec:update_insert_migration}
It corresponds to commits that remove a piece of code (e.g., a method) from a file written in Java and, at the same time, add one or more new files written in Kotlin.
The heuristic checks if a commit $C$ adds a Kotlin file, updates a Java file $F_J$  and the $edit\_script_{Java}$ between $F_J$ and its previous version contains Delete operations that affect methods.

==> Migration Kotlin-Java_4rev/old-content/tab-patterns.tex <==
\begin{table}[t]
\centering
 \begin{tabular}{|c | r |   r|  } 
 \hline
 %min_support: 0.01 minleng: 1 max_len: 6
min_support: 0.01 minleng: 1 max_len: 1
 &10.03 \%& K-UPD-TypeRef$Simple$Piece TypeRef$Simple Type\\
 &9.90 \%& K-UPD-Expr$Name Expr$Call CALL\\
 &7.08 \%& K-INS-Decl$Func Decl$Structured File\\
 

%%


 \hline
 \end{tabular}
\caption{}
\label{tab:patterns}
\end{table}

==> Migration Kotlin-Java_4rev/old-content/tabfindings.tex <==
 \begin{table}[ht]
 \centering
 \scriptsize
 %\renewcommand{\arraystretch}{1.2}
 \caption{Our major findings and their implications.}
 
\begin{tabular}{|p{5.5cm}|p{5.5cm}|}
\hline
\rowcolor{lightgray} \textbf{Findings on Features Adoption} & \textbf{Implications} \\
\hline
(1) 
&
(1) 
\\
\hline
(2) 
&
(2) .
\\

\\
\hline
\rowcolor{lightgray} \textbf{Findings on Moment and Order of Introduction of Features} & \textbf{Implications} \\
\hline

(1) 
& 
(1) 
\\
\hline
\hline

\end{tabular}
\label{tab:findings}
\end{table}

==> Migration Kotlin-Java_4rev/old-content/tmp_infrastructure.tex <==
   
 % \item Kotlin feature study (all) \url{https://github.com/martinezmatias/javavskotlin}
\item Kotlin AST analyzer (dependency to coming), needs a Jar with the Kotlin parser
     \url{https://github.com/martinezmatias/javavskotlin/tree/master/KotlinASTParser}
It's used in the previous paper (somehow)
    
    
\item KotlinDiff \url{https://github.com/martinezmatias/KotlinDiff}. Main project repo with dependency to Kotlin Jar and copied classes from  (Kotlin AST analyzer) 
     
\item Kotlin feature extractor \url{https://github.com/brunomateus/KotlinAstFeatureExtractor/} Find the features. It's the jar we include in the coming extension. In IJ IDE.
    
    
 \item Kastree extension \url{https://github.com/martinezmatias/kastree_ext} In J
 
 
 How to compile in inJ.
 

==> Migration Kotlin-Java_4rev/old-content/update-files.tex <==
\subsubsection{Updates of existing files}

\label{sec:res:updatesfiles}

Now, we focus on commits that updates Java and/or Kotlin codes with the goal later of studying the migration patterns.



\paragraph{Update single language}
\label{sec:res:updatesinglelang}
We now focus on commits that introduces updates on files.
There are 134 projects that have updates of Kotlin files.
Those corresponds, on average, to the 25\% of the commits (21\% in median).

Regarding with Java, 126 projects has commits with updates of Java files.
Those corresponds, on average, to the 34\% of the commits (32\% in median).

Those commits that updates Java and/or Koltin code are the input for studying the \emph{intra-language} change patterns (as we study in Section \ref{}).


%Numbers Updates  java  : len: 126 min: 1 max: 676 mean: 125.42857142857143  median: 60.5 
%Numbers Updates java (Percentage): len: 126 min: 0.0034129692832764505 max: 0.9 mean: 0.338834031250763  median: 0.32307692307692304 
%Numbers Updates  Kotlin : len: 151 min: 1 max: 424 mean: 63.2317880794702  median: 33 
%Numbers Updates   Kotlin (Percentage): len: 151 min: 0.0011235955056179776 max: 0.8549222797927462 mean: 0.28028733651341264  median: 0.24324324324324326 

\paragraph{Update in both Java and Kotlin}
\label{sec:res:updatebothlangs}

From the 142 projects that has in the history both Java and Kotlin,
85 projects has commits that modifies both Kotlin and Java files.
On average the number those commits is 11.3 (which corresponds to the 4\% of the commits on average) and in media is 5.
Some projects such (TrekAdvisor) as  has last number of commits that update both kind of files: 100 (25\%).
Others, such as NHentai-android has few: 

Those commits that introduce modification on both Java and Kotlin are the input for studying the \emph{inter-languages} change patterns (as we study in Section \ref{}). 


\subsubsection{Number of AST changes}
\label{sec:res:astChanges}

==> Migration Kotlin-Java_4rev/old.tex <==
%\IEEEpeerreviewmaketitle

\begin{comment}
\subtitle{}

\titlerunning{Studying the migration from Java to Kotlin of Android Apps}
\author{ Matias Martinez \and  Bruno Gois Mateus}
\institute{
   M. Martinez \at
            Universit\'e Polytechnique Hauts-de-France, France\\
              UVHC - Campus Mont Houy - 59313 Valenciennes, France \\
            \email{Matias.Martinez@uphf.fr}
       \and
B. Gois Mateus \at
            Universit\'e Polytechnique Hauts-de-France, France\\
              UVHC - Campus Mont Houy - 59313 Valenciennes, France \\
              \email{Bruno.GoisMateus@etu.uphf.fr}\\
}

\end{comment}

The research questions that guide our research are:
\begin{enumerate}


\item{\it{\rqwhymig}}

We ask developers that have migrated code from their Android applications the main reasons about the migrations.
This research question is important to understand  limitations of the \emph{traditional} way to written Android apps i.e. using Java language.

\item {\it{ \rqwhynotmig}}

We focus on the application which have both languages on the latest version i.e., not completely migrated at the time of writing this paper.
We contact developers that wrote migrations on those apps to know the reasons about those applications have not been fully migrated yet.

This question is important to detect the difficulties developers have had when they adopted a new programming language to develop Android apps. 

%%%%%%% RQ 3

\item{\it{\rqadvise}}
We present recurrent episodes and advices made by developers gathered from the survey.


\end{enumerate}


%%%%%From dataset.


\subsection{Differences between Legacy migrations and Java to Kotlin migration}
\label{sec:differenceslegacy}
\todo{To intro?/RW?}

A Legacy system can be defined, according to Brodie and Stonebraker, as ``{a system that significantly resists modification and evolution}''~\cite{Brodie1995Legacy}.
Bisbal et al.~\cite{Bisbal1997Migration} mention that legacy systems can host problems as 
\begin{inparaenum}[\it 1)]
\item usually run on obsolete hardware,
\item maintenance can be expensive,
\item lack of clean interfaces to interact with other systems, and 
\item are difficult to extend.
\end{inparaenum}
%%
Consequently, the migration of such legacy systems offers more
flexibility, better system understanding, easier maintenance, and reduced costs~\cite{Bisbal1997Migration}.

However, the migration of Java to Kotlin has some peculiarities compared to legacy migration given by those definitions.
For instance, first, the underlying run-time environment (i.e., the Java virtual machine, or, in case of Android, the Android Runtime -ART- or Dalvik machines) don't need to be updated: Kotlin and Java both are compiled to Java bytecode. 
Second, Java and Kotlin are fully interoperable.
In other types of legacy migrations (e.g., COBOL to web~\cite{Colosimo2009Evaluatinglegacy}), the communication between migrated and not migrated components (or sub-systems) needs \emph{wrappers} (\cite{Bisbal1997Migration,Colosimo2009Evaluatinglegacy}) or \emph{gateways} (\cite{Brodie1995Legacy, Bisbal1997Migration}).
The fully-supported interoperability between Java and Kotlin means that those strategies to allow interoperability are not necessary during the migration from Java to Kotlin.


%%%%%%%%%%%%%%%
We implement the mentioned heuristic on an open-source tool called \miga~\cite{migatool}, built on top of Coming \cite{coming2019}, a framework for studying the evolution of applications.
\miga{} takes as input the location of a cloned GIT repository.
It navigates each branch from the repository in chronological order, starting from the oldest one. 
During the navigation, \miga{} analyzes each commit and applies the heuristic.
Finally, it outputs the list of the migration commits according to the heuristic.
For each commit, it reports:
\begin{inparaenum}[\it a)]
\item commit ID (SHA-1),
\item developer user name,
\item full name,
\item email,
\item branch it belong to, and
\item date.
\end{inparaenum}
That information allows us to contact developers that have migrated code.


\begin{comment}
\subsection{Migrations of Legacy systems}
\label{sec:differenceslegacy}
%\todo{To intro?/RW?}
\todo{moved to new section 2}
A Legacy system can be defined as ``{a system that significantly resists modification and evolution}''~\cite{Brodie1995Legacy}.
Bisbal et al.~\cite{Bisbal1997Migration} mention that legacy systems can host problems as usually run on obsolete hardware and lack of clean interfaces to interact with other systems.
The migration of Java to Kotlin has some peculiarities compared to legacy migration.
First, the underlying run-time environment (i.e., the Java virtual machine)
do not need to be updated: Kotlin and Java both are compiled to Java bytecode. 
Second, 
the communication between migrated and not migrated components on legacy migrations (e.g., COBOL to web~\cite{Colosimo2009Evaluatinglegacy}) needs \emph{wrappers} (\cite{Bisbal1997Migration,Colosimo2009Evaluatinglegacy}) or \emph{gateways} (\cite{Brodie1995Legacy, Bisbal1997Migration}).
The interoperability between Java and Kotlin means that wrappers and gateways are not necessary for migrating Java to Kotlin.

\end{comment}

==> Migration Kotlin-Java_4rev/removed_content_intro.tex <==
\begin{comment}
\finding{We present the ten main reasons we extracted from the survey, those include: 
\begin{inparaenum}[\it a)]
\item to avoid limitations of Java versions, 
\item to produce safer code, 
\item to use a modern program language with new features, and 
\item to follow Google's direction.
\end{inparaenum}
}
\end{comment}

\begin{comment}
\finding{For, at least, the 63\% of the  214 apps not completely migrated, the amount and proportion of Kotlin code increase \inred{along the time}.
The survey shows that they did not finish the migration because of:
\begin{inparaenum}[\it a)]
\item only Java code that needs to be modified is migrated, 
\item only new code is written in Kotlin,
\item lack of time to complete the migration.
\end{inparaenum}
}
\end{comment}



\begin{comment}
\finding{We found that:
\begin{inparaenum}[\it a)]
\item Developers used the auto-converter tool for migrating code, however, the converted code often needs to be manually modified;
\item Coroutines simplify the implementation of concurrency in Android;
\item Kotlin code is easier to read and maintain according to the majority of the interviewed developers.
\end{inparaenum}
}
\end{comment}




{\bf Mining changes using data mining techniques:}
We showed in Section \ref{sec:inter-patterns} that the output of \miga, in particular, the AST changes from migration commits, can be further analyzed to extract knowledge such as migration patterns from migration commits. 
Previous work has applied similar technique on code changes. For example, 
Negara et al. \cite{Negara:2014:MFC} applied frequent item set to detect change patterns from changes done by developers when they write code using IDEs.
Zimmermann et al. \cite{Zimmermann:2004:MVH} data mining techniques  to obtain association rules from version histories for suggesting and predicting likely further changes.
Similarly, Ying et al. \cite{Ying:2004} also used association rule mining to determine the change patterns.
Viggiato et al. \cite{VOFJK:ICSME19}  also used Apriori algorithm to find types of changes that frequently co-occur  in mobile and non-mobile
platforms. 
%They work  focuses on analyzing Java programs, where our focuses on mobile (Android) applications written in Kotlin and Java.
Our experiment, as novelty, focuses on mining patterns composed by changes done in different languages.


\subsubsection{\inred{Move?}Availability of modern features and built-in patterns}


Kotlin languages provides different built-in features that were highlighted by developers. 
One of them is the foremost mentioned Coroutines.
Another one, \emph{Extension function} feature, was mentioned as useful by thirteen developers.
This feature provides the ability to extend a class with new functionality without having to inherit from the class or use design patterns such as Decorator.\footnote{Kotlin Extensions: \url{https://kotlinlang.org/docs/reference/extensions.html}}
%
One developer wrote us about it: 
\quotes{apart from providing a clean way to refactor the code, extensions allow an alternative to Abstraction/Inheritance in order to achieve the Open/Closed Principle, which is invaluable}.

% Ability to extend class definitions and add functions which are available on them is also very useful construct. 

Five developers remarked the \emph{built-in design patterns} provided by Kotlin, which enforces some of the best practices of Java by design.
For example, \emph{Singleton} pattern using the keyword `Object' and \emph{Decorator} pattern using keyword `By'.

Also, most of developers remarked the importance of Kotlin standard libraries, which provide support in, for instance, Collections.
Fourteen developers remarked the importance of having lambdas and streams. 
As one developer said: 
\quotes{Android development stuck on old Java version without e.g. streams (supported only on API 23+). Kotlin standard lib fills these shortcomings}.  

{\bf Implication:} Using Kotlin, Android developers have the possibility to use a modern programming language, with features not always available on Java, and, at the same time, to reach all Android platforms. 


%%%commented
\begin{comment}
\point{Detection of technical debt:} 
\emph{Technical-debt} issues can appear on application after it was (partially or fully) migrated.
According to Avgeriou et al.~\cite{avgeriou_et_al:DR:2016:6693} the term \emph{technical debt} refers to delayed tasks and immature artifacts (code, architecture, design) that incur extra costs in the future in the form of increased cost of change during evolution and maintenance. 

A research challenge is to identify, define, model, and catalogue, technical-debt~\cite{Izurieta2016WorkingTD} associated to the migration from Java and Kotlin.
Other works has focused, for instance, on defining and analyzing the architecture of Android applications (e.g.~\cite{Verdecchia2019Guidelines,Bagheri2016ArchitetureAndroid}) and on the detection of \emph{architectural} technical debt issues (e.g. \cite{Verdecchia2018ATD}).
However, to our knowledge, no work has done studied the impact of the migration on the architecture of the application nor the technical debt that the migration could introduce.
\end{comment}
%% end commented

\begin{comment}
\point{Testing of migrated apps}:
A research challenge is to generate test cases which 
\begin{inparaenum}[\it a)]
\item do \emph{regression testing} after the migration (i.e., to verify the behaviour of the app has not change after the Java to Kotlin conversion)
\item verify the migrated code does not introduce new bugs.
\end{inparaenum}
One of the challenges we envision is to test the interaction between the migrated Kotlin code with the no migrated Java code.
Even both languages are interoperable, Kotlin is a null safe language, it tries to avoid nullable variables.
Consequently, the behaviour of the application can change (i.e., an exception is thrown) when the Java code passes \emph{null} values to the migrated Kotlin code, which could be written without contemplating the nullability of parameters and variables.
\end{comment}

==> Migration Kotlin-Java_4rev/summary_gray_litarature.tex <==
\subsection{Summary of gray-literature}

\cite{daga2018LinkJavaVsKotlin}
\begin{itemize}
    \item learning curve. "Kotlin can be viewed as an improvement on Java, rather than being a full-blown substitute"
     "Java and Kotlin share a number of syntaxes, too, making things easier for developers"
    \item The Issue With NullPointerExceptions
    \item Kotlin Is the "Modern" Language
    \item Interoperability
    \item Community Support
    \item verbosity (Includes dependency)
    \item Checked Exceptions 
    \item Increased Size of .apk
    \item Complete Support for Kotlin in Android Studio. (Includes conversion)
    `` Converting complete source files written in Java to Kotlin is also a breeze. Developers, of course, have to ensure that there are no code losses and/or data corruption during such conversion''
    \item Implicit Widening Conversions and the Question of Stability
    \item No Extra Garbage Collection
    \item First-Class Delegation in Kotlin
    \item Speed of Compilation
    \item Coroutines
    \item Conclusion "It is still advisable for newbie Android developers to learn Java first, and then attempt the switch to Kotlin (type aliases and immutability are two more USPs)"
\end{itemize}

\cite{Sommerhoff2020LinkJavaVsKotlin}

\begin{itemize}
\item Kotlin is more concise: "Features such as type inference, smart casts, data classes, and properties help achieve conciseness."
\item  Kotlin code is safer
\item Kotlin has better support for functional programming
\item  Kotlin speeds up every-day development tasks
\item Kotlin helps reduce errors and bugs in the code `The Kotlin compiler performs many checks, avoiding runtime errors and reducing the cost and effort of error fixes.`
\item The code base shrinks and increases in quality "Technical debt"
\item Developers will be more satisfied and excited about their work
\item  Engineers can take their skills to the next level
\item Kotlin community supports developers
\item Migrate to Kotlin in small steps
`` A good way to start the process is to introduce Kotlin in non-business-critical code to enable initial evaluation and let developers gain experience. For example, test cases can often be greatly simplified using Kotlin. While migration to a new programming language can seem daunting, in this case, the benefits of Kotlin outweigh the costs.``

\end{itemize}

\cite{Rishabh2017LinkKotlinAndroid}

Advantage:
\begin{itemize}
\item  Easy to Set Up: (Android Studio)
\item Interoperable With Java:
\item Includes Synthetic Extension
\item No More NullPointerExceptions (NPEs):
\end{itemize}


\cite{Thornsby2019LinkJavaVsKotlinKeyDiff}
\begin{itemize}
\item offers more succinct code – with no findViewByIds
\item Kotlin is null safe by default
\item Extension functions
\item Coroutines are first-class citizens
\item There are no checked exceptions
\item Native support for delegation (prevent the duplication of code)
``Kotlin’s class delegation is an alternative to inheritance that makes it possible to use multiple inheritance.''
\item Data classes
\item smart class
\item Support for constructors
\item No support for implicit widening conversions
\item Annotation processing libraries with Kotlin
\end{itemize}
``Perhaps most notably: many Android developers are simply more familiar with Java at this point''.


\cite{Caneco2017LinkMigrating}
\begin{itemize}
\item Reduce walls of text: 
\item Null safety: 
\item  built-in
\item Decrease the pain on Code Review: 
\item Run Java and Kotlin side-by-side: 
\item Make use of Java libraries

\end{itemize}

\cite{Caneco2017LinkMigrating}
The converter is a bit conservative on the code conversion, so we needed to perform a few human-based tweaks.




\begin{itemize}
\item  Adjusting nulls 
\item Inline variable initialization
\item Replace “companion object” fields with compile time “const”
\item Keep or remove `@Throws` annotation
\item Replace one-line methods with Kotlin Single Expression method
( Single Expression Functions )
\end{itemize}

"We were able to complete the migration in about six man.hours of effort: three man.hours for converting the code and three more man.hours for peer code review and tweaking.
The code base went down from 1.566 LoC to 1.128 LoC. That’s 23\% less code base to maintain and work on! 
"

\cite{Sommerhoff2015LinkKotlin} 
Enforcing Best Practices

\cite{Butterworth2020LinkMigration}
``There are some tools to help developers achieve this (such as the automatic Java to Kotlin conversion tool), but there are a number of pitfalls to be aware of when it comes to the converter and the interoperability between the languages. ''

``The important thing to remember here is that the Kotlin code generated by the converter may not output the same bytecode as the original Java''

\cite{Paul2018LinkLanguageStart}
``why I suggest a beginner Android developer starting with Java rather than Kotlin.''

``It can help you avoid all boiler-plate code, e.g. you don't need to specify getters and setters, equals(), hashCode() or toString() methods.''


``"What we do is we only take new functionality and write it in Kotlin. It is possible because Kotlin has great interoperability with Java. You can write a single class in Kotlin and keep the rest in Java, or have 99\% of your code in Kotlin and have only some of the leftovers in Java."''

\cite{Heath20LinkSwitch}

\begin{itemize}
\item interoperability
\item Kotlin first
    \item learning curve
    \item idiomatic code, Java style code
\end{itemize}

==> Migration Kotlin-Java_4rev/tableconcepts.tex <==
\begin{table*}[h!]
  \begin{center}
  %\scriptsize
  \small
    \caption{The most frequent codes mined from the survey with developers. Annotations RS, RNM, and RT refer to codes used for responding to research questions 1, 2 and 3, respectively. 
    \new{Those numbered are detailed in Section~\ref{sec:evaluation}.}
   \new{The full table is available in our appendix~\cite{appendix}}.}
    \label{tab:concepts}
    \begin{tabular}{llr} 
    \toprule
      Category	& Code			& \#Dev	\\
      \midrule
    Support	%&			&		\\
	&	Like Google support 	\new{(RS: 2)}	&	32  	\\
	&	Like JetBrains support	\new{(RS)}	&	8	\\
	&	Highlight Importance of IDE for Kotlin		&	6	\\
	&	Adopted due to coolness factor	\new{(RS)}	&	4	\\
	%Advantage Kotlin code w.r.t development and maintainability
	\hline
Advantage of Kotlin %Kotlin code &			&		\\
	&	Reduce code	\new{(RT: 1)}	&	34	\\
code with respect  	&	Easier to read/clear/write/syntactic sugar/easier to maintain	\new{(RT: 1)}	&	23	\\
 to development &	Kotlin has clear syntax		&	17	\\
and maintainability		&	Less Redundant/less verbose 		&	12	\\
	&	Little-to-no boilerplate code		&	9	\\
	&	Kotlin is a modern language/has features from modern languages	\new{(RS)}	&	5	\\
	&	Code more dense/heavy		&	4	\\
	&	Efficient language		&	2	\\
	\hline
Design%	&			&		\\
	&	Ease of implementing MVI (Model-View-Intent) architecture	\new{(RS:3)}	&	6	\\
	&	Ease of implementing MVVM (Model-View-ViewModel) architecture \new{(RS)}		&	1	\\
	&	Availability of Built-in design patterns (e.g., with Extension functions)		&	1	\\
	\hline
Relation with other 	%&			&		\\
	&	Don't want to use Java anymore	\new{(RS: 7)}	&	13	\\
languages	&	Find Java a limitation for Android development	\new{(RS:8)}	&	10	\\
	&	Like Scala	\new{(RS: 6)}	&	5	\\
	&	Like Kotlin Features from C++		\new{(RS: 10)}	&	4	\\
	&	Kotlin has more extensions than Java native package		&	3	\\
	&	Don't like Java	 	\new{(RS)}	&	2	\\
	&	Like Koltin Features from Haskell		\new{(RS)}	&	2	\\
	&	More similarity with Java w.r.t other JVM languages		\new{(RS)}	&	2	\\
	&	Not a fan of Kotlin		&	2	\\
	&	Like  Python		&	1	\\
	&	Similar to Swift	\new{(RS)}	&	1	\\
	\hline
Language	%&			&		\\
Features	&	Like Null safety/Nullability support		\new{(RS:1)}	&	42	\\
	&	Like Extension functions		\new{(RS: 3)}	&	23	\\
	&	Like Coroutine		\new{(RS:3, RT: 2)}	&	21	\\
	&	Like Data class (POJO)		\new{(RS: 3)}	&	16	\\
	&	Highlight Interoperability with Java	\new{(RS: 5)}	&	15	\\
	&	Like lambdas		\new{(RS: 6)}	&	14	\\%/Higher-Order
	&	Like Functional programming available in Kotlin	\new{(RS: 6)}	&	11	\\
	&	Use Coroutines instead of ReactiveX	\new{(RS)}	&	8	\\
	&	More features than Java 	\new{(RS)}	&	7	\\
	&	Like Function as parameters/Higher-Order functions		&	6	\\
	&	Like Immutability		&	5	\\
	&	Highlight Kotlin standard/built-in library		&	5	\\
	&	Like no getters/setters		&	4	\\
	&	Like streams		&	4	\\
	&	Like  built-in API for manipulating collections		&	4	\\
	&	Like default parameters		&	4	\\
	&	Find Kotlin safer than Java		&	3	\\
%		& ...	&...	\\
%	&	Like smart cast		&	3	\\
%	&	Like Type Inference		&	3	\\
%	&	Like Scope Function		&	2	\\
%	&	Like sealed classes 		&	2	\\
%	&	Like named parameters/arguments		&	2	\\
%	&	Like Operator overloading 		&	1	\\
%	&	Find Coroutines  are complex		&	1	\\
%	&	Like Dependency Injection mechanism		&	1	\\
%	&	Like When instruction		&	1	\\
%	&	Like first-class delegation		&	1	\\
\hline
Productivity with Kotlin	%&			&		\\
	&	Increase productivity		&	5	\\
	&	Faster development		&	4	\\
	&	Faster delivery		&	3	\\
	\hline
Running platforms%	&			&		\\
	&	Like Kotlin to write server side apps\footnote{We don't discuss this code in this paper as we focus on Android development.}	\new{(RS)}	&	7	\\
	&	Interested in multiplatform with Kotlin	\new{(RS:9)}	&	6	\\
	&	Kotlin Android Extensions plugin (Android KTX)		\new{(RS)}	&	2	\\
	\hline
Auto-converter%	&			&		\\
	&	Use the auto-converter alongside the migration process		&	36	\\
	&	Had issues when converting using \new{the} auto-converte\new{r} \new{(RT: 2)}		&	24	\\
%se Converter for staring the migration then continue migrating without using it (manual coding
	&	Use \new{the a}uto-converter first, then manual conversion		&	2	\\
	\hline
Migration process%	&			&		\\
	&	App migrated to learn Kotlin	\new{(RS: 4)}	&	19	\\
	&	Migrating using "Boy scout rule" (RNM: 1)		&	14	\\
	&	Only new features would be implemented in Kotlin	(RNM: 2)	&	10	\\
	&	Migrated in one step (i.e., one single commit)		&	9	\\
	&	Migrated only by hand (only manual coding)		&	6	\\
	&	No time to finish	(RNM: 3)	&	5	\\
	&	Only new files in Kotlin/Old code kept in Java	\new{(RNM)}	&	3	\\
	&	Started migration with data class (POJO)		&	2	\\
%	&	Add Java code only to fix legacy code. 		&	1	\\
%	&	Migration Starting with activity		&	1	\\
\hline
Performance %	&			&		\\
	&	Affirm no overhead in performance 		&	2	\\
	&	Affirm no overhead APK size		&	1	\\
	\bottomrule
    \end{tabular}
  \end{center}
\end{table*}

==> future_research_challenges.tex/future_challenges_original.tex <==


\subsection{Main challenges that could be targeted by the research community}
\label{sec:directions}

In this paper we conducted an \emph{exploratory} survey, which are used as pre-study to a more thorough investigation, and may provide new possibilities that could be analyzed and should therefore be followed up in the more focused or thorough survey \cite{experimentationSE2012}. 
In this section, we present those new possibilities that may be exploited by the research community.


\point{Auto-converter tools:}
The survey we conducted show that developers have used the auto-converter code and have modified the output code to have a more idiomatic code.
The automated-generated code is like \quotes{code written with Kotlin syntax but still keeping Java style}.
The potential research directions are twofold. 
First, to detect the cases where Java code that is not correctly converted by state-of-the-art tools.
Second, to define new automated code conversion approaches and tools which generate idiomatic code, and consequently, attempt to reduce the modifications that developers have to do. 
For example, an initial work by Courtney and Neilsen \cite{CATA2019:Vetting} presents an alternative conversion tool.


\point{Detection of technical debt:} 
\emph{Technical-debt} issues can appear on application after it was (partially or fully) migrated.
According to Avgeriou et al.~\cite{avgeriou_et_al:DR:2016:6693} the term \emph{technical debt} refers to delayed tasks and immature artifacts (code, architecture, design) that incur extra costs in the future in the form of increased cost of change during evolution and maintenance. 

A research challenge is to identify, define,  model, and catalogue,   technical-debt~\cite{Izurieta2016WorkingTD} associated to the migration from Java and Kotlin.
Other works has focused, for instance, on defining and analyzing the architecture of Android applications (e.g.~\cite{Verdecchia2019Guidelines,Bagheri2016ArchitetureAndroid}) and on the detection of \emph{architectural} technical debt issues (e.g. \cite{Verdecchia2018ATD}).
However, to our knowledge, no work has done studied the impact of the migration on the architecture of the application nor the technical debt that the migration could introduce.


\point{Refactoring  Kotlin code after migration:}
A challenge for researchers is to define approaches and tools that propose \emph{refactorings} on Kotlin applications after the migration is (partially or fully) done.
We envision two directions.
First, to identify (and potentially automatically remove) \emph{code} technical-debt items (such as code smells and code patterns~\cite{avgeriou_et_al:DR:2016:6693}), previously identified and catalogued. 
According to Snipes and Jedlitschka~\cite{avgeriou_et_al:DR:2016:6693} common tools that support automated refactoring do not address more elaborate technical debt items such as code smells and code patterns. 
Moreover, tools that identify and remove code smells (such as JDeodorant~\cite{Tsantalis2008JDeodorant}) target to Java code. To our knowledge, no refactoring tool targets Kotlin code.
Secondly, we envision refactorings that make Kotlin code (human written or generated by a tool) more idiomatic. 
For example, one could propose the use of new Kotlin features not previously used by the developer, such as \emph{smart casts} or \emph{named parameters}.

\point{Supporting migration activity:}
A potential research direction is to define guidelines, approaches and tools which help developers to migrate their apps.
\emph{Gradual} migrations are convenient for migrating large applications (e.g. Duolingo~\cite{duolingo_migration2020}), because it allows developers and companies to migrate some parts of their apps at the same time they evolve other parts, add new features and release new versions.
 

Gradual (or iterative) migration has been already studied on legacy applications~(e.g., \cite{DeLucia2008DevelopingLegacy}) and consists on first decomposing the legacy apps~\cite{Brodie1995Legacy} and then integrating the decomposed parts using \emph{wrappers} (e.g.,~\cite{CANFORA200099}). 
On the contrary, migration from Java and Kotlin does not need such wrappers, as both languages are interoperable. 
There, a developer needs to define a \emph{migration strategy} which defines consecutive migration steps, and for each of them, a subset of components or code files to be migrated.
This could be a challenging task, specially on large applications: the wrong selection of files to be migrated could increase the migration effort due to emerging errors~\cite{AbdelAziz2020MigEnterprise}. 
We envision the definition of guidelines, approaches and tools which help developers to define a migration strategy and to select the files, packages, or components to be migrated in one particular step in order to minimize the migration effort.


\point{Estimating cost of migration:}
One of the main problems about migrations reported by our survey and by literature on migration (e.g., \cite{Khadka2014LegacyModernization}) is about unfinished migrations due to lack of time or resources.
Models for estimating cost and effort of migration could help developers and companies to  forecast those issues.
Cost and effort estimation of development and maintenance activities has been widely studied during last 30 years (see survey from~\cite{Jorgensen2007SurveyCost}).
A challenge for researchers on migration is to define models that estimate the cost of \emph{migrating} Android apps to Kotlin. 
For that, we envision the estimation of three costs:
\begin{inparaenum}[\it 1.]
\item  cost of migrating the code from Java to Kotlin (C1),
\item cost of  maintaining the migrated Kotlin code (C2), and
\item cost of  maintaining the existing code without migrating it to Kotlin (C3) (which could computed based on existing costs models e.g., \cite{Jorgensen1995,KITCHENHAM200257}).
\end{inparaenum}
Then, by comparing those costs (i.e. C1 + C2 vs C3), developers could better support their decisions about to migrate or not, and consequently, to eventually save time, effort and money.

\point{Kotlin code comprehensibility:} Some participants from our survey mentioned us that the compact syntax of Kotlin affected the readability of code.
A research direction could focus on empirically studying the comprehensibility of Kotlin code.
For doing that, it would be necessary to implement static code analysis tools and to, potentially, define new comprehensibility measures that target Kotlin code.
As pointed by Wyrich et al. ~\cite{Wyrich2020Comprehensibility} those tools would attempt to automatically measure code comprehensibility, to point out sections of the code that are difficult to comprehend and should therefore be refactored.
To our knowledge, there is  no previous work on comprehensibility of Kotlin code.


\point{Testing of migrated apps}:
A research challenge is to generate test cases which 
\begin{inparaenum}[\it a)]
\item  do \emph{regression testing} after the migration (i.e., to verify the behaviour of the app has not change after the Java to Kotlin conversion)
\item verify the migrated code does not introduce new bugs.
\end{inparaenum}
One of the challenges we envision is to test the interaction between the migrated Kotlin code with the no migrated Java code.
Even both languages are interoperable, Kotlin is a null safe language, it tries to avoid nullable variables.
Consequently, the behaviour of the application can change (i.e., an exception is thrown) when the Java code passes \emph{null} values to the migrated Kotlin code, which could be written without contemplating the nullability of parameters and variables.



==> links_gray_biblio.tex <==
Section 3.1.1 
"One of them one told us:
In short I was sick of using java. As a professional android developer there is no reason to use java, especially the incredibly limited version of java you get on Android.}
The majority of the interviewed developers stated that migrating to Kotlin was a way to ``hack'' this problematic: Kotlin provides  moderns features (e.g., lambdas, data class, smart cast, null safe)"
https://dzone.com/articles/java-vs-kotlin-which-programming-language-is-bette -> See the section Kotlin Is the "Modern" Language 
https://blog.udemy.com/kotlin-vs-java-9-benefits-of-kotlin-for-your-business/ -> Third benefit

Section 3.1.2
"Kotlin eliminates the possibility of empty pointers froma compilation perspective: potential NPEs are detected at compile time instead of crashing apps at runtime" 
https://blog.udemy.com/kotlin-vs-java-9-benefits-of-kotlin-for-your-business/ -> second benefit
https://dzone.com/articles/java-vs-kotlin-which-programming-language-is-bette ->Section Issue With NullPointerExceptions
https://www.rishabhsoft.com/blog/kotlin-for-android-development
https://www.androidauthority.com/kotlin-vs-java-783187/
https://docs.google.com/document/d/1ReS3ep-hjxWA8kZi0YqDbEhCqTt29hG8P44aA9W0DM8/edit#heading=h.v6i4iyf7kkxh -> The author of this document is a very well-know Android developer, he was the creator of famous Android Library
https://engineering.talkdesk.com/migrating-from-java-to-kotlin-the-easy-way-37b25a379d72
http://petersommerhoff.com/dev/kotlin/kotlin-for-java-devs/#what-now
https://engineering.autotrader.co.uk/2020/02/21/migrating-to-kotlin-what-to-look-out-for.html
Section 3.1.3
https://dzone.com/articles/java-vs-kotlin-which-programming-language-is-bette -> Community support
https://dzone.com/articles/java-vs-kotlin-which-language-android-developer-sh -> "Even though currently, almost all Android code, examples, and apps are in Java, it will change in the future because Google has declared Kotlin as the official language for Android app development. Many companies have already started using Kotlin for their Android app development, and that's the main reason I think Java developers should learn Kotlin in 2018."
https://www.techrepublic.com/article/should-android-devs-switch-from-java-to-kotlin-heres-googles-advice-on-swapping-programming/
Other links:
https://www.toptal.com/android/kotlin-boost-android-development

==> logs.tex <==

Red-moon
commit ed27961ca829124dcf81ff40945394dc6d268b4d
Author: Stephen Michel <stephen.michel@tufts.edu> 2016-11-11 01:19:09
Committer: Stephen Michel <stephen.michel@tufts.edu> 2016-11-11 01:19:09
Parent: 52a4c3933bfeca188dc8fa398ac0098c59891882 (fix errors in automatic kotlin conversion)
Child: de6b6843cad3e56d3271db4f81ebe1d686e6d306 (fix build errors and some warnings)
Branches: master, origin/HEAD, origin/feature_android-tv, origin/master, origin/onboarding, origin/root-mode, origin/tileLogging, origin/v1-rootmode

Mostly functional location switch. convert to kotlin because studio is stupid.

Automatic conversion also automatically stages the file, making it impossible
to for me to separate changes I made before converting (which were going to
be in a separate commit) and the conversion itself. Thanks, Obama.


==> migratedExamples.tex <==
Case one commit migrated (in branch Develop) but not merged into the master:

``This branch is 4 commits ahead, 1 commit behind master.''

https://github.com/fennifith/Status/compare/develop

https://github.com/fennifith/Status/commit/5790480a4176f1dc089d42169955cafd5b5e73c9


## https://github.com/k9mail/k-9/compare/manage-folders-item


## lot of commits in develop branch
https://github.com/TwidereProject/Twidere-Android





==> old-content/notes-ideas.tex <==



%%% An idea of story:

Does Kotlin help developers to write Android apps with better quality?

If yes: 

How can be help Java developers to 
migrate Java apps to Kotlin?
encourage and help to start developing on Kotlin?

If no:

Which features of Kotlin must evolve for a massive adoption? (Note: maybe out of scope for us, but, we can collaborate with JetBrains -I have a contact there-)
%%



\mcomment{Remark the option to upload patterns -preload patterns already discovered-}
\mcomment{To preload is the key for the gerenal experiment: compute patterns from all projects, then load, then compute frequency (intra-extra-projects)}

\mcomment{Recall two step pattern recognition: patterns coming from individual mappings}

\mcomment{Diffs of patterns}


\mcomment{The algorithm also shows if we consider the parents of the affected node: we can scale up in the affected AST.}

\mcomment{Role matching}

\mcomment{two additional matching features: considering context (Parent) + Roles in labels}


\mcomment{Users using rename command}




What happen in the migration.
e.g. in the Java code when a file is migrated.
1 file is migrated, the other is 

Migration
a1dcbf9f97202bb85d2cb5fc4873dc16854f1a86

Test
eed2f2ec3dabb28199450c54aae6745125adead0

%Patterns from mappings:
%The algorithm  has the ability to add to the pool patterns  

==> old-content/old_miga.tex <==
\section{\miga{}: a framework for analyzing the migration of an application along its software history}
\label{sec:migaframework}

\subsection{Goals of \miga{}}
\label{sec:miga_goal}

\miga{} is a framework for studying the evolution of software applications i.e., the changes done over an application along its history.
In particular, \miga{} focuses on studying applications that, during its evolution, have been migrated to one programming language to another (or others).
Thus, \miga{} aims at extracting knowledge about that languages migration activity.
This extracted knowledge would allow a researcher to understand how developers use new technologies (e.g., emerging programming languages used -specially- in mobile such as Kotlin), and to characterize the migration activity from one technology (e.g., Java) to another (e.g, Kotlin).

%the history of applications of that have been migrated from one or more program language to another (or others)  with the goal of extract knowledge about the language(s) migration.

\subsection{\miga{} in a Nutshell}
\label{sec:miga_nutshell}

%Figure \ref{} shows the steps done by \miga.
 \miga{} receives as input a list of versions of one applications (chronologically ordered) and produces as output the summary of its evolution including all the information about the migration from one language to another.
That output contains for each version $v_i$ different information such the program languages affected in that version, the changes done by $v_i$ at different levels (e.g., line and AST level), and the different change patterns found.



\subsection{Architecture and Implementation of \miga{}}
\label{sec:architecture}

The \miga{} framework is built on top of Coming \cite{coming2019}, a framework built on Java for studying the evolution of applications.
\miga{} frameworks takes as input the location of a GIT repository on disk.
It navigates each commit in chronological order, starting from the oldest one.
Each \emph{commit} adds, removes or introduces changes into \emph{files}, producing a new version of the application.

Beyond Git repositories, Coming (and consequently \miga{}) is capable of analyzing other types of inputs such as pairs of files located in the file system.\footnote{\url{https://github.com/SpoonLabs/coming/blob/master/docs/extension_points.md#input-reader}}


\miga{} applies over each commit a series of \emph{Analyzers}.
Analyzers are organized as a pipeline: each one does a specific task, takes as input all the files affected by the commit (including added, removed, modified files), processes the input, and finally passes the result of its analysis (in addition to the input received) to the next analyzers.

%The analyzers that \miga{} currently provides are:
The current implementation of \miga{} provides analyzers to: 
\begin{enumerate}
\item {Analyze added, removed and modified files from a commit},
\item {Analyze commit messages}
\item {Compute lines of code of a version associated to a commit}
\item {Create  Java ASTs for the Java files affected by a commit},
\item {Create  Kotlin ASTs for the Kotlin files affected by a commit},
\item {Compute the differences introduced by a commit at the AST level},
\item {Detect and analyze commits that migrate code}.
%\item {Kotlin AST diff} (as explained in Section \ref{}),
%\item {Features extractor from Diff\inred{mention?}}
%\item {\inred{Pattern matching from Kotlin changes}},%AST diff
%\item {Pattern matching from Java changes (as explained in Section \ref{})}
\end{enumerate}

%\inred{in the algorithm to put the diff algo as input}
Finally, once \miga{} processes all the commits from the input, it processes the results produced by each analyzer from each commit, with the goal of creating the summary of the results. 
The Output Processor are the components that takes the output produced by one or more analyzers and produces a new output. 
For example, an output processor  counts the number of commits that have both modifications in both Java and Kotlin files. Another output processor exports all the results to JSON format.

All the analyzers previously presented have been used in this paper to study the applications that are migrated to one language to another.

%In particular, \miga{} 
%it computes the intra-language change patterns (i.e., the patterns that express changes from one language) and the inter-languages change patterns (i.e., the patterns that express changes happening in two or more program languages).

\miga{} can be easily extended using the extension mechanism provided by the underlying platform (Coming \cite{coming2019}):
new analyzers and output processors can be easily added.\footnote{Extension points of Coming: \url{https://github.com/SpoonLabs/coming/blob/master/docs/extension_points.md}}


\subsection{Analyzers from \miga{} for studying code migration}
\label{sec:miga:migrationanalyzers}

In this section we detail the functionality provided by \miga{} for studying the migration of applications.
Note that this functionality is not fully provided by the core of Coming.



\subsubsection{Analyzing Files from Commit}
\label{sec:files_commit}

\newcommand{\langsrc}{\new{$Lang\_Src$}}
\newcommand{\langdst}{\new{$Lang\_Dst$}}

\miga{} extends Coming by adding the functionality for analyzing commits written in more than one language. (Note that Coming only focuses on Java code).
This functionality is required for studying the migration of applications.

A commit can modify a version of an application in different ways.
For instance, if we consider one applications having two programming languages, one called \langsrc{} (Source) and another \langdst{} (Destination), there are 6 different \emph{actions}  done by a commit:

\newcommand{\Caddsrc}{\new{$Commit\_add\_src$}}
\newcommand{\Cadddst}{\new{$Commit\_add\_dst$}}
\newcommand{\Cremsrc}{\new{$Commit\_rem\_src$}}
\newcommand{\Cremdst}{\new{$Commit\_rem\_dst$}}
\newcommand{\Cupsrc}{\new{$Commit\_up\_src$}}
\newcommand{\Cupdst}{\new{$Commit\_up\_dst$}}


\begin{enumerate}
    \item \Caddsrc: Add new \langsrc{} file,
    \item \Cadddst{}: Add new \langdst{} file,
     \item \Cremsrc{}: Remove \langsrc{} file, 
    \item \Cremdst{}: Remove \langdst{} file, 
    \item \Cupsrc{}: Updates Files in language \langsrc,
    \item \Cupdst{}: Updates Files in language \langdst.
\end{enumerate}

In particular, the current implementation of \miga{} is able to work with two program languages: Java and Kotlin. In case of analyzing the migration of Java app to Kotlin, the \langsrc{}  language is Java, and the \langdst{} is Kotlin.

\subsubsection{File-level Migration}
\label{sec:file_migration}

The first analyzer provided by \miga{} is able to detect commits that carry out \emph{File-level Migrations}.
This case represents the migration of code from one file written in one language to another file written in a different language.
According to the actions presented in Section \ref{sec:files_commit}, this migration case happens when a commit Adds and Removes files from different languages: a commit containing action  \Caddsrc{} and \Cremdst{},  or \Cadddst{} and \Cremsrc{}), and the names of the files are the same (excluding the file extension).

\subsubsection{Analyzing Finer-grained Migration (code level)}
\label{sec:fine_grained_migration}

In addition to the file-level migration explained in Section \ref{sec:file_migration}, \miga{} is able to analyze the migration at a fine-grained level, which we named \emph{code-level migration}.
This migration happens when a developers migrates code by, for instance, updating two (or more) existing files written in two different languages. 
This situation corresponds to the cases \Cupsrc{} and \Cupdst{} from Section \ref{sec:files_commit}.
From one of those files, code is removed (e.g., Java code) and in the other, code is added (e.g., Kotlin code).

The current implementation of  \miga{} provides an analyzer that focuses on detecting one particular \emph{code-level} migrations: \emph{methods}.
The goal is to detect migration cases that migrate a particular method written in Java to a new method written in Kotlin. Note that \miga{} is also capable to detect migrations from Kotlin to Java, however, in this paper we focus on the migration Java to Kotlin.

In this paper we focus on method-level migration, even \miga{} also provides the possibility to detect other code-level migrations, such as properties or blocks. 


\paragraph{From file to AST}
\label{sec:ast_parser}

The  Finer-grained Migration analyzer works at the AST level. 
Thus, \miga{} converts every code file affected by a commit to an AST (Abstract Syntax Tree) and stores them for further analysis such as fine-grained differencing.

If a commit modifies a file $f$, \miga{} creates the AST for the version of the file \emph{before}  the modification (i.e., the previous version of the file), and another AST for the file with the changes introduced by the commit.
Then, \miga{} stores that pairs of ASTs.

\miga{} provides code source parser for different program languages. In this work, we focus on two: one for parsing Java code, another for parsing Kotlin code.


\paragraph{Computing AST diff}
\label{sec:ast_diff}


%\miga{} 
MigA focuses on studying the changes that happen in files that are modified  by a commit (cases from  \Cupsrc{} and \Cupdst{}).
Thus, for each  commit $c$ that updates a file $f$, \miga{} computes the differences between the AST of the previous version of the file $f$ (i.e., the version without having the change introduced by $c$) and the current version of  $f$ (i.e., the version with the changes introduced by $c$).
For computing the AST diff, \miga{} uses GumTree algorithm \cite{Falleri:2014:FAS}.
The output of that comparison is a list of AST changes, where each change is an operation (GumTree has four: Insert, Remove, Update and Move) over an AST node.
%%%



\paragraph{Detection of code-level migration}
\label{sec:method_migration}

As difference from the migration case mentioned in Section \ref{sec:file_migration}, the code-level migration is at a fine-grained level: a portion of a file (e.g., a method) is migrated rather than the complete file.

For detecting code-level migration in one commit $c$, \miga{} takes as input the output of the AST diff algorithm explained in Section \ref{sec:ast_diff}.
There, \miga{} computes the AST diff for each updated file $c$.
Then, \miga{} checks the extension of the updated files to verify that the commits affects code written in more than one language. 
If the commit only affects code written in one language, the code-level migration does not take place.
If the commit affects two or more files, i.e., updates files from different languages, 
then \miga{} computes the $diff$ for each file and its precedent version. 
Thus,  each $diff$ is related to a particular language.
 
Finally, 
\miga{} finds for INSERT operations that affect \emph{methods} in one diff (e.g., a diff from Kotlin files), *and* DELETE operations that also affect methods in the other diff (e.g., a diff from Java files).
If \miga{} found those pairs of operations, it stores them for a subsequent analysis.
Note that, by default, \miga{} does not match  the method names, even it is possible to do it.

%After that, \miga{} checks the method names of each pair of INSERT - DELETE operation.
%if the names matches, it is a \emph{perfect} migration.

%%name analysis.

\subsection{Detection of other types of migrations}

\miga{} is able to detect other types of migrations.
One that combines the two previous strategies consist on finding commits that do both:
\begin{inparaenum}[\it a) ]
\item adds a \langdst{} file, and
\item updates a \langsrc{} file by removing a method.
\end{inparaenum}
This case contemplates that a developer removes a method from a file written in one language \langsrc{} (e.g., Java) and adds, at the same time, a new file written in \langdst{} language (e.g., Kotlin) containing the new implementation of the removed method.

Our goal is that other researcher uses the analyzers provided by \miga{} for creating new strategies for detecting migrations of code.


%%%%%%%%%



\begin{comment}


\subsection{Discovering Code Change Patterns}
\label{sec:change_patterns}


\subsubsection{Pattern detection algorithm}
The goal of \miga{} is to detect the most frequent code changes that happen on this scenario (i.e., when files are updated).\inred{UPDATE}
For that, in this paper we propose a new algorithm, called \algoname{}, for  change pattern detection which we introduce below in the next Section \ref{sec:pattern_detection}.
%Using this algorithm, called \algoname{}, we are able to capture, the patterns 
%We use this algorithm for detecting two kind of patterns:
%1) frequent changes that happens in one language (be Src or Dest),
%2) patterns of changes between two or more languages.


%The goal of \migga{} is to extract knowledge about the migration.
%In particular, 
\miga{} focuses on extracting two types of code change patterns:
\begin{inparaenum}
\item intra-languages change patterns which capture frequent changes produced in one particular language.
\item inter-languages change pattern (\emph{migration patterns}) which capture frequent changes involving two or more languages.
\end{inparaenum}
Moreover, \miga{} classifies commits according to a migration taxonomy.
%


\subsubsection{Intra-language change pattern}

\miga{} reads those inputs for each project analyzed and, to compute the most frequent patterns, applies a procedure similar to that one explained in Section \ref{}.
It first creates an empty Pattern pool.
Then, it gradually reads each pattern and compare it with those already in the pool using the algorithm presented in \ref{}.
if the pattern already exists ($pt$), it associates all instances from project into ($pt$). Otherwise it add it to the pool.

\subsubsection{Inter-language change pattern}

Similar to \ref{}. the difference is that a pattern has two components: one represents the Java pattern, the other one the Kotlin pattern.
When \miga{} matches two patterns, it applies two times the algorithms \ref{}: one for the Java part, the other for the Kotlin.
\miga will consider a pattern matching if the similarity of \emph{both} parts are larger than a threshold $txxxx$.


\subsection{Analyzing commit message}
\label{sec:commit message}

Previously in this section, we have focused on studying the files affected by the commit for detecting migration cases.
The  \emph{commit message} is written by the developers with the propose of explaining what the commit has, the main changes introduced by it, etc.
\miga{} also is able to study the \emph{commit message} for detecting commits that migrate code.
For that, \miga{} filters commits which message includes keywords such as `migration', `converted', etc.

\end{comment}

%%commit message keywords: converted, automated


%%%%%%%%%%%%%%%%%%%%%
%%%
%%%%%%%

\section{Methodology}
\label{sec:methodology}


%\newcommand{\rqevolution}{{RQ 1: How do mobile apps having Kotlin code evolve during their history?
%}}

\newcommand{\rqappsmigrated}{{RQ 1: How many Android applications have been fully migrated to Kotlin?
}}


\newcommand{\rqwhymig}{{RQ 2: 
%Why did developers migrate?
For which reasons have developers migrated their Android applications from Java to Kotlin?
}} %%


\newcommand{\rqmigrationdone}{{
%Previous
%RQ2: How the migration from Java to Kotlin is done?
%\new{What are the strategies of migration code?}
\new{RQ 3: How did developers migrate from Java to Kotlin?}
}}


\newcommand{\rqproportion}{{RQ 3: Are the mobile apps which latest versions have both Java and Kotlin in  process of being migrated?}}
%%How does not migrated 



==> old-content/others-old.tex <==
%files after the introduction of Dst
\begin{comment}
\begin{enumerate}
    \item Add Kotlin file Remove Java file
    \item Add Java file Remove Remove file

Add Java File

    \item Updates Changes in Java (language Src)
    \item Updates Changes in Kotlin (language Dest)
    
    
\end{enumerate}
\end{comment}

==> old-content/removed_Methodology_TSE.tex <==

\section{Methodology}
\label{sec:methodology}

To respond the research questions, in this section we first present a tool, named \miga{}, that analyzes repositories of applications.
Then, we explain how we used it to respond the research questions.
Finally, we present the methodology we applied to carry out a survey which consisted on interviews with developers that migrated code to Kotlin.


\subsection{Methodology applied for analyzing commits}

To detect commits that migrate code, we build a tool called \miga{}.
%
It allows researchers to study the evolution of software applications i.e., the changes done over an application along its history.
In particular, \miga{} focuses on analyzing applications that, during their evolution, have been migrated to one programming language to another (or others).
%
In this section we present \miga{} and we describe how we process its output for responding the research questions.
%
\label{sec:migaframework}

\subsubsection
{Architecture and Implementation of \miga{}}
\label{sec:architecture}


\miga{} is built on top of Coming \cite{coming2019}, a framework for studying the evolution of applications.
\miga{} frameworks takes as input the location of a GIT repository on disk. 
It navigates each commit in chronological order, starting from the oldest one.
\miga{} extends Coming with new analyzers for studying the migration of applications. 
In particular, \miga{}: 
\begin{inparaenum}[\it a)]
\item {Analyzes added, removed and modified files from a commit},
\item {Analyzes commit messages},
\item {Compute lines of code of a version associated to a commit},
\item {Creates  Java ASTs for the Java files affected by a commit},
\item {Creates  Kotlin ASTs for the Kotlin files affected by a commit},
\item {Computes the differences introduced by a commit at the AST level},
\item {Detects commits that migrate code}.
As output, \miga{} generates a JSON file containing, for each commit, the information produced by each aforementioned analyzers.
%\item {Features extractor from Diff\inred{mention?}}
%\item {\inred{Pattern matching from Kotlin changes}},%AST diff
%\item {Pattern matching from Java changes (as explained in Section \ref{})}
\end{inparaenum}


\subsubsection{Lines of code per language}
For responding the first research question (RQ1), we analyze the output of \miga{} containing  per each commits $C$:
\begin{inparaenum}[\it a)]
\item the lines of source code (sLOC), and 
\item number of files 
\end{inparaenum} for each program language used on the version associated to $C$.


\subsubsection{Migration interval}
\label{sec:method:migrationinterval}

For responding the second research question (RQ2), 
we detect from the \miga's output, for each application:
\begin{inparaenum}[\it a)]
\item the first commit that uses Kotlin code, and
\item the last that  uses Java code.
\end{inparaenum} 
We call \emph{migration interval} to the portion of the application's history between those two commits.
%
The \emph{migration interval length} of a migrated application is the number of commits that happen between the two previously retrieved commits.
%
%$Migration\; Interval \; Length \;(MIL)  = Index_{last\_Java\_commit} - Index_{first\_Kotlin\_commit}$, 
%where $Index_{c}$ is the  $index$  of  commit $c$ from a list of commits chronologically sorted.

We further compute the \emph{proportion} of the migration interval w.r.t all the commits from the history of one application by dividing the length of the interval by the total number of commits.


\subsubsection{Detecting commits that migrate code}
\label{sec:commit_migration}

Moreover, also for responding research question 2, we implemented on \miga{} the detection of three types of commits that migrate code.
Those are:

\paragraph{File-level Migration}
\label{sec:file_migration}
\miga{} is able to detect \emph{File-level Migrations} commits.
They are commits that migrate code
by removing one Java file and adding a new Kotlin file.
\miga{} checks that  the names of those files are the same (excluding the file extension).

\paragraph{Finer-grained code level migration}
\label{sec:fine_grained_migration}
\label{sec:method_migration}

\miga{} is able to detect  commits that migrate code at a fine-grained level, which we named \emph{code-level migration}.
This type of migration happens when a developer migrates code by updating two (or more) existing files written in two different languages: 
Java code is removed and Kotlin code is added.
%
The current implementation of  \miga{}  is able of detecting on \emph{methods} level migrations.\footnote{
Even it is not covered in this paper, \miga{} can detect other code-level migrations, such as properties or blocks.}

For detecting method-level migration commits, \miga{} applies the following steps on each commit:
\begin{inparaenum}[\it a)]
\item verifies that 1 or more Java files \emph{and} 1 or more Kotlin files are updated by a commit $c$;
\item for each updated Java or Kotlin file $f$, \miga{} creates an AST (Abstract Syntax Tree) from $f$ and another from the previous version of $f$, i.e. $f_p$;
\item \miga{} computes the differences between the ASTs obtained from $f$ and  $f_p$, using GumTree algorithm \cite{Falleri:2014:FAS}. The output is a list of AST changes, where each change is an operation (Insert, Remove, Update and Move) done over an AST node;
\item \miga{} finds for INSERT operations that affect \emph{methods} in the $diff$ obtained from comparing Kotlin files, and DELETE operations that also affect methods in the other $diff$ obtained from comparing Java files.\footnote{By default, \miga{} does not match the method names, even it is possible to apply string matching heuristics.}
\end{inparaenum}

\paragraph{Update-Insert Migration}
\label{sec:update_insert_migration}
%
%
\miga{} can detect commits that removes a piece of code (e.g., method) from a file written in Java and, at the same time, adds a new file written written in Kotlin.
The implementation of this detector is based on the two previously described cases.

\paragraph{Other types of migrations}
Beyond those three types of commits that migrate code, there could be other that also migrate code.
%
We leave the discover and characterization of such types, and the detection of commit corresponding to the emerging types for future work. In Section \ref{sec:discussion} we discuss some future directions for discovering them.


\begin{comment}
\subsubsection{Commit composition}
\label{sec:method:proportion}
\todo{re-do?}
Moreover, in RQ 1, we study the composition of commits according to the program languages they affect.
The classify commits in 4 types \todo{weird sentence}: 
\begin{inparaenum}[\it 1)]
\item Pure-Java (commits that affect Java code but not Kotlin),
\item Pure-Kotlin (commits that affect Kotlin code but not Java),
\item Mix (commits that affects both Java and Kotlin code),
\item Other (commits that do not affect nether Java nor Kotlin code, e.g., XML files).
\end{inparaenum}
%By affected we mean that a commit adds, modifies or removes one or more files.
\todo{To me moved to Migration study and to compute it after Kotlin is introduced}
\end{comment}



\subsubsection{Amount and proportion of Kotlin code}
\label{sec:method:amountkotlin}

For responding the first  and fourth research questions, 
\miga{} computes, for each application $a$ and for each commit $c$, the number of Java and Kotlin lines of codes (sLOC) of the version of $a$ given by $c$.
It also computes the proportion of Kotlin code by dividing the sLOC of Kotlin per the total sLOC (i.e., Java sLOC + Kotlin sLOC).
Then, for each application, 
we compute the variation of both amount of sLOC and proportion between the latest commit done and an older commit.
In particular, we consider two older commits:
\begin{inparaenum}[\it 1)]
\item the \emph{first commit} that introduces Kotlin,  and
\item a ``\emph{recent commit}'', which corresponds to the commit done just before the latest 10\% of all commits.
\end{inparaenum}
For example, if one application has 110 commits and Kotlin was introduced in the commit \#10, we compare the amount/proportion of Kotlin code between the commit \#110 (latest) and: 
\begin{inparaenum}[\it a)]
\item the \emph{first commit}: \#10 (first Kotlin commit),
\item  the \emph{recent commit}: \#100 (beginning of the last 10\%  from all the Kotlin commits).
\end{inparaenum}


\subsection{Methodology applied for executing the survey}
\label{sec:methodology:survey}

For responding research questions 3, 4 and 5, we conducted a survey with developers.
In this section, we detail the characteristics and initial results of this survey.

\subsubsection{Survey purpose}

We carry out a survey with the main goal of collecting information about the migration of Java code to Kotlin in the context of Android development.
Our survey is explanatory~\cite{experimentationSE2012}: we try to explain why developers migrated their applications. 
The survey follows the format of interviews via email and aims at gathering both qualitative and quantitative data.

We initially asked developers a single question via email:
\quotes{Why did you migrate code from Java to Kotlin?}.
Then, once we received an answer from them, we further asked new questions according to their replies.
For example: 
\begin{inparaenum}[\it a)]
\item \quotes{Did you use the auto-converter code tool provided by the IDE?},
\item \quotes{Which was the criterion (if any) to choose those classes to migrate?},
\item \quotes{Your project still has Java code, Why has it not been completely migrated yet?}.
\end{inparaenum}

We choose this format of exploratory survey, composed of an initial question and followed by a loosely structured questionnaire, to follow the recommendations given by~\cite{experimentationSE2012}, which indicates that letting interviewers handle the questionnaire instead of the respondents themselves offers a number of advantage, such as observing the answers and ask questions according to the observation. 

\subsubsection{Survey setup}

\miga{} framework is able to return \emph{all} commits that migrate Java code to Kotlin from our dataset of Android applications (Section \ref{sec:dataset}).
From each commit, we retrieved the name 
and the email address of the developer that made the commit.
That information is the repository history (GIT).
Then, we sent to each developer that made a migration a personalised email that mentioned that we have analyzed the code of her/his application (mentioning the app name) and we have detected that she/he has write a commit (or several) that migrated code from Java to Kotlin. 

\subsection{Survey results}

We could successfully send, in total, 249 emails.\footnote{Some emails could not be successfully delivered (e.g., those from development companies which employers do not work there any more).}
We got the response from \nremailreplies{} developers, all them from different projects.
This means that $\sim$30\% of developers that migrated Java code to Kotlin in applications from the dataset we study (Section \ref{sec:dataset}) have participated in our survey.
Those interviewed developers are from, at least, 17 countries.
%Even the goal of this paper is not to present a demography study of developers (we did not ask about their country, experience, current status, etc), 
%by analyzing their profiles and email addresses we obtained that those developers are from, at least, 17 different countries. 
%Germany, United States, Korea, Japan, China, India, Brazil, Portugal, Czech Republic,  Spain, France, Canada, Portugal, Italy, Switzerland, Netherlands, among others.
Note that not all participants replied \emph{all} the questions we asked them.
Along this paper we \emph{literally} present answers from developers, without doing any kind of modification (e.g., typos or grammar issues).

Once we collected all answers, 
we detailed analyzed each interview (i.e., a thread of emails with answers and responses) to collect all valuable information for responding research questions 3 (why they migrated), 4 (why not fully migrated) and 5 (advises).


\subsection{Dataset of Android Applications studied}
\label{sec:dataset}
Given Google has officially adopted Kotlin as programming language for Android, 
our goal is to study the migration from Java to Kotlin of Android applications.
For this reason, we analyze Android applications from the FAMAZOA dataset \cite{GoisMateus2019}, which contains 374 Android  with at least one commit done in Kotlin.
FAMAZOA dataset was built by combining open-source applications mined from different sources such as F-Droid\footnote{F-Droid: dataset of open-source Android applications \url{https://f-droid.org}} repository and Android Time Machine \cite{Geiger2018:data}.


%%%%%%%

==> old-content/removed_TSER1.tex <==
%%%% From discussion part

\subsection{Future Uses of \miga{}}

\miga{} can be used by other researchers to study the evolution of the migration activity of applications written in other program languages.
\miga{} can be extended using the extension mechanism provided by the underlying platform (Coming \cite{coming2019}).
%\footnote{Extension points: \url{https://github.com/SpoonLabs/coming/blob/master/docs/extension_points.md}}
A researcher can add: 
\begin{inparaenum}[\it a)]
\item new programming language parsers (currently \miga{} provides parsers for Java and Kotlin, and
\item new analyzers (in addition to those presented in Section \ref{sec:architecture}).
%\item and output processors.
\end{inparaenum}

One of the future direction we plan to study is the detection of migration change patterns.
This will allow us to detect commits that migrates code which do not fall into the three types of migration commits we defined in Section \ref{sec:commit_migration}.
For that, we define \emph{inter-languages change pattern} as a pattern which captures frequent changes involving two or more languages.
We aim at detecting
\emph{Inter-language change patterns} that occur on commits that affect both Kotlin and Java files.
We now present an initial experiment in that direction.

\subsubsection{Discovering Inter-language change patterns}
\label{sec:inter-patterns}
We carried out a first experiment for discovering Inter-language change patterns.
We applied frequent itemset (FIS) algorithm \cite{Agrawal:1993:MAR}, in particular Apriori algorithm \cite{Agrawal:1996:FDA},
on commits that update one or more Kotlin files \emph{and} one or mode Java files.
A \emph{frequent itemset} is, given examples that are sets of items and a minimum frequency,  any set of items that occur at least in the minimum number of examples \cite{Toivonen2010}. 
We created an itemset per each commit, where each item is a single AST change.
Each itemset has 1 or more changes on the Java AST \emph{and} 1 or more changes on the Kotlin AST.
As mentioned in Section \ref{sec:architecture} \miga{} outputs this information per each commit.
%
We applied FIS over the changes extracted from 422 commits that update both Java and Kotlin, those commits come from 33 migrated apps (note that the remaining 53 out of 86 apps from set \emph{\migrapps{}} do not have any commits that updates both Java and Kotlin).

Table \ref{tab:apriori} shows a sample of the most frequent \emph{inter-language change patterns} we found using FIS. 
The first row shows that the 1.6\% of the commits analyzed update a Method Invocation located inside a Java method  \emph{and also} it updates method Invocation located inside in a Kotlin Function.
One frequent item (row 7) corresponds to the method-level migration discussed in Section \ref{sec:res:methodlevelmigration}.
However, beyond that pattern,  most of frequent itemsets do not  remove code.
This can be explained by the fact that, when migrating, developers also need to update the remaining Java code (e.g., to update the references to the migrated code).
%
We leave for future work the research on other pattern detection algorithms.


\subsection{Further characterization of migrations}

One of our goals was to understand which functionality was migrated to Kotlin.
We aimed to respond the question: \quotes{Which functionality was migrated to Kotlin?}.
Most of developers confirmed us that they have started the migration by migrating POJO (Plain Old Java Object) to Kotlin's \emph{Data Classes}.
They all agreed that is a straightforward and simple migration.
However, beyond that finding, due to the diversity and complexity of the answers, we could not develop generalized conclusions about which functionalities.
%
We let this question open for future work.

%%%%%%%%%%%%%%
%% OLD RQ 4
%%****

\subsection{\rqproportion}
\label{sec:rq:proportion}

\begin{figure}
\captionsetup{justification=centering}
    \centering
 \begin{subfigure}[b]{0.15\textwidth}%%0.32
        \includegraphics[width=\textwidth]{lines_Passandroid.pdf}
        \caption{{\scriptsize PassAndroid}: Amount and proportion of Kotlin code increase.}
        \label{fig:linesPassandroid}
    \end{subfigure}
    \begin{subfigure}[b]{0.15\textwidth}
         \includegraphics[width=\textwidth]{lines_Photolinkviewer.pdf}
           \caption{
           %Photolinkviewer App:  Amount of Kotlin and Java code decrease, proportion of Kotlin code also decreases.
           {\scriptsize PhotoLinkViewer}:  Amount and proportion  of Kotlin code decrease.
           }
      \label{fig:linesPhotolinkviewer}
    \end{subfigure}
     \begin{subfigure}[b]{0.15\textwidth}
    \includegraphics[width=\textwidth]{lines_Daycounter.pdf}
        \caption{{\scriptsize DayCounter}: Amount of Kotlin code increase, but the proportion decreased. % due to the reintroduction of Java code.
        }
    \label{fig:linesDaycounter}
    \end{subfigure}

    \caption{Evolution of 3 apps not yet fully migrated. Axis X corresponds to commits, axis Y to sLOC.}
 
    \label{fig:evolutions_trends}
\end{figure}



\begin{table}[t]
\centering
\label{tab:summarybothlang}
 \begin{tabular}{|c |  r r r |r|  } \hline
Latest $c$ & Prop $\uparrow$ & Prop $\downarrow$&  Prop = & Total\\
 \cline{2-5}
 
versus& \multicolumn{4}{c|}{Amount Kotlin  $\uparrow$} \\
\cline{2-5}

\hline
 First  $c$  & 163 (76.17\%) & 35 (16.36\%) & 0 (0.00\%) & 198 (92.52\%)  \\
%Last  50\% & 148 (69.16\%) & 32 (14.95\%) & 0 (0.00\%) & 180 (84.12\%)  \\
%Last 30\%& 149 (69.63\%) & 22 (10.28\%) & 0 (0.00\%) & 171 (79.91\%)  \\
%Last  20\% & 148 (69.16\%) & 15 (7.01\%) & 0 (0.00\%) & 163 (76.17\%)  \\
Recent $c$& 139 (64.95\%) & 13 (6.07\%) & 0 (0.00\%) & 152 (71.03\%)  \\
\hline
\hline
&  \multicolumn{4}{c|}{Amount Kotlin  $\downarrow$}\\
\cline{2-5}
%& Prop $\uparrow$ & Prop $\downarrow$&  Prop = & Total\\
\hline
 First $c$ & 1 (0.47\%) & 4 (1.87\%) & 0 (0.00\%) & 5 (2.34\%)  \\
%Last  50\% & 5 (2.34\%) & 5 (2.34\%) & 0 (0.00\%) & 10 (4.67\%)  \\
%Last  30\% & 5 (2.34\%) & 12 (5.61\%) & 0 (0.00\%) & 17 (7.94\%)  \\
%Last   20\% & 3 (1.40\%) & 17 (7.94\%) & 0 (0.00\%) & 20 (9.35\%)  \\
Recent $c$& 4 (1.87\%) & 22 (10.28\%) & 0 (0.00\%) & 26 (12.15\%)  \\
\hline
\hline
 &  \multicolumn{4}{c|}{Amount Kotlin =}  \\
\cline{2-5}
%& Prop $\uparrow$ & Prop $\downarrow$&  Prop = & Total\\
\hline
 First $c$ & 0 (0.00\%) & 6 (2.80\%) & 5 (2.34\%) & 11 (5.14\%)  \\
%Last    50\% & 4 (1.87\%) & 12 (5.61\%) & 8 (3.74\%) & 24 (11.21\%)  \\
%Last    30\% & 4 (1.87\%) & 13 (6.07\%) & 9 (4.21\%) & 26 (12.15\%)  \\
%Last    20\% & 4 (1.87\%) & 15 (7.01\%) & 12 (5.61\%) & 31 (14.49\%)  \\
Recent $c$& 5 (2.34\%) & 16 (7.48\%) & 15 (7.01\%) & 36 (16.82\%)  \\
 \hline
 \end{tabular}
\caption{The table groups the apps that increase ($\uparrow$), decrease ($\downarrow$) or equality ($=$):
{\it a)} the amount of Kotlin code, 
{\it b)} the proportion of Kotlin code.
For each application, we made two comparisons:
{\it 1)} the latest commit and the first commit that  introduces Kotlin, 
{\it 2)} the latest commit and a \emph{recent} commit with Kotlin. (The letter $c$ means `commit').
}

\label{tab:result}
\end{table}

We now study the evolution of the applications that have not been completely migrated to Kotlin yet (i.e., set  \emph{\colanguage}).
As reported in Section \ref{sec:res:langusedhistory}, the number of such applications is 214 (out of 374). 

We response this research question via two studies.
First, we present a quantitative study based on the evolution of the amount of code computed using \miga.
Then, we present a qualitative study based on the interviews we made to developers.


\subsubsection{Evolution of Amount of Java and Kotlin Code}
Table \ref{tab:result}  shows the results: each cell corresponds to the number of applications having the amount and proportion of Kotlin code increased~($\uparrow$), decreased~($\downarrow$) and equals~($=$) w.r.t. a previous commit done in the past.
We now discuss three cases of code evolution.

\todo{move to partially}

\paragraph{Case 1: Amount of Kotlin Code Increase}
\label{sec:amountincrease}

Let's focus on the first section of the Table \ref{tab:result} (Amount  Kotlin~$\uparrow$).
For the 92.52\% of the applications, the latest commits has more Kotlin code that the first commit that introduced code.
Figure \ref{fig:linesPassandroid}  shows the evolution of the amount of Java and Koltin code from one of those apps.
However, the number of apps that have more Kotlin code in the latest w.r.t a \emph{recent commit} (see definition in \ref{sec:method:amountkotlin}) is lower:  71\%.
Figure \ref{fig:linesPhotolinkviewer} shows the evolution of code from one apps.

Moreover, the 76.17\% of the apps (163 apps) have a larger proportion of code w.r.t the first version.
The percentage is lower when we compare the proportion of the last commit and the \emph{recent} commit: 64.95\% (139 apps).
We believe that those applications are potentially in process of being migrated. 
That situation  could eventually lead into the total migration of the Java code to Kotlin.
On the contrary, for 16.36\% of the apps (35 apps) proportion of Kotlin code has decreased (column Prop $\downarrow$).
This means that those apps have received more Java code than Kotlin.
Figure \ref{fig:linesDaycounter} shows one of those apps: after a total migration to Kotlin, Java code was reintroduced.


\paragraph{Case 2: Amount of Kotlin code decreases}
\label{sec:amountdecreate}
The second section from Table \ref{tab:result} (Amount Kotlin $\downarrow$) shows that few apps (5, i.e. 2.34\%) have less Kotlin code than the initial commit with Kotlin.
However, the 12\% of the apps (26) have less code than their \emph{recent commit}.
We suspect that this reduction is consequence of code refactoring.


\paragraph{Case 3: Amount of Kotlin code remains constant}
\label{sec:amountequals}
Last section from Table \ref{tab:result} (Amount Kotlin~$=$) shows that the 16.82\% of the applications (36) have the same amount of Kotlin code w.r.t the \emph{recent commit} (last row). 
For the 7.48\% (column 3, Prop~$\downarrow$) of them, new Java code is introduced in the latest commits, guiding the evolution of such apps. 


\begin{tcolorbox}
%The 76.17\% 
The 64.95\% of the applications having both Kotlin and Java in their latest version evolves increasing both the amount and the proportion of Kotlin code. 
We conjecture that, if those applications continue evolving following that evolution trend, in the near future they could be completely migrated to Kotlin.
\end{tcolorbox}

%%%%%%%%%%% END OLD RQ 4 Mining analysis


%%% OLD RQ 1 and 2********


\subsection{\rqappsmigrated{}}
\todo{fully or partially}


\todo{Two subsection: Fully migrated and partially migrated, with the content of RQ4}
To respond this research question, we first analyze the languages used:
\begin{inparaenum}[\it a)]
\item at the beginning of the development, 
\item during the development of an application, and finally
\item  in the last commit.
\end{inparaenum}
%
The fully migrated applications detected in this research question, as well those not fully migrated, will be studied in the next research questions.

\subsubsection{Initial Programming Language}
\label{sec:res:initiallang}


We analyze 374 Android applications from \dataset{} dataset.
By construction, all applications from there have, at least, one file with Kotlin code and, eventually, one file with Java code.

Table \ref{tab:lang} presents the results. 
In total, 65  apps were initially written only using Kotlin code.\footnote{\label{lab:javatest}
From the 65 apps, 21 have Java code corresponding to test cases  named `ExampleUnitTest.java' and `ApplicationTest.java' automatically generated by IDEs such as Android Studio when a project is created. Those tests have not been modified after the creation. For this reason, we ignore them.}
%One example of such applications is Kingfish, which initial commit\footnote{Initial commit of app Kingfish: 5c448ed6a2805a23b002c8e5e156fb43ca1d3cf7.} has a Kotlin file and two automatically generated Java test files named `ExampleUnitTest.java' and  `ApplicationTest.java'.  Note that developers from those projects did not modify those tests during the evolution of the apps. 
%
From the remaining 309 apps, 269 started being developed just using Java code (i.e., Java code was used before  Kotlin code),
and 40 apps have been developed using both Kotlin and Java since the first version pushed to their respective version control systems.


\begin{table}[t]
\centering
 \begin{tabular}{|l||  r | r |   } 
 \hline
Language& \multicolumn{2}{c|}{Number  Applications having:} \\
\cline{2-3}
& Initial  version  & Latest version  \\
\hline
Java &269&4\\
\hline
Kotlin &65&156\\%%60+96
\hline
Both &40&214\\
\hline
\hline
Total& \multicolumn{2}{c|}{374}\\
 \hline
 \end{tabular}
\caption{Number of apps having Java and Kotlin version in their first and last versions.\todo{remove}}
\label{tab:lang}
\end{table}

\subsubsection{Languages used along the history}
\label{sec:res:langusedhistory}

Our dataset has in total 60 apps (16\%) completely written in Kotlin along their history.\footnote{
Between the 60 apps, there are 16 that introduce (but not evolve) the automatically generated tests mentioned in footnote \ref{lab:javatest}.}
%
The rest, 314 apps  (84\%), evolves by adding and modifying Kotlin and Java code (at the same or different time).
%%%Long version commented
\begin{comment}

In total, 44 apps have been developed using just Kotlin code along their complete history, without having a single line of Java code. 
Moreover, we found that 16 additional apps that were written in Kotlin and have one or more commits including the mentioned  test files automatically written in Java (Section \ref{sec:res:initiallang}) and no more Java code in any commit from their history.\footnote{In Section \ref{sec:res:initiallang} we report 21 apps that introduce automated generated tests in their first commits, and in Section \ref{sec:res:langusedhistory}  we report 16 apps that  introduce those tests in any part of their history, not only at the beginning. This means that 5 apps (21 - 16) add one or more Java files (different from those testing files) during their evolution.} 
Consequently, by ignoring such files and considering those apps as Pure Kotlin, our dataset has in total 60 (16\%) apps completely written in Kotlin.
%
The rest, 314 apps  (84\%) evolve by adding and modifying Kotlin and Java code (at the same or different time).
\end{comment}

\newcommand{\migrapps}{{Migrated-Apps-j2k}}
\newcommand{\colanguage}{{Mix-Java-Kotlin Apps}}

\subsubsection{Languages used in the last version}
\label{sec:res:langusedlastversion}

We now focus on the remaining 314 apps (i.e., 374 - 60) which have Java and, eventually, Kotlin.
%
214 apps have both Kotlin and Java in the latest commit. 
Those apps form the set named \emph{\colanguage{}}.
%
%
Now, let's inspect the remaining 100 apps (314 - 214).
In this paper we are particularly interested in 86 of them, which have been initially written exclusively on Java and \emph{fully} migrated to Kotlin. Those apps from the set named \emph{\migrapps}.

We now describe the other 14 apps (100 - 86), which we do not study in this paper.
First, there are 10 apps that have  initial commits written in Koltin,  and Java code was introduced and subsequently removed.
\begin{comment}
\begin{inparaenum}[\it a)]
\item  5 apps have been initially written using both Kotlin and Java.
\item 5 apps have only Kotlin code in their initial version, and Java code was introduced and subsequently removed.
\end{inparaenum}
\end{comment}
Then, the remaining 4 applications had Kotlin code but it was removed, remaining only Java code in their latest versions.
\begin{comment}
%({Material-flashlight})
For one of them, their developers have started written it in Kotlin and, at the middle of its history, the developers completely migrated to Java.
The others 3 app have been initially developed in Java, then the developers added some functionalities on Kotlin, which were finally removed, remaining, again, only Java code.
\end{comment}
We interviewed one developer that introduced Kotlin on one of those apps.
He told us: 
\quotes{I tried to migrate [...] but other contributors just find it complicated to incorporate two languages style in a single project and, eventually reverted the project to some time before}.


\begin{tcolorbox}
86 Android applications (out of 314) were completely migrated from Java to Kotlin.
Then, 
214 apps were initially written in Java and they have been partially migrated.
\end{tcolorbox}

%%%Removed, not interesting here%%
\begin{comment}
\subsubsection{Moment of First use of Kotlin}
\label{sec:res:kotlinfirstintroduction}


\begin{figure}[t]
\centering
%\begin{subfigure}
 \includegraphics[scale=0.5]{histogram_introduction_kotlin_percentage_374.pdf}
  \caption{Distribution of Introduction moments of  Kotlin code for all applications (374). Zero value means the beginning of the history, 1 means the end. Consequently, the histogram shows that  more than 110 apps have an introduction moment near to zero, which means that Kotlin is used for a first time at the beginning of the project history.}
 \label{fig:hist_kotlin_intro_all}
%\end{subfigure}
\end{figure}

Histogram \ref{fig:hist_kotlin_intro_all} shows the distribution of the \emph{Introduction moment}  of Kotlin code (as explained in Section \ref{sec:method:intromoment}).
%The \emph{introduction moment} is  measure that divides the commit number (following a chronologically order) that introduces Kotlin for the first time into an app $A$   by the total number of commits from $A$.
%
The mean and the median are both ~0.40, which means that Kotlin is introduced, on average, after the first 40 \% of the commits of the application.
%For X applications the introduction  moment  is 0, which means that Kotlin is used from scratch.
We found that 62  apps have a later introduction greater than 0.8, which mean that Kotlin was introduced at the end of the application history. 

%%%Removed, not interesting here%%
\end{comment}


%'project': 'Voice', 'range': 2017,


%allInitsKotlin: len: 374 min: 0.0 max: 0.9837745516652434 mean: 0.40154541258002113  median: 0.4047670695908008 standdesv: 0.3387344410657114 
%late introduction  62: ['zandy', 'k-9', 'DnestrCinema', 'DocScan', 'SimpleHTMLTesterAndroid', 'StreetComplete', 'SystemUITuner2', 'insapp-android', 'madrid-pollution-android-app', 'GeoQuake', 'dlt', 'YoNoDesperdicio', 'trolley-tracker-android-client', 'Botanist', 'spaRSS-DecSync', 'Alarmio', 'Screenshot-Sharer', 'MensaUPB', 'GrowTracker-Android', 'uhabits', 'kiwix-android', 'MGit', 'youreawinner', 'FRCAndroidWidget', 'ComputingTutorAndroidApp', 'SimpleBitcoinWidget', 'easysshfs', 'FAST', 'penn-mobile-android', 'Geocaching4Locus', 'SimpleMarkdown', 'Retribution', 'PosTrainer', 'Status', 'CCIP-Android', 'UnitConverterUltimate', 'rectball', 'materialistic', 'PushNotificationTester_App', 'SoundWaves', 'Lawnchair', 'Sofia-Traffic', 'EH17Fahrplan', 'cpustats', 'rxbsuir', 'ShutUp', 'ContractionTimer', 'LocalStorage', 'buntata-app', 'unitconverter-android', 'BibleQuote-for-Android', 'Umweltzone', 'android-app', 'commcare-android', 'NHentai-android', 'KonashiInspectorForAndroid', 'opacclient', 'speedofsound', 'mtmods4android', 'AutoStopRace', 'NCBSinfo', 'Checklist']



%OpenLaunc migrates one component and the rolback.
%sexytopo introduces one file written in Kotlin and then it is removed.


\subsection{\rqmigrationdone}
\label{sec:res:migration}

We now focus on the 86 apps from set  \emph{\migrapps} that started being developed using Java and were subsequently completely migrated to Kotlin.

To respond this research question, 
we do two experiments.
First, we study the \emph{migration intervals} to characterize the duration of the migrations in terms of commits.
%
Then, we analyze commits inside the migration interval to detect those that could have migrated code. 

\subsubsection{Migration Intervals}

\todo{Summarize and move to RQ 1}

Histogram \ref{fig:kotlin_migration_duration} shows the distribution of the length the \emph{migration intervals}\footnote{For ease of reading, we removed from the Histogram \ref{fig:kotlin_migration_duration} two \emph{outliers}: Rocket.Chat.Android which  interval has 1988 commits  and Voice with 2018.}
and Histogram \ref{fig:kotlin_migration_duration_normalized} shows the distribution of  their lengths normalized by the total number of commits from the application.
This normalization has as goal to observe the duration of the migration w.r.t the complete history of one application.
%For example, the interval of the previously mentioned Red app covers the 37\% of its history (i.e., the proportion is 0.37 =  187 / 502, where 502 is the total number of  commits).
%
From them, we identified two main migration strategies. Those are:

\begin{figure}[t]
\captionsetup{justification=centering}
    \centering
 \begin{subfigure}[b]{0.15\textwidth}%0.42
        \includegraphics[width=\textwidth]{lines_Simplebitcoinwidget.pdf}
        %%simple
        \caption{SBitcoinWidget: $mi$ = 1 commit}
        \label{fig:linesSimplebitcoinwidget}
    \end{subfigure}
    \begin{subfigure}[b]{0.15\textwidth}
         \includegraphics[width=\textwidth]{lines_Localstorage.pdf}
           \caption{Localstorage: $mi$ = 4 commits}
      \label{fig:linesLocalstorage}
    \end{subfigure}
    \begin{comment}
     \begin{subfigure}[b]{0.15\textwidth}
 \includegraphics[width=\textwidth]{lines_Uncmorfi.pdf}
  \caption{UNCmorfi: $mi$ =  28   commits \todo{to remove it}}
 \label{fig:lines-UNCmorfi}
    \end{subfigure} 
      \end{comment}
     \begin{subfigure}[b]{0.15\textwidth}
    \includegraphics[width=\textwidth]{lines_Red.pdf}
        \caption{Red: $mi$ = 188   commits}
    \label{fig:linesRed}
    \end{subfigure}
    \caption{Evolution of Kotlin and Java code for 3 applications having  migration intervals  ($mi$) with different lengths. Axis X corresponds to commits, axis Y to sLOC.}
    \label{fig:examples_mig_interval}
\end{figure}

\begin{figure}[t]

\begin{subfigure}{0.48\linewidth}
 \includegraphics[scale=0.3]{histogram_range_84.pdf}
  \caption{Lengths of Migration Intervals (in number of commits)}
 \label{fig:kotlin_migration_duration}
\end{subfigure}
\hfil
%\begin{figure}[t!]
\begin{subfigure}{0.48\linewidth}
 \includegraphics[scale=0.3]{histogram_range_Percentage_84.pdf}
  \caption{Lengths of Migration Intervals divided by number of commits.\todo{remove/appendix}}
 \label{fig:kotlin_migration_duration_normalized}
\end{subfigure}
\caption{Distribution of the migration interval  lengths corresponding to the 86 apps from set  \emph{\migrapps}.}
\label{fig:kotlin_migration_duration_main}
\end{figure}


%rangeZero 29: ['SimpleBitcoinWidget', '2chmatome', 'PosTrainer', 'JanYoShare', 'FRCAndroidWidget', 'KonashiInspectorForAndroid', 'NCBSinfo', 'kmn_bot-tool', 'SimpleHTMLTesterAndroid', 'easysshfs', 'VoiceMessageBoard', 'Android-SearchView-Demo', 'home-button', 'stew', 'Status-Bar-Tachometer', 'vanilla-music-metadata-fetch', 'AnkiEditor', 'Stratum0Widget', 'MockAppDemo', 'Screenshot-Sharer', 'SunWidget', 'SystemUITunerRedesign', 'speedofsound', 'Simple-Thank-You', 'baresip-studio', 'Simple-Flashlight', 'SELinuxModeChanger', 'tincapp', 'youreawinner']

\paragraph{One-Step migration}
%%33.7\%

%% Clarification: 31 are the 29 with 1 + 2 apps with negative 33.7\%
In total, 31  projects (out of 86 apps from \emph{\migrapps}, that is, the 36\%)  have migration interval lengths equals to 1, which means that they were migrated in \emph{exactly} one commit.
Those commits remove all Java files and introduce the Kotlin code. 
One of those applications is `SimpleBitcoinWidget', which code  evolution is presented in Figure \ref{fig:linesSimplebitcoinwidget}. 
%: in one commit the complete Java code is replaced by Kotlin code.
%\footnote{Commit id: 417e2e86c8d7c72b77443b273b36b885276d285f from app SimpleBitcoinWidget.} 

Eight developers that replied to our interview request had migrated their apps in one single commits. 
Half of them confirmed us that they migrated the code using the converter tool provided by the IDE Android Studio.
%
%The other ones migrated \emph{by hand}.
%One developer told us about that: \quotes{The app is not a large project so migrating from Java was not a big deal}.

%Another one told us that, beyond migrating its app in One-step: \quotes{I converted the entire project class by class, over the course of weeks}.


%project': 'red', 'range': 187, 'rangepercentage': 0.37250996015936255}

%%Not necessary to mention
\begin{comment}
Additionally, we found  two applications which migration intervals are \emph{negative}.
However, the migration were done quite similarly to the previous 29 apps: 
one commit first removes all Java code, and then, in the next commit, the Kotlin code is introduced.
%rangeNegative 2: ['remindermail', 'DeuFeiTage']
\end{comment}

\begin{tcolorbox}
%The 33.7\%
The 36\% of the migrated applications were completely migrated  in one step (i.e one single commit).
\end{tcolorbox}

%%% Escalonadas

\paragraph{Staggered migration}

For the rest of the 55 applications (out of 86,  i.e., that is the 64\%), their \emph{migration interval lengths} are greater than one commit.
There, the migrations were gradually done: some version have both Java and Kotlin code.
For example, LocalStorage and Red apps, which code evolution trends are presented in Figures \ref{fig:linesLocalstorage}  and \ref{fig:linesRed}, present intervals with length 4 and 188 commits, respectively.
%
Histogram \ref{fig:kotlin_migration_duration} shows the distribution of the migration intervals for all migrated applications.
Even discarding those 31 migrated in one-step, we observe that most apps were fully migrated in intervals smaller than 50 commits.
However, there are apps with larger intervals. 
For example, that one from SimpleGalery has 266 commits.

We then normalized the intervals. 
As shown by the Histogram \ref{fig:kotlin_migration_duration_normalized}, for most of the apps, the normalized interval's lengths are near to zero, which means that their migrations happened during a short period during their history. 
Coming back to SimpleGalery app, even its interval is one of the largest we found, it's relative small compared to its large complete history: the proportion is 0.093.
%There are some applications with short migration intervals, but they cover a larger portion of history.
%For example, the migration interval of Unstoppable app has 6 commits, and the total number of commits from its history is 23, thus the proportion is 0.26.
%On the contrary, other apps have larger intervals but smaller proportions. For example, SimpleGalery has an interval of 266 and the proportion is 0.093. 


%rangePositive 55: ['red-moon', 'LocalStorage', 'slounik', 'red', 'Simple-Calendar', 'coins-android', 'DmsExplorer', 'davdroid', 'Wiktor-Navigator', 'SheepsGoHome', 'whitakers-words-android', 'Cineaste', 'Voice', 'Podcasts-RAC1-Android', 'ShowsRage', 'toto-anticipation', 'icsdroid', 'Geocaching4Locus', 'AndroidCupsPrint', 'Fractals', 'bo-android', 'PlanningPoker', 'Simple-Notes', 'ScreenStream', 'Msync', 'cryptogram', 'android-torchlight', 'android-app', 'Rocket.Chat.Android', '2050', 'Electric-Fields', 'wulkanowy', 'StockTicker', 'Simple-Draw', 'PackageTracker', 'progressbars', 'hand-and-foot-scores', 'Simple-App-Launcher', 'UNCmorfi', 'Monger-Android', 'Simple-File-Manager', 'show-java', 'Simple-Music-Player', 'unstoppable', 'Simple-Gallery', 'ValenBisi', 'aaf-easydiary', 'Simple-Camera', 'si_counter', 'GPS-Texter', 'VNDB-Android', 'BatteryChargeLimit', 'NightLight', 'apolline-android', 'LanbahnPanel']

\begin{comment}
Figure \ref{fig:scatter_range} shows the relation between the \emph{migration interval}  and that normalized value.
At the left-bottom of the plot  where both proportion of migration and length trend to zero,  are located most of the applications, including the 29 mentioned applications with interval equals to zero. 
This means that migrations happens in few commits consecutive commits inside a large history in terms of number of commits. 
There are some application with short migration intervals, but they covers a larger portion of history, e.g., `Unstoppable' app has 6 commits in its migration interval but the total number of commit is 23, thus the proportion is 0.26.
On the contrary, other projects, such as  SimpleGalery, have larger intervals but the its proportion is lower (for SimpleGalery those values are  266 and 0.093, resp.).


 \begin{figure}[t]
\centering
    \includegraphics[width=0.75\textwidth]{scatter_range_84.pdf}
       \caption{Length (axis X) and proportion (axis Y) of the Migration interval of each migrated application.}
    \label{fig:scatter_range}
 \end{figure}

\end{comment}

%%%%%

\begin{tcolorbox}
Most of the  apps were completely migrated from Java to Kotlin in few commits and the migration interval represents less than the 10\% of the complete history of those applications.
\end{tcolorbox}


%Small: (32) ['SimpleBitcoinWidget', 'remindermail', '2chmatome', 'PosTrainer', 'JanYoShare', 'FRCAndroidWidget', 'KonashiInspectorForAndroid', 'NCBSinfo', 'kmn_bot-tool', 'SimpleHTMLTesterAndroid', 'AndroidCupsPrint', 'easysshfs', 'VoiceMessageBoard', 'DeuFeiTage', 'Android-SearchView-Demo', 'home-button', 'stew', 'Status-Bar-Tachometer', 'vanilla-music-metadata-fetch', 'AnkiEditor', 'Stratum0Widget', 'MockAppDemo', 'Screenshot-Sharer', 'SunWidget', 'SystemUITunerRedesign', 'speedofsound', 'Simple-Thank-You', 'baresip-studio', 'Simple-Flashlight', 'SELinuxModeChanger', 'tincapp', 'youreawinner'] 

%Si_counter special case few Java code

%Davdroid most migration in few

%Rocket.Chat.Android remains two dummies test until 9f39b8645fb50124f6656fe3f334ad4e80aa5b45.
%%last with Java 3ee6de980dd77680c896fe6954c5f817540ec340
%%5509fb5b16fea584f9dbdd985834b9ec9efcf922 remove all Java

\begin{comment}
A particular case is Rocket.Chat.Android, which interval is an \emph{outlier}. 
Their developers stared developing that application in Java, arriving to version  with 20K lines of Java code. 
Later, In the commit, they introduced Kotlin language and during X commits the amount of Kotlin commit moderaly increases, remaining the amount of Java code almost constant. However, in one particular commit\footnote{5509fb5b16fea584f9dbdd985834b9ec9efcf922 } both Java and Kotlin are removed, and the next step the app is rewritten from scracht using mainly Kotlin. 
Few Java code is introduced in this new version, which is gradually removed until the app only contain Kotlin code.
\end{comment}

%%%%%%%%%%%%%%%%
%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsubsection{Detection of commits that Migrate Java to Kotlin}
\label{sec:res:migtypes}

\todo{Remove?}
We now focus on the detection of commits that migrates code from the 86 completely migrated apps. %from Java to Kotlin.
%
We aim to detect the three types of migration commits presented in  Section \ref{sec:commit_migration}. 

\paragraph{Migrations of Files}
\label{sec:res:migrationfiles}

\begin{figure}[t]
%\centering
\begin{subfigure}{0.45\linewidth}% 0.45
 \includegraphics[scale=0.30]{histogram_migrationCommits_84.pdf} % 0.40
  \caption{Distribution of  the number of File-migration commits.}
 \label{fig:kotlin_migration_commits}
\end{subfigure}
\hfil
%\begin{figure}[t!]
\begin{subfigure}{0.45\linewidth}
 \includegraphics[scale=0.30]{histogram_migrationCommits_proportion_84.pdf}
  \caption{Distribution of Proportion of File-migration commits. 
  }
 \label{fig:kotlin_migration_commits_proportion}
\end{subfigure}
\caption{Distribution of the number and proportion of  commits that migrate Files from Java to Kotlin per application.
}
 \label{fig:kotlin_migration_commits_all}
\end{figure}
%computeMigrationFilesAndMigInterval.py


The histogram \ref{fig:kotlin_migration_commits}  shows the distribution of the number of commits that migrate Files (Section \ref{sec:file_migration}) from the set  \emph{\migrapps} (in total 86 apps).
It shows that the majority of the applications (i.e.~$>$50) have few commits that migrate files: from 1 to 5. 
%For example, on of those apps is FRCAndroidWidget, which has one commit\footnote{Commit id: 5d3a0d5a3158b9b463a00ff347f1d5d0398cfa67 from app FRCAndroidWidget} that migrates all the 43 files written in Java to Kotlin. 
%There, its migration interval is 1.
%
On average the number of migration commits is  8.25  and the median is  2.
%The project with greatest number of migration commits is  DmsExplore. %, with 71 of such commits done in a migration interval of 274 (proportion of 25.8\%).

The histogram  \ref{fig:kotlin_migration_commits_proportion} shows the proportion of File migration commits divided by the lengths of the migration intervals.
In total, for 35 apps the proportion is 1 (the bar at the rightmost), meaning that \emph{every} commit in the migration interval migrates, at least, one file from Java to Kotlin.
%commits that migrate files cover the whole migration interval. 
%One of those apps is the previously mentioned FRCAndroidWidget.
%%Commented to reduce the length
\begin{comment}
%Another one, named Cineaste, has a migration interval of 11: on each commit done on that interval, at least one file is migrated to Kotlin, having some commits that migrates up to 12 files.
\end{comment}
\begin{comment}
%%Reduced  
Another app, named UNCmorfi which code evolution is presented in Figure \ref{fig:lines-UNCmorfi}, has an interval with 28 commits,  27  of them commits migrate a single file. 
The proportion of migration commits is  0.96 (96\%,  27/28). 
Note that those commits eventually also modify already written code. 
For instance, commit e446dd\footnote{Commit id: e446dd6e7f4311f9d85e8e6c4c16b58c193b4edd from app UNCmorfi.} modifies Kotlin code from a file (MenuFragment.kt) that was migrated from Java to Kotlin ten commits before.\footnote{Commit id: 5a2111e9b45552f3aaa7850518734a623eebe6ac from app UNCmorfi.}
\end{comment}
On the contrary, the proportion of commits that migrate files inside the migration interval is lower for other apps.
For instance, the application GPS-Texter has a migration interval of 93 commits and only 15 of them (16\%)  migrate code. 
Those commits are alternated with others that are not related to such type of migration.
%, e.g. there are commits such as c82a1d\footnote{commit id: c82a1d5221f27977a322da47dfebda81a03a49d8. Commit message: ``Refactoring: Changed layout names.''} that exclusively updates 7 existing Java files.
%\new{The evolution of those applications mixes both 
%\begin{inparaenum}[\it a)]
%\item maintenance of Java code,
%\item migration of Java code to Kotlin.
%\end{inparaenum}
% }

\begin{tcolorbox}
We identified two groups of apps, based on their  migration interval lengths:
\begin{inparaenum}[\it 1)]
\item apps which most of the commits from their intervals migrate Files, 
%(e.g., FRCAndroidWidget, UNCmorfi);
\item apps which migrations of files are \emph{mixed} with  maintenance activities such as refactoring of Java code. %(e.g., GPS-Texter).
\end{inparaenum}
\end{tcolorbox}

We suspect that file-level migration is done using the auto-converter tool provided by IDEs, which allows developer to migrate a single Java file to Kotlin.

 
%Project DmsExplorer: 71 275 0.258182

%%MigJvToKt: len: 84 min: 1 max: 71 mean: 8.25  median: 2.0 
%MigJv2Kt (proportion): len: 84 min: 0.0029498525073746312 max: 1.0 mean: 0.5681630774635431  median: 0.6666666666666666 

%MigJvToKt AR: len: 84 min: 0 max: 9 mean: 0.8214285714285714  median: 0.0 
%MigJv2Kt AR (proportion): len: 84 min: 0.0 max: 1.0 mean: 0.13478755306942516  median: 0.0 

%MigJvToKt MIG: len: 84 min: 0 max: 71 mean: 7.988095238095238  median: 2.0 
%MigJv2Kt MIG (proportion): len: 84 min: 0.0 max: 1.0 mean: 0.5593078803114628  median: 0.6333333333333333 

\begin{comment}
\begin{figure}[t]
\centering
 \includegraphics[scale=0.45]{scatter_migcommit_vs_miginterval_84.pdf}
  \caption{}
 \label{fig:scatter_migcomit_interval}
\end{figure}
\end{comment}


%\inred{IntersectionL plot distribution of size according to the proportion.}
%Figure \ref{fig:scatter_migcomit_interval}

%%%%%%%%%%%

\paragraph{Fine-grained code migrations}
\label{sec:res:methodlevelmigration}

\todo{Remove?}
We found 11 projects (out of 86 fully migrated projects) that contain, at least, one commit that removes one method from a Java file and adds a method in a Kotlin file (Section \ref{sec:method_migration}).
The average and median number of Method-level migration commits on those 11 projects are 2.36 and 2 respectively.
%Stats project Mig2Mig : len: 11 min: 1 max: 6 mean: 2.3636363636363638  median: 2 standdesv: 1.3666633071248098 
Moreover, we found 13 projects having, at least one commit that removes methods from Java files and, at the same time, adds a new Kotlin file (Section \ref{sec:update_insert_migration}). 
The average and median number of such commits on the 13 projects are 2.3  and  2,  respectively.
%len: 13 min: 1 max: 5 mean: 2.3076923076923075  median: 2 standdesv: 1.3234346564680963

%The commits that present this type of migration shows that there are developers do migration \emph{by hand} because the IDE does only provide (up to now) a tool that converts Java file to  Kotlin file.

We suspect that commits of this type of migration correspond to  migrations written \emph{by hand} because the IDE does only provide (up to now) a tool that converts Java file to Kotlin file.

\begin{tcolorbox}
The migration of Java to Kotlin is mainly done through File-level migrations.
Those convert one Java file to Kotlin and preserve the file names (excepting the file extension).
\end{tcolorbox}

%%%%%% Commented 
\begin{comment}

\newcommand{\lstbg}[3][0pt]{{\fboxsep#1\colorbox{#2}{\strut #3}}}
\lstdefinelanguage{diff}{
 % basicstyle=\ttfamily\small,
   basicstyle=\ttfamily\tiny,
  morecomment=[f][\lstbg{red!20}]-,
  morecomment=[f][\lstbg{green!20}]+,
  morecomment=[f][\textit]{@@},
}

\begin{figure}[t]
\caption{Commit that migrates one method from Java (left) to Kotlin (right)}
\begin{subfigure}{.20\textwidth}
\begin{lstlisting}[language=diff]
diff --git a/app/.../Preview.java 
b/app/.../Preview.java
index df8bfee..a563fb9 100644
@@ -305,20 +305,6 @@
 .....
-  private int getMaxVideoResolution() {
-      final int maxRes = 
-     mConfig.getMaxVideoResolution();
-      switch (maxRes) {
-          case 0:
-              return 400000;
-          case 1:
-              return 1000000;
-          case 2:
-              return 2100000;
-          default:
-              return 0;
-      }
-  }
...
}
\end{lstlisting}
%\caption{Java version}
\end{subfigure}
\begin{subfigure}{.20\textwidth}
\begin{lstlisting}[ language=diff]
diff --git a/app/.../Utils.kt 
b/app/.../Utils.kt
index 436d973..24797c4 100644
@@ -150,5 +150,21 @@
 ...... 
+
+     fun getMaxVideoResolution(config: Config): Int {
+         return 
+  when (config.maxVideoResolution) {
+             0 -> 400000
+             1 -> 1000000
+             2 -> 2100000
+             else -> 0
+         }
+     }
  }
 }
\end{lstlisting}
%\caption{Kotlin version}
\end{subfigure}
\label{fig:method_migration}
\end{figure}


Figure \ref{fig:method_migration}  shows as example one of such commits, found in app Simple-Camera.\footnote{Commit: e8cb8d14648a1f8472c266001db0233d69258eeb from app Simple-Camera.}
The commit removes the method named `getMaxVideoResolution'  which contains a Switch-Case statement in its body.
At the same time, the commit adds into an existing Kotlin file (`Utils.kt') a new method also called `getMaxVideoResolution' containing in its body a `When' statement, which is the Kotlin version of the Java Switch-Case instruction.

\end{comment}

\begin{comment}
\begin{tcolorbox}
The file-level  commit migration is much frequent than the method-level commit migration.
However, it still contributes to the migration  from Java to Kotlin of 13 apps.
\end{tcolorbox}
\end{comment}

%Project with method mig Java to Kotlin File Insert 13: dict_keys(['red', 'Simple-Calendar', 'coins-android', 'Voice', 'Podcasts-RAC1-Android', 'Simple-Notes', 'Rocket.Chat.Android', 'wulkanowy', 'Simple-File-Manager', 'Simple-Music-Player', 'Simple-Gallery', 'aaf-easydiary', 'apolline-android']) 
%All with method migration 16: {'Simple-Gallery', 'aaf-easydiary', 'wulkanowy', 'Simple-Camera', 'PackageTracker', 'Simple-Calendar', 'red', 'Simple-Notes', 'Podcasts-RAC1-Android', 'Simple-Music-Player', 'ShowsRage', 'apolline-android', 'coins-android', 'Simple-File-Manager', 'Rocket.Chat.Android', 'Voice'}


%%%%%%%%%%
%%%%%% RQ 
%%%%%%%%%%%



\section{Methodology}
\label{sec:methodology}

To respond the research questions, in this section we first present a tool, named \miga{}, that analyzes repositories of applications.
Then, we explain how we used it to respond the research questions.
Finally, we present the methodology we applied to carry out a survey which consisted on interviews with developers that migrated code to Kotlin.


\subsection{Methodology applied for analyzing commits}

To detect commits that migrate code, we build a tool called \miga{}.
%
It allows researchers to study the evolution of software applications i.e., the changes done over an application along its history.
In particular, \miga{} focuses on analyzing applications that, during their evolution, have been migrated to one programming language to another (or others).
%
In this section we present \miga{} and we describe how we process its output for responding the research questions.
%
\label{sec:migaframework}

\subsubsection
{Architecture and Implementation of \miga{}}
\label{sec:architecture}


\miga{} is built on top of Coming \cite{coming2019}, a framework for studying the evolution of applications.
\miga{} frameworks takes as input the location of a GIT repository on disk. 
It navigates each commit in chronological order, starting from the oldest one.
\miga{} extends Coming with new analyzers for studying the migration of applications. 
In particular, \miga{}: 
\begin{inparaenum}[\it a)]
\item {Analyzes added, removed and modified files from a commit},
\item {Analyzes commit messages},
\item {Compute lines of code of a version associated to a commit},
\item {Creates  Java ASTs for the Java files affected by a commit},
\item {Creates  Kotlin ASTs for the Kotlin files affected by a commit},
\item {Computes the differences introduced by a commit at the AST level},
\item {Detects commits that migrate code}.
As output, \miga{} generates a JSON file containing, for each commit, the information produced by each aforementioned analyzers.
%\item {Features extractor from Diff\inred{mention?}}
%\item {\inred{Pattern matching from Kotlin changes}},%AST diff
%\item {Pattern matching from Java changes (as explained in Section \ref{})}
\end{inparaenum}


\subsubsection{Lines of code per language}
For responding the first research question (RQ1), we analyze the output of \miga{} containing  per each commits $C$:
\begin{inparaenum}[\it a)]
\item the lines of source code (sLOC), and 
\item number of files 
\end{inparaenum} for each program language used on the version associated to $C$.


\subsubsection{Migration interval}
\label{sec:method:migrationinterval}

For responding the second research question (RQ2), 
we detect from the \miga's output, for each application:
\begin{inparaenum}[\it a)]
\item the first commit that uses Kotlin code, and
\item the last that  uses Java code.
\end{inparaenum} 
We call \emph{migration interval} to the portion of the application's history between those two commits.
%
The \emph{migration interval length} of a migrated application is the number of commits that happen between the two previously retrieved commits.
%
%$Migration\; Interval \; Length \;(MIL)  = Index_{last\_Java\_commit} - Index_{first\_Kotlin\_commit}$, 
%where $Index_{c}$ is the  $index$  of  commit $c$ from a list of commits chronologically sorted.

We further compute the \emph{proportion} of the migration interval w.r.t all the commits from the history of one application by dividing the length of the interval by the total number of commits.


\subsubsection{Detecting commits that migrate code}
\label{sec:commit_migration}

Moreover, also for responding research question 2, we implemented on \miga{} the detection of three types of commits that migrate code.
Those are:

\paragraph{File-level Migration}
\label{sec:file_migration}
\miga{} is able to detect \emph{File-level Migrations} commits.
They are commits that migrate code
by removing one Java file and adding a new Kotlin file.
\miga{} checks that  the names of those files are the same (excluding the file extension).

\paragraph{Finer-grained code level migration}
\label{sec:fine_grained_migration}
\label{sec:method_migration}

\miga{} is able to detect  commits that migrate code at a fine-grained level, which we named \emph{code-level migration}.
This type of migration happens when a developer migrates code by updating two (or more) existing files written in two different languages: 
Java code is removed and Kotlin code is added.
%
The current implementation of  \miga{}  is able of detecting on \emph{methods} level migrations.\footnote{
Even it is not covered in this paper, \miga{} can detect other code-level migrations, such as properties or blocks.}

For detecting method-level migration commits, \miga{} applies the following steps on each commit:
\begin{inparaenum}[\it a)]
\item verifies that 1 or more Java files \emph{and} 1 or more Kotlin files are updated by a commit $c$;
\item for each updated Java or Kotlin file $f$, \miga{} creates an AST (Abstract Syntax Tree) from $f$ and another from the previous version of $f$, i.e. $f_p$;
\item \miga{} computes the differences between the ASTs obtained from $f$ and  $f_p$, using GumTree algorithm \cite{Falleri:2014:FAS}. The output is a list of AST changes, where each change is an operation (Insert, Remove, Update and Move) done over an AST node;
\item \miga{} finds for INSERT operations that affect \emph{methods} in the $diff$ obtained from comparing Kotlin files, and DELETE operations that also affect methods in the other $diff$ obtained from comparing Java files.\footnote{By default, \miga{} does not match the method names, even it is possible to apply string matching heuristics.}
\end{inparaenum}

\paragraph{Update-Insert Migration}
\label{sec:update_insert_migration}
%
%
\miga{} can detect commits that removes a piece of code (e.g., method) from a file written in Java and, at the same time, adds a new file written written in Kotlin.
The implementation of this detector is based on the two previously described cases.

\paragraph{Other types of migrations}
Beyond those three types of commits that migrate code, there could be other that also migrate code.
%
We leave the discover and characterization of such types, and the detection of commit corresponding to the emerging types for future work. In Section \ref{sec:discussion} we discuss some future directions for discovering them.


\begin{comment}
\subsubsection{Commit composition}
\label{sec:method:proportion}
\todo{re-do?}
Moreover, in RQ 1, we study the composition of commits according to the program languages they affect.
The classify commits in 4 types \todo{weird sentence}: 
\begin{inparaenum}[\it 1)]
\item Pure-Java (commits that affect Java code but not Kotlin),
\item Pure-Kotlin (commits that affect Kotlin code but not Java),
\item Mix (commits that affects both Java and Kotlin code),
\item Other (commits that do not affect nether Java nor Kotlin code, e.g., XML files).
\end{inparaenum}
%By affected we mean that a commit adds, modifies or removes one or more files.
\todo{To me moved to Migration study and to compute it after Kotlin is introduced}
\end{comment}



\subsubsection{Amount and proportion of Kotlin code}
\label{sec:method:amountkotlin}

For responding the first  and fourth research questions, 
\miga{} computes, for each application $a$ and for each commit $c$, the number of Java and Kotlin lines of codes (sLOC) of the version of $a$ given by $c$.
It also computes the proportion of Kotlin code by dividing the sLOC of Kotlin per the total sLOC (i.e., Java sLOC + Kotlin sLOC).
Then, for each application, 
we compute the variation of both amount of sLOC and proportion between the latest commit done and an older commit.
In particular, we consider two older commits:
\begin{inparaenum}[\it 1)]
\item the \emph{first commit} that introduces Kotlin,  and
\item a ``\emph{recent commit}'', which corresponds to the commit done just before the latest 10\% of all commits.
\end{inparaenum}
For example, if one application has 110 commits and Kotlin was introduced in the commit \#10, we compare the amount/proportion of Kotlin code between the commit \#110 (latest) and: 
\begin{inparaenum}[\it a)]
\item the \emph{first commit}: \#10 (first Kotlin commit),
\item  the \emph{recent commit}: \#100 (beginning of the last 10\%  from all the Kotlin commits).
\end{inparaenum}


\subsection{Methodology applied for executing the survey}
\label{sec:methodology:survey}

For responding research questions 3, 4 and 5, we conducted a survey with developers.
In this section, we detail the characteristics and initial results of this survey.

\subsubsection{Survey purpose}

We carry out a survey with the main goal of collecting information about the migration of Java code to Kotlin in the context of Android development.
Our survey is explanatory~\cite{experimentationSE2012}: we try to explain why developers migrated their applications. 
The survey follows the format of interviews via email and aims at gathering both qualitative and quantitative data.

We initially asked developers a single question via email:
\quotes{Why did you migrate code from Java to Kotlin?}.
Then, once we received an answer from them, we further asked new questions according to their replies.
For example: 
\begin{inparaenum}[\it a)]
\item \quotes{Did you use the auto-converter code tool provided by the IDE?},
\item \quotes{Which was the criterion (if any) to choose those classes to migrate?},
\item \quotes{Your project still has Java code, Why has it not been completely migrated yet?}.
\end{inparaenum}

We choose this format of exploratory survey, composed of an initial question and followed by a loosely structured questionnaire, to follow the recommendations given by~\cite{experimentationSE2012}, which indicates that letting interviewers handle the questionnaire instead of the respondents themselves offers a number of advantage, such as observing the answers and ask questions according to the observation. 

\subsubsection{Survey setup}

\miga{} framework is able to return \emph{all} commits that migrate Java code to Kotlin from our dataset of Android applications (Section \ref{sec:dataset}).
From each commit, we retrieved the name 
and the email address of the developer that made the commit.
That information is the repository history (GIT).
Then, we sent to each developer that made a migration a personalised email that mentioned that we have analyzed the code of her/his application (mentioning the app name) and we have detected that she/he has write a commit (or several) that migrated code from Java to Kotlin. 

\subsection{Survey results}

We could successfully send, in total, 249 emails.\footnote{Some emails could not be successfully delivered (e.g., those from development companies which employers do not work there any more).}
We got the response from \nremailreplies{} developers, all them from different projects.
This means that $\sim$30\% of developers that migrated Java code to Kotlin in applications from the dataset we study (Section \ref{sec:dataset}) have participated in our survey.
Those interviewed developers are from, at least, 17 countries.
%Even the goal of this paper is not to present a demography study of developers (we did not ask about their country, experience, current status, etc), 
%by analyzing their profiles and email addresses we obtained that those developers are from, at least, 17 different countries. 
%Germany, United States, Korea, Japan, China, India, Brazil, Portugal, Czech Republic,  Spain, France, Canada, Portugal, Italy, Switzerland, Netherlands, among others.
Note that not all participants replied \emph{all} the questions we asked them.
Along this paper we \emph{literally} present answers from developers, without doing any kind of modification (e.g., typos or grammar issues).

Once we collected all answers, 
we detailed analyzed each interview (i.e., a thread of emails with answers and responses) to collect all valuable information for responding research questions 3 (why they migrated), 4 (why not fully migrated) and 5 (advises).


\subsection{Dataset of Android Applications studied}
\label{sec:dataset}
Given Google has officially adopted Kotlin as programming language for Android, 
our goal is to study the migration from Java to Kotlin of Android applications.
For this reason, we analyze Android applications from the FAMAZOA dataset \cite{GoisMateus2019}, which contains 374 Android  with at least one commit done in Kotlin.
FAMAZOA dataset was built by combining open-source applications mined from different sources such as F-Droid\footnote{F-Droid: dataset of open-source Android applications \url{https://f-droid.org}} repository and Android Time Machine \cite{Geiger2018:data}.


%%%%%%%%%% RQs from TSE


%\newcommand{\rqevolution}{{RQ 1: How do mobile apps having Kotlin code evolve during their history?
%}}


\newcommand{\rqappsmigrated}{{RQ 1: How many Android applications have been fully migrated to Kotlin?
}}


\newcommand{\rqmigrationdone}{{
RQ 2: How did developers migrate from Java to Kotlin?
}}

\newcommand{\rqwhymig}{{RQ 3: 
%Why did developers migrate?
Why (for which reasons) have developers migrated their Android applications from Java to Kotlin?
}}


\newcommand{\rqwhynotmig}{{RQ 3: 
Why do developers not \emph{fully} migrate their Android applications from Java to Kotlin?
}}


\newcommand{\rqproportion}{{RQ 4: Are the mobile apps which latest versions have both Java and Kotlin in  process of being migrated?}}




\newcommand{\rqadvise}{{RQ 5: What are the main advises to Android developers based on the interviews?}} 


The research questions that guide our research are:
\begin{enumerate}

\item{\it{ \rqappsmigrated{} }}

We automatically analyze a dataset of Android apps having Kotlin code to filter those that have been fully migrated from Java to Kotlin.

%{\bf \underline{Finding}:} 
\finding{From 374 Android apps analyzed, 86 apps have been completely migrated from Java to Kotlin.}

%\new{To know how many applications were migrated from Java to Kotlin, we analyze the programming language used at the beginning of the development (i.e., firsts commits) and at the most recent commits.
%This analysis would allow to classify apps in 3 classes:
%\begin{inparaenum}[\it a)]
%\item apps only written in Kotlin
%\item Apps fully migrated from Java to %Kotlin
%\item Apps partially migrated from Java to Kotlin.
%\end{inparaenum}
%}


\item  {\it{\rqmigrationdone}}

We analyze the history (code repository) of Android applications that have been fully migrated.
We compute for each app the portion of the history corresponding to the migration.
Then, we  retrieve the commits that carry out the code migration.
From them, we are able to identify the developers that have written the migrations.

\finding{
%The majority of those apps (53) have been migrated in less than 10 consecutive commits \todo{continue}
The  36\%  of  the  migrated  applications  were  completely migrated in one single commit.
%
Those apps do not have any version that contains both Java and Kotlin.
%Moreover, 
}

%
%This allow us 

%In this section we analyze the apps that were initially  written in Java and then, along their history,  were completely migrated to Kotlin with the goal of characterizing the migration activity.

%We analyze the following dimensions:
%\begin{enumerate}
%\item Duration of the migration from  Java to Kotlin (in terms of \#commits),
%\item Detection of commits that migrate code,
%In particular, we focus on two types of migrations defined in Section \ref{sec:miga:migrationanalyzers}:
%\begin{inparaenum}[\it 1)]
%\item File-level migration, and 
%\item Method-level migration. 
%\end{inparaenum}
%\item Inter-language change patterns  that occur on commits that affect both Kotlin and Java files, 
%\item Commit messages of migration commits.
%\item \new{use of Tool?}.
%\end{enumerate}


\item{\it{\rqwhymig}}

We ask developers that have migrated code the main reasons of migrating their Android applications.
%of adopting Kotlin code.
%


\finding{We present the ten main reasons we extracted from the interviews, those include: 
\begin{inparaenum}[\it a)]
\item to avoid limitations of Java versions, 
\item to produce safer code, 
\item to use a modern program language with new features, and 
\item to follow Google's direction.
\end{inparaenum}
}

\item {\it{ \rqproportion}}

We study the apps apps having both languages, but not completely migrated, to determine whether they are in the process of being  migrated from Java to Kotlin.
%\todo{Say something about the trend}
We also contact those developers to know the reasons about those application have not been fully migrated yet.

\finding{For, at least, the 63\% of the  214 apps not completely migrated, the amount and proportion of Kotlin code increase along the time.
The interviews with developers show that they did not finish the migration because of:
\begin{inparaenum}[\it a)]
\item only Java code that needs to be modified is migrated, 
\item only new code is written in Kotlin,
\item lack of time to complete the migration.
\end{inparaenum}
}

\item{\it{\rqadvise}}

We present recurrent episodes and advises that developers mentioned us during the interviews.
%We summarize the main advises developers mentioned us during development 
%based on the interviews which can be used as advises by
%Android developers that plan to migrate from Java to Kotlin.

\finding{We found that:
\begin{inparaenum}[\it a)]
\item Developers used the auto-converter tool for migrating code, however, the converted code often needs to be manually modified;
\item Coroutines simplify the implementation of concurrency in Android;
\item Kotlin code is easier to read and maintain according to the majority of the interviewed developers.
\end{inparaenum}
}

%\new{The interviews with Android developers give us the opportunity to capture the events that could we used by Android developers that have not programmed their Android apps using Kotlin yet.
%\todo{refine}}


\end{enumerate}


%%%%%%%%%end RQs from TSE


%%%% Table Future work
\begin{table}[t]
%\scriptsize
\tiny
\centering
 \begin{tabular}{|l |l|l|} 
\hline
{\tiny Size}&{\tiny Support}&Frequent Item sets\\
\hline
\hline
2 &1.60 \%&  UPD-Invocation in Method (J), UPD-Method Invocation in Method (K)\\
\hline
2 &0.94 \%&  UPD-Local Variable in If (J),UPD-Method Invocation in Method (K)\\
\hline
2 &0.94 \%&  UPD-Invocation in Method  (J), UPD-Property Declaration (K)\\
\hline
2 &0.75 \%& UPD-Local Variable  in Method (J),  UPD-Method Invocation inside If (K)\\
\hline
2 &0.72 \%&  UPD-Invocation in Method (J), INS-Method in Class (K)\\
\hline
\multicolumn{3}{|c|}{...}\\
\hline
2 &0.42 \%&  DEL-Method in Class (J), INS-Method in Class (K)\\
\hline
\multicolumn{3}{|c|}{...}\\
\hline
%2 &0.70 \%&  UPD-Invocation Method (J), INS-Property Declaration inside Method (K)\\
%\hline
%\multicolumn{3}{|c|}{...}\\
%\hline
4 &0.40 \%& DEL-If in Method (J), DEL-Assignment in If (J),\\
 &&  UPD-Local Variable Method (K), UPD-Method Invocation in If (K)\\
\hline

\multicolumn{3}{|c|}{...}\\

\hline

 \end{tabular}
\caption{Sample of most frequent item sets. Each item is composed by
a) action (Insert, Delete, Update),
b) entity type (e.g., Invocation),
c) language (`J' for Java, `K' for Kotlin).
}
\label{tab:apriori}
\end{table}

%%%%%%%%%%%%


%%% Miga steps:
\subsubsection
{Architecture and Implementation of \miga{}}
\label{sec:architecture}


\miga{} is built on top of Coming \cite{coming2019}, a framework for studying the evolution of applications.
\miga{} frameworks takes as input the location of a GIT repository on disk. 
It navigates each commit in chronological order, starting from the oldest one.
\miga{} extends Coming with new analyzers for studying the migration of applications. 
In particular, \miga{}: 
\begin{inparaenum}[\it a)]
\item {Analyzes added, removed and modified files from a commit},
\item {Analyzes commit messages},
\item {Creates  Java ASTs for the Java files affected by a commit},
\item {Creates  Kotlin ASTs for the Kotlin files affected by a commit},
\item {Computes the differences introduced by a commit at the AST level},
\item {Based on the output previous steps, it detects commits that migrate code using heuristics}.
As output, \miga{} generates a JSON file containing, for each commit, the information produced by each aforementioned analyzers.
\end{inparaenum}


\subsubsection{Heuristics for Detecting commits that migrate code}
\label{sec:commit_migration}

We now focus on the three heuristics we implement on  \miga{} to detect three types of commits that migrate code.

\paragraph{File-level Migration}
\label{sec:file_migration}
\miga{} is able to detect \emph{File-level Migrations} commits.
They are commits that migrate code
by removing one Java file and adding a new Kotlin file.
\miga{} checks that  the names of those files are the same (excluding the file extension).

\paragraph{Finer-grained code level migration}
\label{sec:fine_grained_migration}
\label{sec:method_migration}

\miga{} is able to detect  commits that migrate code at a fine-grained level, which we named \emph{code-level migration}.
This type of migration happens when a developer migrates code by updating two (or more) existing files written in two different languages: 
Java code is removed and Kotlin code is added.
%
The current implementation of  \miga{}  is able of detecting on \emph{methods} level migrations.\footnote{
Even it is not covered in this paper, \miga{} can detect other code-level migrations, such as properties or blocks.}

For detecting method-level migration commits, \miga{} applies the following steps on each commit:
\begin{inparaenum}[\it a)]
\item verifies that 1 or more Java files \emph{and} 1 or more Kotlin files are updated by a commit $c$;
\item for each updated Java or Kotlin file $f$, \miga{} creates an AST (Abstract Syntax Tree) from $f$ and another from the previous version of $f$, i.e. $f_p$;
\item \miga{} computes the differences between the ASTs obtained from $f$ and  $f_p$, using GumTree algorithm \cite{Falleri:2014:FAS}. The output is a list of AST changes, where each change is an operation (Insert, Remove, Update and Move) done over an AST node;
\item \miga{} finds for INSERT operations that affect \emph{methods} in the $diff$ obtained from comparing Kotlin files, and DELETE operations that also affect methods in the other $diff$ obtained from comparing Java files.\footnote{By default, \miga{} does not match the method names, even it is possible to apply string matching heuristics.}
\end{inparaenum}

\paragraph{Update-Insert Migration}
\label{sec:update_insert_migration}
%
%
\miga{} can detect commits that removes a piece of code (e.g., method) from a file written in Java and, at the same time, adds a new file written written in Kotlin.
The implementation of this detector is based on the two previously described cases.

\paragraph{Other types of migrations}
Beyond those three types of commits that migrate code, there could be other that also migrate code.
%
We leave the discover and characterization of such types, and the detection of commit corresponding to the emerging types for future work. In Section \ref{sec:discussion} we discuss some future directions for discovering them.


% end miga steps

==> old-content/removed_initial_version.tex <==
%%%%Old metodology 3.3.3

\subsubsection{Introduction moment}
\label{sec:method:intromoment}

For responding the two first research questions (RQ1 and RQ2), we find, for each application $A$, the commit that first introduces Kotlin code. Then we compute the number of that commit  i.e., the index of them in a list of commits from $A$, chronologically sorted.
Finally, the \emph{introduction moment} is this commit number divided by the total number of commits from $A$. For example, if an application has 60 commits and Kotlin is introduced in the commit number 25, the \emph{introduction moment}  is 15 / 60 = 0.25.


%%%%Old 4.2.1
\subsubsection{Introduction of Kotlin}
\label{sec:res:introkotlinmig}

\begin{figure}[!t]
\centering
%\begin{subfigure}
 \includegraphics[scale=0.5]{histogram_introduction_kotlin_percentage_86.pdf}
  \caption{Introduction of Kotlin on the 86 applications from set \emph{\migrapps}  initially written  in Java and then completely migrated to Kotlin.}
 \label{fig:kotlin_intro_totally_migrated}
%\end{subfigure}
\end{figure}

Histogram from Figure \ref{fig:kotlin_intro_totally_migrated} shows the \emph{introduction} moment of those applications completely migrated from Java to Kotlin. 
We highlight from the figure three \emph{clusters} of applications. 
\begin{inparaenum}[\it a)]
\item A first group of apps written in with Kotlin since the beginning (but not necessary since the first version). 
App `{SheepsGoHome}' is one of those apps. 
\item A second group were Kotlin was introduced at the middle of the application's history, for example, app `Coins-android' has 702 commits and Kotlin was introduced in the commit number 379.
\item A last group (smaller than the previous two) with a \emph{late} introduction of Kotlin. 
Apps `SimpleBitcoinWidget', `LocalStorage', which code evolutions are presented in Figures \ref{fig:linesSimplebitcoinwidget} and \ref{fig:linesLocalstorage} respectively, are two apps with late introduction of Kotlin.
\end{inparaenum}


%%%OLD 4.1.4

\subsubsection{Types of files affected by commits}
\label{sec:commitscomposition}


\begin{figure}[t!]
\begin{subfigure}{0.48\linewidth}
 \includegraphics[scale=0.4]{compositionMigratedFromJava.pdf}
  \caption{Distribution of the percentage of commits according to the type  considering Apps completely migrated from Java to Kotlin. (86 apps in total)}
 \label{fig:composition_commits_migrated}
\end{subfigure}
\hfil
\begin{subfigure}{0.48\linewidth}
 \includegraphics[scale=0.4]{compositionBoth.pdf}
\caption{Distribution of the percentage of commits according to the type  considering  Apps with Java and Kotlin at the latest version (214 apps in total).}
 \label{fig:composition_commits_both_final}
 \end{subfigure}
\caption{Distribution of Types of Commits: Pure-Java, Pure-Kotlin, Mix-Java-Kotlin, Other (e.g., configuration files). \todo{It should be nice pre-and post introduction}}
\label{fig:dist_commits}
\end{figure}




Figure \ref{fig:dist_commits} presents the distribution of the percentage of commits  of apps previously mentioned according to the commit classification presented in Section \ref{sec:method:proportion}. 

Sub-figures \ref{fig:composition_commits_migrated}  considers only commits from the set \emph{\migrapps} and shows that most of the commits affect files that  include neither Java nor Kotlin (bar `Other`), for example, those are XML and pom (Maven configuration) files. 
Then, the rest of the commits affects one program language (either Java or Kotlin). 
The distribution of Pure-Java and Pure-Kotlin commits are similar, but with a slightly larger percentage of Pure-Kotlin  commits than Pure-Java.
Finally, few commits affect both languages at the same time (Mix-Java-Kotlin). 

Sub-figure \ref{fig:composition_commits_both_final} considers apps from \emph{\colanguage{}}.
The distribution is different from that one observed from completely migrated apps (set \emph{\migrapps}): they have more Pure-Java commits than Pure-Kotlin.
Moreover, the distribution of Other files seems similar.
Finally, the percentage of commits affecting both Kotlin and Java (`Mix') is lower than those `Pure', but larger than the distribution of the same type of commits on set \emph{\migrapps}.
Indeed, Mix commits presents some outliers showing that those can represent more than the 20\% of the commits. %\footnote{BikeSharing is one for such apps: :  BikeSharing: 52.38 9.52 28.57 9.52 100.00 } 


\begin{tcolorbox}
%Finding: 
Most of the commits from apps having both languages only affect one single programming language. Few commits affect, at the same time, Kotlin and Java code.
\end{tcolorbox}

%%%%%

%%From  methodology
\subsubsection{Inter-language change pattern}
\label{sec:method:changepatterns}

%\subsubsection{Detecting change patters using frequent itemsets}
%\label{sec:method:fis}

In this work, we focus on finding change patterns (we call them `Inter-language change pattern')  that represent  frequent changes  done by commits that affect both Kotlin and Java code
%Those changes are present in commits that updates one or more Kotlin files and one or mode Java Files.
For that, we apply frequent itemset  algorithm \cite{Agrawal:1993:MAR} over the code changes taken from such commits.
A \emph{frequent itemset} is, given examples that are sets of items and a minimum frequency,  any set of items that occurs at least in the minimum number of examples \cite{Toivonen2010}.  
In our case, an \emph{item} is a single AST change  (see Section \ref{sec:ast_diff}) and an \emph{example} is a set of all AST changes  associated to a code element (e.g., a Commit, Method, File, etc.) affected by a commit.
%We represent a item as follow
An item is represented as a String, thus we transform an AST change  by joining:
\begin{inparaenum}[\it a)]
\item AST action (e.g., Insert),
\item type of the affected AST node,
\item the types of the parent's node,
\item the language (Koltin or Java)
\end{inparaenum}
In this experiment we use the code granularity defined by ChangeDistiller \cite{Fluri2007CDT} (e.g., invocations, assignments, control flow instructions).

Then, we create examples from all commits  affecting both Java and Kotlin files by combining each example taken from an updated Java file  with each one taken from an updated Kotlin file.
Consequently, each example has: 
\begin{inparaenum}[\it a)]
\item one or more items corresponding to changes in Kotlin code, and 
\item one or mores item corresponding to changes in Java code.
\end{inparaenum}


\begin{comment}

In this paper, we focus on finding change patterns at the \emph{method}-level, as done by different previous work \cite{}.
Consequently, an \emph{example} has all the changes from a commit associated to a particular method.
This means that, for example, we create 2 examples from a commit that changes two methods. 
We use Apriori  algorithm \cite{Agrawal:1996:FDA} for finding frequent itemsets.


\end{comment}

\subsubsection{Analysis of Commit Messages from Migration commit}
\label{sec:method:commitmessages}
\todo{remove?}
We find for keywords  that may sugest  migrations inside the  messages  asociated to migration commits (Section \ref{sec:file_migration}) from applications that have been completely migrated from Java to Kotlin.
The list of keywords we used is: 
`convert*',  `migrat*', `rewrit*', `updat*', `port*', `switch*', `transf*', `mov*', and `shift*'.

\new{
We found that the official Kotlin documentation highlights the ability of doing the staggered migration:
\quotes{Kotlin's philosophy is that you don't have to migrate the entire application. Start with a single module or feature, see how it goes, and then gradually move other parts as you see fit}.\footnote{Kotlin documentation: last visit 20-03-2020. \url{https://www.jetbrains.com/lp/mobilecrossplatform/}}
This is possible because Java and Kotlin are 100\% interoperable.
}


%%%%%% OLDS methodology - heuristic

%
\paragraph{Method-level migration}
\label{sec:method_migration}
It corresponds to commits that  remove a method from a Java file and add a method in a Kotlin file.
The heuristic for detecting such migration first verifies, for each commit $C$, that 1 or more Java files \emph{and} 1 or more Kotlin files are updated by $C$.
If that happens, the heuristic computes the two edit-scripts using the AST (Abstract Syntax Tree) differencing algorithm GumTree \cite{Falleri:2014:FAS}.
An AST level edit-script is a set of operations (Insert, remove, update and move) that transform one AST from a file into another AST.
The first one, $edit\_script_{Java}$,  contains the changes between the Java file updated by $C$ and its previous version.
The second one, $edit\_script_{Kotlin}$, contains the changes between the Kotlin file updated by $C$ and its previous version.
Finally, the heuristic searches for Delete operations that affect methods from $edit\_script_{Java}$ and for Insert operations that affect methods from $edit\_script_{Kotlin}$.
If it finds those methods, it marks commit $C$ as \emph{method}-level migration.

\paragraph{Update-Insert Migration}
\label{sec:update_insert_migration}
It corresponds to commits that remove a piece of code (e.g., a method) from a file written in Java and, at the same time, add one or more new files written in Kotlin.
The heuristic checks if a commit $C$ adds a Kotlin file, updates a Java file $F_J$  and the $edit\_script_{Java}$ between $F_J$ and its previous version contains Delete operations that affect methods.

==> old-content/tab-patterns.tex <==
\begin{table}[t]
\centering
 \begin{tabular}{|c | r |   r|  } 
 \hline
 %min_support: 0.01 minleng: 1 max_len: 6
min_support: 0.01 minleng: 1 max_len: 1
 &10.03 \%& K-UPD-TypeRef$Simple$Piece TypeRef$Simple Type\\
 &9.90 \%& K-UPD-Expr$Name Expr$Call CALL\\
 &7.08 \%& K-INS-Decl$Func Decl$Structured File\\
 

%%


 \hline
 \end{tabular}
\caption{}
\label{tab:patterns}
\end{table}

==> old-content/tabfindings.tex <==
 \begin{table}[ht]
 \centering
 \scriptsize
 %\renewcommand{\arraystretch}{1.2}
 \caption{Our major findings and their implications.}
 
\begin{tabular}{|p{5.5cm}|p{5.5cm}|}
\hline
\rowcolor{lightgray} \textbf{Findings on Features Adoption} & \textbf{Implications} \\
\hline
(1) 
&
(1) 
\\
\hline
(2) 
&
(2) .
\\

\\
\hline
\rowcolor{lightgray} \textbf{Findings on Moment and Order of Introduction of Features} & \textbf{Implications} \\
\hline

(1) 
& 
(1) 
\\
\hline
\hline

\end{tabular}
\label{tab:findings}
\end{table}

==> old-content/tmp_infrastructure.tex <==
   
 % \item Kotlin feature study (all) \url{https://github.com/martinezmatias/javavskotlin}
\item Kotlin AST analyzer (dependency to coming), needs a Jar with the Kotlin parser
     \url{https://github.com/martinezmatias/javavskotlin/tree/master/KotlinASTParser}
It's used in the previous paper (somehow)
    
    
\item KotlinDiff \url{https://github.com/martinezmatias/KotlinDiff}. Main project repo with dependency to Kotlin Jar and copied classes from  (Kotlin AST analyzer) 
     
\item Kotlin feature extractor \url{https://github.com/brunomateus/KotlinAstFeatureExtractor/} Find the features. It's the jar we include in the coming extension. In IJ IDE.
    
    
 \item Kastree extension \url{https://github.com/martinezmatias/kastree_ext} In J
 
 
 How to compile in inJ.
 

==> old-content/update-files.tex <==
\subsubsection{Updates of existing files}

\label{sec:res:updatesfiles}

Now, we focus on commits that updates Java and/or Kotlin codes with the goal later of studying the migration patterns.



\paragraph{Update single language}
\label{sec:res:updatesinglelang}
We now focus on commits that introduces updates on files.
There are 134 projects that have updates of Kotlin files.
Those corresponds, on average, to the 25\% of the commits (21\% in median).

Regarding with Java, 126 projects has commits with updates of Java files.
Those corresponds, on average, to the 34\% of the commits (32\% in median).

Those commits that updates Java and/or Koltin code are the input for studying the \emph{intra-language} change patterns (as we study in Section \ref{}).


%Numbers Updates  java  : len: 126 min: 1 max: 676 mean: 125.42857142857143  median: 60.5 
%Numbers Updates java (Percentage): len: 126 min: 0.0034129692832764505 max: 0.9 mean: 0.338834031250763  median: 0.32307692307692304 
%Numbers Updates  Kotlin : len: 151 min: 1 max: 424 mean: 63.2317880794702  median: 33 
%Numbers Updates   Kotlin (Percentage): len: 151 min: 0.0011235955056179776 max: 0.8549222797927462 mean: 0.28028733651341264  median: 0.24324324324324326 

\paragraph{Update in both Java and Kotlin}
\label{sec:res:updatebothlangs}

From the 142 projects that has in the history both Java and Kotlin,
85 projects has commits that modifies both Kotlin and Java files.
On average the number those commits is 11.3 (which corresponds to the 4\% of the commits on average) and in media is 5.
Some projects such (TrekAdvisor) as  has last number of commits that update both kind of files: 100 (25\%).
Others, such as NHentai-android has few: 

Those commits that introduce modification on both Java and Kotlin are the input for studying the \emph{inter-languages} change patterns (as we study in Section \ref{}). 


\subsubsection{Number of AST changes}
\label{sec:res:astChanges}

==> old.tex <==
%\IEEEpeerreviewmaketitle

\begin{comment}
\subtitle{}

\titlerunning{Studying the migration from Java to Kotlin of Android Apps}
\author{ Matias Martinez \and  Bruno Gois Mateus}
\institute{
   M. Martinez \at
            Universit\'e Polytechnique Hauts-de-France, France\\
              UVHC - Campus Mont Houy - 59313 Valenciennes, France \\
            \email{Matias.Martinez@uphf.fr}
       \and
B. Gois Mateus \at
            Universit\'e Polytechnique Hauts-de-France, France\\
              UVHC - Campus Mont Houy - 59313 Valenciennes, France \\
              \email{Bruno.GoisMateus@etu.uphf.fr}\\
}

\end{comment}

The research questions that guide our research are:
\begin{enumerate}


\item{\it{\rqwhymig}}

We ask developers that have migrated code from their Android applications the main reasons about the migrations.
This research question is important to understand  limitations of the \emph{traditional} way to written Android apps i.e. using Java language.

\item {\it{ \rqwhynotmig}}

We focus on the application which have both languages on the latest version i.e., not completely migrated at the time of writing this paper.
We contact developers that wrote migrations on those apps to know the reasons about those applications have not been fully migrated yet.

This question is important to detect the difficulties developers have had when they adopted a new programming language to develop Android apps. 

%%%%%%% RQ 3

\item{\it{\rqadvise}}
We present recurrent episodes and advices made by developers gathered from the survey.


\end{enumerate}


%%%%%From dataset.


\subsection{Differences between Legacy migrations and Java to Kotlin migration}
\label{sec:differenceslegacy}
\todo{To intro?/RW?}

A Legacy system can be defined, according to Brodie and Stonebraker, as ``{a system that significantly resists modification and evolution}''~\cite{Brodie1995Legacy}.
Bisbal et al.~\cite{Bisbal1997Migration} mention that legacy systems can host problems as 
\begin{inparaenum}[\it 1)]
\item usually run on obsolete hardware,
\item maintenance can be expensive,
\item lack of clean interfaces to interact with other systems, and 
\item are difficult to extend.
\end{inparaenum}
%%
Consequently, the migration of such legacy systems offers more
flexibility, better system understanding, easier maintenance, and reduced costs~\cite{Bisbal1997Migration}.

However, the migration of Java to Kotlin has some peculiarities compared to legacy migration given by those definitions.
For instance, first, the underlying run-time environment (i.e., the Java virtual machine, or, in case of Android, the Android Runtime -ART- or Dalvik machines) don't need to be updated: Kotlin and Java both are compiled to Java bytecode. 
Second, Java and Kotlin are fully interoperable.
In other types of legacy migrations (e.g., COBOL to web~\cite{Colosimo2009Evaluatinglegacy}), the communication between migrated and not migrated components (or sub-systems) needs \emph{wrappers} (\cite{Bisbal1997Migration,Colosimo2009Evaluatinglegacy}) or \emph{gateways} (\cite{Brodie1995Legacy, Bisbal1997Migration}).
The fully-supported interoperability between Java and Kotlin means that those strategies to allow interoperability are not necessary during the migration from Java to Kotlin.


%%%%%%%%%%%%%%%
We implement the mentioned heuristic on an open-source tool called \miga~\cite{migatool}, built on top of Coming \cite{coming2019}, a framework for studying the evolution of applications.
\miga{} takes as input the location of a cloned GIT repository.
It navigates each branch from the repository in chronological order, starting from the oldest one. 
During the navigation, \miga{} analyzes each commit and applies the heuristic.
Finally, it outputs the list of the migration commits according to the heuristic.
For each commit, it reports:
\begin{inparaenum}[\it a)]
\item commit ID (SHA-1),
\item developer user name,
\item full name,
\item email,
\item branch it belong to, and
\item date.
\end{inparaenum}
That information allows us to contact developers that have migrated code.


\begin{comment}
\subsection{Migrations of Legacy systems}
\label{sec:differenceslegacy}
%\todo{To intro?/RW?}
\todo{moved to new section 2}
A Legacy system can be defined as ``{a system that significantly resists modification and evolution}''~\cite{Brodie1995Legacy}.
Bisbal et al.~\cite{Bisbal1997Migration} mention that legacy systems can host problems as usually run on obsolete hardware and lack of clean interfaces to interact with other systems.
The migration of Java to Kotlin has some peculiarities compared to legacy migration.
First, the underlying run-time environment (i.e., the Java virtual machine)
do not need to be updated: Kotlin and Java both are compiled to Java bytecode. 
Second, 
the communication between migrated and not migrated components on legacy migrations (e.g., COBOL to web~\cite{Colosimo2009Evaluatinglegacy}) needs \emph{wrappers} (\cite{Bisbal1997Migration,Colosimo2009Evaluatinglegacy}) or \emph{gateways} (\cite{Brodie1995Legacy, Bisbal1997Migration}).
The interoperability between Java and Kotlin means that wrappers and gateways are not necessary for migrating Java to Kotlin.

\end{comment}

==> removed_content_intro.tex <==
\begin{comment}
\finding{We present the ten main reasons we extracted from the survey, those include: 
\begin{inparaenum}[\it a)]
\item to avoid limitations of Java versions, 
\item to produce safer code, 
\item to use a modern program language with new features, and 
\item to follow Google's direction.
\end{inparaenum}
}
\end{comment}

\begin{comment}
\finding{For, at least, the 63\% of the  214 apps not completely migrated, the amount and proportion of Kotlin code increase \inred{along the time}.
The survey shows that they did not finish the migration because of:
\begin{inparaenum}[\it a)]
\item only Java code that needs to be modified is migrated, 
\item only new code is written in Kotlin,
\item lack of time to complete the migration.
\end{inparaenum}
}
\end{comment}



\begin{comment}
\finding{We found that:
\begin{inparaenum}[\it a)]
\item Developers used the auto-converter tool for migrating code, however, the converted code often needs to be manually modified;
\item Coroutines simplify the implementation of concurrency in Android;
\item Kotlin code is easier to read and maintain according to the majority of the interviewed developers.
\end{inparaenum}
}
\end{comment}




{\bf Mining changes using data mining techniques:}
We showed in Section \ref{sec:inter-patterns} that the output of \miga, in particular, the AST changes from migration commits, can be further analyzed to extract knowledge such as migration patterns from migration commits. 
Previous work has applied similar technique on code changes. For example, 
Negara et al. \cite{Negara:2014:MFC} applied frequent item set to detect change patterns from changes done by developers when they write code using IDEs.
Zimmermann et al. \cite{Zimmermann:2004:MVH} data mining techniques  to obtain association rules from version histories for suggesting and predicting likely further changes.
Similarly, Ying et al. \cite{Ying:2004} also used association rule mining to determine the change patterns.
Viggiato et al. \cite{VOFJK:ICSME19}  also used Apriori algorithm to find types of changes that frequently co-occur  in mobile and non-mobile
platforms. 
%They work  focuses on analyzing Java programs, where our focuses on mobile (Android) applications written in Kotlin and Java.
Our experiment, as novelty, focuses on mining patterns composed by changes done in different languages.


\subsubsection{\inred{Move?}Availability of modern features and built-in patterns}


Kotlin languages provides different built-in features that were highlighted by developers. 
One of them is the foremost mentioned Coroutines.
Another one, \emph{Extension function} feature, was mentioned as useful by thirteen developers.
This feature provides the ability to extend a class with new functionality without having to inherit from the class or use design patterns such as Decorator.\footnote{Kotlin Extensions: \url{https://kotlinlang.org/docs/reference/extensions.html}}
%
One developer wrote us about it: 
\quotes{apart from providing a clean way to refactor the code, extensions allow an alternative to Abstraction/Inheritance in order to achieve the Open/Closed Principle, which is invaluable}.

% Ability to extend class definitions and add functions which are available on them is also very useful construct. 

Five developers remarked the \emph{built-in design patterns} provided by Kotlin, which enforces some of the best practices of Java by design.
For example, \emph{Singleton} pattern using the keyword `Object' and \emph{Decorator} pattern using keyword `By'.

Also, most of developers remarked the importance of Kotlin standard libraries, which provide support in, for instance, Collections.
Fourteen developers remarked the importance of having lambdas and streams. 
As one developer said: 
\quotes{Android development stuck on old Java version without e.g. streams (supported only on API 23+). Kotlin standard lib fills these shortcomings}.  

{\bf Implication:} Using Kotlin, Android developers have the possibility to use a modern programming language, with features not always available on Java, and, at the same time, to reach all Android platforms. 


%%%commented
\begin{comment}
\point{Detection of technical debt:} 
\emph{Technical-debt} issues can appear on application after it was (partially or fully) migrated.
According to Avgeriou et al.~\cite{avgeriou_et_al:DR:2016:6693} the term \emph{technical debt} refers to delayed tasks and immature artifacts (code, architecture, design) that incur extra costs in the future in the form of increased cost of change during evolution and maintenance. 

A research challenge is to identify, define, model, and catalogue, technical-debt~\cite{Izurieta2016WorkingTD} associated to the migration from Java and Kotlin.
Other works has focused, for instance, on defining and analyzing the architecture of Android applications (e.g.~\cite{Verdecchia2019Guidelines,Bagheri2016ArchitetureAndroid}) and on the detection of \emph{architectural} technical debt issues (e.g. \cite{Verdecchia2018ATD}).
However, to our knowledge, no work has done studied the impact of the migration on the architecture of the application nor the technical debt that the migration could introduce.
\end{comment}
%% end commented

\begin{comment}
\point{Testing of migrated apps}:
A research challenge is to generate test cases which 
\begin{inparaenum}[\it a)]
\item do \emph{regression testing} after the migration (i.e., to verify the behaviour of the app has not change after the Java to Kotlin conversion)
\item verify the migrated code does not introduce new bugs.
\end{inparaenum}
One of the challenges we envision is to test the interaction between the migrated Kotlin code with the no migrated Java code.
Even both languages are interoperable, Kotlin is a null safe language, it tries to avoid nullable variables.
Consequently, the behaviour of the application can change (i.e., an exception is thrown) when the Java code passes \emph{null} values to the migrated Kotlin code, which could be written without contemplating the nullability of parameters and variables.
\end{comment}

==> summary_gray_litarature.tex <==
\subsection{Summary of gray-literature}

\cite{daga2018LinkJavaVsKotlin}
\begin{itemize}
    \item learning curve. "Kotlin can be viewed as an improvement on Java, rather than being a full-blown substitute"
     "Java and Kotlin share a number of syntaxes, too, making things easier for developers"
    \item The Issue With NullPointerExceptions
    \item Kotlin Is the "Modern" Language
    \item Interoperability
    \item Community Support
    \item verbosity (Includes dependency)
    \item Checked Exceptions 
    \item Increased Size of .apk
    \item Complete Support for Kotlin in Android Studio. (Includes conversion)
    `` Converting complete source files written in Java to Kotlin is also a breeze. Developers, of course, have to ensure that there are no code losses and/or data corruption during such conversion''
    \item Implicit Widening Conversions and the Question of Stability
    \item No Extra Garbage Collection
    \item First-Class Delegation in Kotlin
    \item Speed of Compilation
    \item Coroutines
    \item Conclusion "It is still advisable for newbie Android developers to learn Java first, and then attempt the switch to Kotlin (type aliases and immutability are two more USPs)"
\end{itemize}

\cite{Sommerhoff2020LinkJavaVsKotlin}

\begin{itemize}
\item Kotlin is more concise: "Features such as type inference, smart casts, data classes, and properties help achieve conciseness."
\item  Kotlin code is safer
\item Kotlin has better support for functional programming
\item  Kotlin speeds up every-day development tasks
\item Kotlin helps reduce errors and bugs in the code `The Kotlin compiler performs many checks, avoiding runtime errors and reducing the cost and effort of error fixes.`
\item The code base shrinks and increases in quality "Technical debt"
\item Developers will be more satisfied and excited about their work
\item  Engineers can take their skills to the next level
\item Kotlin community supports developers
\item Migrate to Kotlin in small steps
`` A good way to start the process is to introduce Kotlin in non-business-critical code to enable initial evaluation and let developers gain experience. For example, test cases can often be greatly simplified using Kotlin. While migration to a new programming language can seem daunting, in this case, the benefits of Kotlin outweigh the costs.``

\end{itemize}

\cite{Rishabh2017LinkKotlinAndroid}

Advantage:
\begin{itemize}
\item  Easy to Set Up: (Android Studio)
\item Interoperable With Java:
\item Includes Synthetic Extension
\item No More NullPointerExceptions (NPEs):
\end{itemize}


\cite{Thornsby2019LinkJavaVsKotlinKeyDiff}
\begin{itemize}
\item offers more succinct code – with no findViewByIds
\item Kotlin is null safe by default
\item Extension functions
\item Coroutines are first-class citizens
\item There are no checked exceptions
\item Native support for delegation (prevent the duplication of code)
``Kotlin’s class delegation is an alternative to inheritance that makes it possible to use multiple inheritance.''
\item Data classes
\item smart class
\item Support for constructors
\item No support for implicit widening conversions
\item Annotation processing libraries with Kotlin
\end{itemize}
``Perhaps most notably: many Android developers are simply more familiar with Java at this point''.


\cite{Caneco2017LinkMigrating}
\begin{itemize}
\item Reduce walls of text: 
\item Null safety: 
\item  built-in
\item Decrease the pain on Code Review: 
\item Run Java and Kotlin side-by-side: 
\item Make use of Java libraries

\end{itemize}

\cite{Caneco2017LinkMigrating}
The converter is a bit conservative on the code conversion, so we needed to perform a few human-based tweaks.




\begin{itemize}
\item  Adjusting nulls 
\item Inline variable initialization
\item Replace “companion object” fields with compile time “const”
\item Keep or remove `@Throws` annotation
\item Replace one-line methods with Kotlin Single Expression method
( Single Expression Functions )
\end{itemize}

"We were able to complete the migration in about six man.hours of effort: three man.hours for converting the code and three more man.hours for peer code review and tweaking.
The code base went down from 1.566 LoC to 1.128 LoC. That’s 23\% less code base to maintain and work on! 
"

\cite{Sommerhoff2015LinkKotlin} 
Enforcing Best Practices

\cite{Butterworth2020LinkMigration}
``There are some tools to help developers achieve this (such as the automatic Java to Kotlin conversion tool), but there are a number of pitfalls to be aware of when it comes to the converter and the interoperability between the languages. ''

``The important thing to remember here is that the Kotlin code generated by the converter may not output the same bytecode as the original Java''

\cite{Paul2018LinkLanguageStart}
``why I suggest a beginner Android developer starting with Java rather than Kotlin.''

``It can help you avoid all boiler-plate code, e.g. you don't need to specify getters and setters, equals(), hashCode() or toString() methods.''


``"What we do is we only take new functionality and write it in Kotlin. It is possible because Kotlin has great interoperability with Java. You can write a single class in Kotlin and keep the rest in Java, or have 99\% of your code in Kotlin and have only some of the leftovers in Java."''

\cite{Heath20LinkSwitch}

\begin{itemize}
\item interoperability
\item Kotlin first
    \item learning curve
    \item idiomatic code, Java style code
\end{itemize}
